Hub-Accelerator: Fast and Exact Shortest Path Computation in Large Social Networks

Shortest path computation is one of the most fundamental operations for managing and analyzing large social networks. Though existing techniques are quite effective for finding the shortest path on large but sparse road networks, social graphs have quite different characteristics: they are generally non-spatial, non-weighted, scale-free, and they exhibit small-world properties in addition to their massive size. In particular, the existence of hubs, those vertices with a large number of connections, explodes the search space, making the shortest path computation surprisingly challenging. In this paper, we introduce a set of novel techniques centered around hubs, collectively referred to as the Hub-Accelerator framework, to compute the k-degree shortest path (finding the shortest path between two vertices if their distance is within k). These techniques enable us to significantly reduce the search space by either greatly limiting the expansion scope of hubs (using the novel distance- preserving Hub-Network concept) or completely pruning away the hubs in the online search (using the Hub2-Labeling approach). The Hub-Accelerator approaches are more than two orders of magnitude faster than BFS and the state-of-the-art approximate shortest path method Sketch for the shortest path computation. The Hub- Network approach does not introduce additional index cost with light pre-computation cost; the index size and index construction cost of Hub2-Labeling are also moderate and better than or comparable to the approximation indexing Sketch method.

==> Figures/ALT.tex <==
\begin{algorithm}[t!]
\caption{ALT\_Query($s$,$t$)}
\label{alg:altquery}
\begin{small}
\begin{algorithmic}[1]
\REQUIRE procedure $ALT\_Preprocessing$ has been invoked to maintain distance vector $D(v)$ for each vertex $v$;
\STATE $Q_f \leftarrow V$; $Q_b \leftarrow V$; \COMMENT{they are priority queue for forward and backward search}
\STATE $Label_f(s) \leftarrow reach$; $Label_b(t) \leftarrow reach$;
\STATE $p_f(t) \leftarrow 0$; $p_b(s) \leftarrow 0$; \COMMENT{$p_f$ and $p_b$ are consistent potential functions based on vector $D$}
\STATE $d_f(s) \leftarrow 0$; $d_b(t) \leftarrow 0$;
\STATE $\mu \leftarrow \infty$; \COMMENT{shortest distance between $s$ and $t$}
\WHILE{TRUE}
%    \COMMENT{forward search}
    \STATE $v \leftarrow Q_f.top()$; \COMMENT{select $v$ from $Q_f$ with smallest $d_f(v)+p_f(v)$}
    \STATE $Label_f(v) \leftarrow scanned$;
    \IF{$Label_b(v) == scanned$}
        \RETURN $\mu$;
    \ENDIF
    \FORALL{$w \in Neighbor(v)$}
        \IF{$Label_b(w) == scanned$ \\ and $d_f(v) + l(v,w) + d_b(w) < \mu$}
            \STATE $\mu \leftarrow d_f(v)+l(v,w)+d_b(w)$;
        \ENDIF
        \IF{$d_f(v) + l(v,w) < d_f(w)$}
            \STATE $d_f(w) \leftarrow d_f(v)+l(v,w)$;
            \STATE decrease key of $w$ (i.e., $d_f(w)+p_f(w)$) in $Q_f$;
        \ENDIF
    \ENDFOR \\
    \COMMENT{backward search (omitted for simplicity)}
\ENDWHILE
\end{algorithmic}

\begin{algorithmic}[1]
\PROCEDURE{ALT\_Preprocessing($G=(V,E)$)}
\STATE select a set of vertices $L$ as landmarks based on certain criterion;
\FORALL{$v \in V$}
    \STATE compute vector $D(v)$ indicating the distances between $v$ and each vertex in $L$;
\ENDFOR
\end{algorithmic}

\end{small}
\end{algorithm}


==> Figures/CoreExtraction.tex <==
\begin{algorithm}[t!]
\caption{CoreExtraction($G=(V,E)$, $r$)}
\label{alg:coreextraction}
\begin{small}
\begin{algorithmic}[1]
\REQUIRE $r$ is the diameter constraint for core component
\STATE $V_c \leftarrow \emptyset$; $E_c \leftarrow \emptyset$; \COMMENT{$V_c$ and $E_c$ are vertex set and edge set for core}
\STATE randomly sample a set of vertices $R \subset V$ ($|R| = 0.01|V|$);
\STATE $Q \leftarrow \emptyset$; \COMMENT{$Q$ is priority queue to store edges in $P$ in the order of their betweenness $b(e)$}
\FORALL{$v \in R$}
    \STATE perform BFS from $v$ based on fixed node ordering and collect shortest paths with length $5$ and $6$ in $P$;
    \IF{$e \notin Q$}
        \STATE $Q.insert(e)$;
    \ELSE
        \STATE update key of edge $e$ (betweenness $b(e)$) in $Q$;
    \ENDIF
\ENDFOR
\WHILE{$Q \neq \emptyset$}
    \STATE select edge $e=(u,v)$ with maximum $b(e)$ from $Q$;
    \IF{$v \in V_c$ and $u \notin V_c$}
        \STATE generate BFS tree $T_u$ from $u$ by expanding $r$ steps;
        \IF{$V_c \subseteq V(T_u)$}
            \STATE $V_c \leftarrow V_c \cup \{u\}$;
            \STATE $E_c \leftarrow E_c \cup \{e\}$;
            \STATE collect the vertices $S \subseteq V_c$ such that shortest paths from $u$ to any $x \in S$ in $T_u$ do not pass any vertex in $V_c$;
            \FORALL{$x \in S$}
                \STATE $E_c \leftarrow E_c \cup \{(u,x)\}$ \COMMENT{weighted shortcut is added};
            \ENDFOR
        \ENDIF
    \ENDIF \\
    \COMMENT{consider the case $v \notin V_c$ and $u \in V_c$ in the same way, omitted here}
    \IF{$u \notin V_c$ and $v \notin V_c$}
        \STATE generate BFS trees $T_u$ and $T_v$ by expanding $r$ steps;
        \IF{$V_c \subseteq V(T_v)$}
            \STATE $V_c \leftarrow V_c \cup \{v\}$;
            \STATE collect the vertices $S \subseteq V_c$ such that shortest paths from $v$ to any $x \in S$ in $T_v$ do not pass any vertex in $V_c$;
            \FORALL{$x \in S$}
                \STATE $E_c \leftarrow E_c \cup \{(v,x)\}$ \COMMENT{weighted shortcut is added};
            \ENDFOR
        \ENDIF \\
        \COMMENT{process $T_u$ in the same way, omitted here}
        \IF{$V_c \subseteq V(T_u)$ and $V_c \subseteq V(T_v)$}
            \STATE $E_c \leftarrow E_c \cup \{e=(u,v)\}$;
        \ENDIF
    \ENDIF
\ENDWHILE
\RETURN $C_0 = (V_c,E_c)$;
\end{algorithmic}
\end{small}
\end{algorithm}


==> Figures/GreedyOrder.tex <==
\begin{algorithm}[t!]
\caption{GreedyOrdering($G=(V,E)$)}
\label{alg:greedyorder}
\begin{small}
\begin{algorithmic}[1]
\STATE $U \leftarrow \{(u,v) | d(u,v)=2\}$;
\FORALL{$v \in V$}
    \FORALL{$u,w\in N(v)$ and $(u,w) \notin E$}
        \STATE $C_v \leftarrow C_v \cup \{(u,w)\}$;
    \ENDFOR
\ENDFOR
\STATE $T \leftarrow \emptyset$; \COMMENT{$T$ records the selected vertices}
\FOR{$i=1$ to $|V|$}
    \STATE select vertex $x$ such that $|\{(u,v)| (u,v)\in C_x\cap U \mbox{ and } u,v\notin T\}|$ is maximized;
    \STATE $U \leftarrow U \setminus \{(u,v)|(u,v)\in C_x \mbox{ and } u,v \notin T\}$;
    \STATE $x.order \leftarrow |V|-i+1$;
    \STATE $T \leftarrow T \cup \{x\}$;
\ENDFOR
\end{algorithmic}
\end{small}
\end{algorithm}


==> Figures/GreedyOrder1.tex <==
\begin{algorithm}[t!]
\caption{GreedyOrderingMin($G=(V,E)$)}
\label{alg:greedyordermin}
\begin{small}
\begin{algorithmic}[1]
\FORALL{$v \in V$}
    \STATE $v.order \leftarrow \infty$;
\ENDFOR
\FOR{$i=1$ to $|V|$}
    \STATE select $v$ such that $|\{u | u\in N(v) \mbox{ and } u.order \neq \infty\}|$ is minimized;
    \STATE $v.order \leftarrow |V|-i+1$;
\ENDFOR
\end{algorithmic}
\end{small}
\end{algorithm}


==> Figures/HubExample.tex <==
\begin{figure*}[t!]
    \label{fig:coreindexexample}
    \centering
    \mbox{
        \subfigure[Original Graph]{\includegraphics[scale=0.5]{Figures/graph.eps}\label{graph}}
        \hspace{10mm}
        \subfigure[Hub$^2$]{\includegraphics[scale=0.4]{Figures/hubsquare.eps}\label{hubsquare}}
        \hspace{10mm}
        \subfigure[Hub Labeling]{\includegraphics[scale=0.6]{Figures/hubindexexample.eps}\label{hubindex}}
    }
    \vspace*{-1.0ex}
    \caption{{\small Example of Hub$^2$-Labeling}}
\end{figure*}

\comment{
\begin{example}
Now, let us take the Flicker as an example  network we used in experiments as example to get in-depth understanding.
The network contains around $1.7$ millions vertices and $22.6$ millions edges and we select $10K$ highest degree vertices as hub-set.
Using core landmark indexing scheme, each vertex only needs to record around $232$ core-hubs (i.e., around $2.3\%$ of entire hub-set), and total number of entries for Hub$^2$ is at most $100$ millions.
Distributing materialization cost of Hub$^2$ to each vertex, each vertex at most needs to record around $290$ ($=232+\frac{100M}{1.7M}$) entries, which is still significantly smaller than $10K$ in traditional landmark indexing scheme.
\end{example}
}


==> Figures/Landmark.tex <==
\begin{algorithm}[t!]
\caption{ALT\_LandmarkSelection($G=(V,E)$,$K$)}
\label{alg:altlandmark}
\begin{small}
\begin{algorithmic}[1]

\REQUIRE $K$ is the number of landmarks
\STATE select a set of vertices $S$ by random sampling;
\STATE $L \leftarrow \emptyset$; $Q \leftarrow \emptyset$; \COMMENT{priority queue for ranking boundary nodes}
\FORALL{$v \in S$}
    \STATE generate BFS tree from root $v$ and record its leaves by $Leaves(v)$;
    \FORALL{$w \in Leaves(v)$}
        \STATE $Q.insert(w)$;
        \STATE $s(w) \leftarrow s(w)+d(w)$; \COMMENT{$s(w)$ is accumulated distance from distance $d(w)$ in each BFS tree}
        \STATE $c(w) \leftarrow c(w)+1$; \COMMENT{$c(w)$ is the number of BFS trees taking $w$ as leaf}
    \ENDFOR
\ENDFOR
\FORALL{$v \in Q$}
    \STATE update key of $v$ by $s(w)/c(w)$ in $Q$;
\ENDFOR
\FOR{$i = 1$ to $K$}
    \STATE $L.push\_back(v=Q.pop())$; \COMMENT{extract the node with maximum key from $Q$ as landmark}
    \STATE remove nodes in $Q$ whose distance to $v$ is no greater than $3$;
\ENDFOR
\RETURN $L$;
\end{algorithmic}
\end{small}
\end{algorithm}


==> Figures/NodeContraction.tex <==
\begin{algorithm}[t!]
\caption{ContractionHierarchy($G=(V,E)$)}
\label{alg:nc}
\begin{small}
\begin{algorithmic}[1]
\REQUIRE node ordering is provided;
\STATE $E_2 \leftarrow \emptyset$; $E_3 \leftarrow \emptyset$; $E_4 \leftarrow \emptyset$; \COMMENT{$E_i$ is edge set storing shortcuts with length $i$} \\
\COMMENT{Following node order}
\FORALL{$v \in V$}
    \FORALL{unique shortest path $p=(u,v,w)$}
        \STATE $E_2 \leftarrow E_2 \cup \{u,w\}$;
    \ENDFOR
\ENDFOR \\
\COMMENT{Generate $E_3$}
\FORALL{$e=(u,v) \in E_2$}
    \FORALL{unique shortest path $p=(u,v,w)$ and $d(v,w)=1$}
        \STATE $E_3 \leftarrow E_3 \cup \{u,w\}$;
    \ENDFOR
\ENDFOR \\
\COMMENT{Generate $E_4$}
\FORALL{$e=(u,v) \in E_2$}
    \FORALL{unique shortest path $p=(u,v,w)$ and $(v,w) \in E_2$}
        \STATE $E_4 \leftarrow E_4 \cup \{u,w\}$;
    \ENDFOR
\ENDFOR
\FORALL{$e=(u,v) \in E_3$}
    \FORALL{unique shortest path $p=(u,v,w)$ and $d(v,w)=1$}
        \STATE $E_4 \leftarrow E_4 \cup \{u,w\}$;
    \ENDFOR
\ENDFOR
\end{algorithmic}
\end{small}
\end{algorithm}


==> Figures/QueryTimeFigures.tex <==
\begin{figure*}[tb]
    \label{fig:distquerytime}
    \centering
    \mbox{
        \subfigure[Facebook]{\includegraphics[width=1.6in,height=1.0in]{Figures/facebook-wall_randqtime_results.eps}\label{facebookwall}}
        \hspace{-10mm}
        \subfigure[Slashdot]{\includegraphics[width=1.6in,height=1.0in]{Figures/Slashdot_randqtime_results.eps}\label{slashdot}}
        \hspace{-10mm}
        \subfigure[BerkStan]{\includegraphics[width=1.6in,height=1.0in]{Figures/web-BerkStan_randqtime_results.eps}\label{webberkstan}}
        \hspace{-10mm}
        \subfigure[Youtube]{\includegraphics[width=1.6in,height=1.0in]{Figures/youtube_randqtime_results.eps}\label{youtube}}
        \hspace{-10mm}
        \subfigure[As-skitter]{\includegraphics[width=1.6in,height=1.0in]{Figures/as-skitter_randqtime_results.eps}\label{asskitter}}
%       \hspace{-10mm}
%       \subfigure[Flickr]{\includegraphics[scale=0.3]{Figures/Flickr_randqtime_results.eps}\label{flickr}}
    }
    \mbox{
	\subfigure[Flickr]{\includegraphics[width=1.6in,height=1.0in]{Figures/Flickr_randqtime_results.eps}\label{flickr}}
	\hspace{-10mm}
        \subfigure[Flickr-growth]{\includegraphics[width=1.6in,height=1.0in]{Figures/flickr-growth_randqtime_results.eps}\label{flickrgrowth}}
        \hspace{-10mm}
        \subfigure[WikiTalk]{\includegraphics[width=1.6in,height=1.0in]{Figures/WikiTalk_randqtime_results.eps}\label{wikitalk}}
        \hspace{-10mm}
        \subfigure[Orkut]{\includegraphics[width=1.6in,height=1.0in]{Figures/orkut_randqtime_results.eps}\label{orkut}}
%        \hspace{-10mm}
%        \subfigure[cit-Patents]{\includegraphics[scale=0.3]{Figures/cit-Patents_randqtime_results.eps}\label{citpatents}}
        \hspace{-10mm}
        \subfigure[LiveJournal]{\includegraphics[width=1.6in,height=1.0in]{Figures/soc-Journal1_randqtime_results.eps}\label{socjournal1}}
%        \hspace{-10mm}
%        \subfigure[topology]{\includegraphics[scale=0.3]{Figures/topology_randqtime_results.eps}\label{topology}}
    }
    \vspace*{-1.0ex}
    \caption{{\small Average Query Time (ms) on Random Query with Different Distance}}
\end{figure*}


==> Figures/RandomPreprocessing.tex <==
\begin{table*}[!ht]
\begin{center}
{\scriptsize
\begin{tabular}{|l|r|r|r|r|r|r|r|}
\hline
\multirow{2}{*}{Dataset}&  \multicolumn{ 5}{c|}{Indexing Cost (MB)} & \multicolumn{2}{c|}{Procomp. Time (min.)} \\
 \cline{2-8}
 &
\multicolumn{1}{c|}{Sketch-db} & \multicolumn{1}{c|}{Sketch-path}
& \multicolumn{1}{c|}{HL-index} & \multicolumn{1}{c|}{HL-path} & \multicolumn{1}{c|}{HL-total} &
\multicolumn{1}{c|}{Sketch} & \multicolumn{1}{c|}{HL} \\ \hline

%Email-Enron    &   10.2    &   52.9    &   15.3    &   663.9   &   679.2   &   3.2 &   1.3 \\  \hline
Facebook    &   10.2    &   107.2   &   20.5    &   1174.2  &   1194.7  &   3.2 &   1.4 \\  \hline
Slashdot    &   26.1    &   171.6   &   38.5    &   491.4   &   529.9   &   6.5 &   4.3 \\  \hline
BerkStan    &   193 &   2035    &   386.4   &   217.4   &   603.8   &   64.3    &   1.7 \\  \hline
%Google &   171.6   &   2035    &   495.4   &   121.9   &   617.2   &   73.9    &   1.5 \\  \hline
Youtube &   217.2   &   2575.6  &   656.8   &   503.1   &   1159.9  &   100.8   &   66  \\  \hline
As-skitter  &   391.3   &   2897.5  &   965 &   268.3   &   1233.3  &   109.9   &   31.7    \\  \hline
Flickr  &   626.7   &   4641.2  &   1059.3  &   344.5   &   1403.7  &   163.8   &   202.5   \\  \hline
Flickr-growth    &   1003.9  &   6608.3  &   1312    &   338.7   &   1650.7  &   242.8   &   363.5   \\  \hline
WikiTalk    &   -   &   -   &   1364.4  &   446.9   &   1811.2  &   -   &   41.2    \\  \hline
Orkut   &   6608.3  &   8363.6  &   13173.3 &   312 &   13485.4 &   773.2   &   1431.6  \\  \hline
%cit-Patents &   793.2   &   2897.5  &   2154.2  &   2.6 &   2156.8  &   115.9   &   1   \\  \hline
LiveJournal   &   2289.4  &   19074.8 &   17244.3 &   443 &   17687.3 &   707.3   &   693.3   \\  \hline
%topology &   6608.3  &   30554   &   9769.7  &   274 &   10043.8 &   1494.4  &   1322.6  \\  \hline


\end{tabular}
}
\end{center}
\vspace{-2.0ex}
\caption{Preprocessing Cost based on Random Query}
\label{tab:precomp}
\vspace*{-1.0ex}
\end{table*}


\comment{
\begin{table*}
\begin{center}
{\small
\begin{tabular}{|l|r|r|r|r|r|r|r|r|}
\hline
\multirow{2}{*}{Dataset}&  \multicolumn{ 6}{c|}{Indexing Cost (MB)} & \multicolumn{2}{c|}{Procomp. Time (min.)} \\
 \cline{2-9}
 &
\multicolumn{1}{c|}{Sketch-db} & \multicolumn{1}{c|}{Sketch-path} & \multicolumn{1}{c|}{Sketch-total}
& \multicolumn{1}{c|}{CL-landmark} & \multicolumn{1}{c|}{CL-path} & \multicolumn{1}{c|}{CL-total} &
\multicolumn{1}{c|}{Sketch} & \multicolumn{1}{c|}{CL} \\ \hline

%Email-Enron    &   10.2    &   52.9    &   63.1    &   15.3    &   663.9   &   679.2   &   3.2 &   1.3 \\  \hline
Facebook    &   10.2    &   107.2   &   117.4   &   20.5    &   1174.2  &   1194.7  &   3.2 &   1.4 \\  \hline
Slashdot    &   26.1    &   171.6   &   197.7   &   38.5    &   491.4   &   529.9   &   6.5 &   4.3 \\  \hline
BerkStan    &   193 &   2035    &   2228.1  &   386.4   &   217.4   &   603.8   &   64.3    &   1.7 \\  \hline
%Google &   171.6   &   2035    &   2206.6  &   495.4   &   121.9   &   617.2   &   73.9    &   1.5 \\  \hline
Youtube &   217.2   &   2575.6  &   2792.8  &   656.8   &   503.1   &   1159.9  &   100.8   &   66  \\  \hline
As-skitter  &   391.3   &   2897.5  &   3288.8  &   965 &   268.3   &   1233.3  &   109.9   &   31.7    \\  \hline
Flickr  &   626.7   &   4641.2  &   5268    &   1059.3  &   344.5   &   1403.7  &   163.8   &   202.5   \\  \hline
Flickr-g    &   1003.9  &   6608.3  &   7612.2  &   1312    &   338.7   &   1650.7  &   242.8   &   363.5   \\  \hline
WikiTalk    &   -   &   -   &   -   &   1364.4  &   446.9   &   1811.2  &   -   &   41.2    \\  \hline
Orkut   &   6608.3  &   8363.6  &   14971.9 &   13173.3 &   312 &   13485.4 &   773.2   &   1431.6  \\  \hline
%cit-Patents &   793.2   &   2897.5  &   3690.7  &   2154.2  &   2.6 &   2156.8  &   115.9   &   1   \\  \hline
LiveJournal &   6608.3  &   30554   &   37162.3 &   9769.7  &   274 &   10043.8 &   1494.4  &   1322.6  \\  \hline
%topology    &   2289.4  &   19074.8 &   21364.2 &   17244.3 &   443 &   17687.3 &   707.3   &   693.3   \\  \hline


\end{tabular}
}
\end{center}
\vspace{-2.0ex}
\caption{Preprocessing Cost based on Random Query}
\label{tab:precomp}
\vspace*{-1.0ex}
\end{table*}
}


==> Figures/SizevarQueryTime.tex <==
\begin{table}
\begin{center}
{\scriptsize
\begin{tabular}{|l|r|r|r|r|r|r|r|}
\hline
Dataset &  BFS  & BiBFS & HL-5K  & HL-8K & HL-10K & HL-12K & HL-15K \\ \hline

Facebook    &   0.76    &   0.03    &   0.0022  &   0.0007  &   0.0005  &   0.0005  &   0.0148  \\  \hline
Slashdot    &   2.04    &   0.05    &   0.0045  &   0.0011  &   0.0006  &   0.0005  &   0.0242  \\  \hline
BerkStan    &   0.66    &   0.1 &   0.0138  &   0.0094  &   0.0071  &   0.0052  &   0.0048  \\  \hline
Youtube &   52.64   &   0.37    &   0.0583  &   0.0157  &   0.0277  &   0.0196  &   0.0161  \\  \hline
As-skitter  &   17.62   &   0.29    &   0.0784  &   0.0442  &   0.0348  &   0.0254  &   0.0226  \\  \hline
Flickr  &   187.3   &   0.74    &   0.2317  &   0.2063  &   0.1844  &   0.1738  &   0.1609  \\  \hline
Flickr-growth    &   249.27  &   0.95    &   0.3384  &   0.3116  &   0.2755  &   0.2697  &   0.2447  \\  \hline
WikiTalk    &   40.41   &   0.17    &   0.0018  &   0.0009  &   0.0007  &   0.0007  &   0.0006  \\  \hline
Orkut   &   862.39  &   16.89   &   1.0911  &   1.3141  &   1.4383  &   1.4582  &   2.1896  \\  \hline
cit-Patents &   0.19    &   0.11    &   0.0838  &   0.0814  &   0.0875  &   0.0787  &   0.0832  \\  \hline
LiveJournal &   586.95  &   2.93    &   0.5236  &   0.6177  &   0.6863  &   0.7413  &   2.3184  \\  \hline
topology &   1490.63 &   8.44    &   0.5782  &   0.5003  &   0.4095  &   0.4189  &   0.3814  \\  \hline

\end{tabular}
}
\end{center}
\vspace*{-2.0ex}
\caption{Average Query Time (ms) of Random Queries on Different Landmark Size}
\label{tab:sizevarquerytime}
\vspace*{-1.0ex}
\end{table}


==> Figures/SizevarResults.tex <==
\begin{table*}
{\small

\begin{tabular}{|l|r|r|r|r|r|r|r|r|r|}
    \hline
    \multirow{2}{*}{Dataset}&  \multicolumn{ 5}{c|}{Indexing Cost } & \multicolumn{3}{c|}{Preproc.Time(min)} \\
    \cline{2-9}
    &
     \multicolumn{1}{c|}{Sketch-path} & \multicolumn{1}{c|}{HN-total} & \multicolumn{1}{c|}{HL-total}
    & \multicolumn{1}{c|}{{\small avg.$|L_H(v)|$}} & \multicolumn{1}{c|}{Hub$^2$} &
    \multicolumn{1}{c|}{Sketch} & \multicolumn{1}{c|}{HN} & \multicolumn{1}{c|}{HL} \\ \hline

Facebook	&	10.2MB	&   & 955.2MB	&	8.2	&	953.0MB	&	3.2	&  &	1.4	\\	\hline
%Slashdot	&	26.1MB	&   &	496.3MB	&	11.1	&	491.4MB	&	6.5	&  &	4.3	\\	\hline
BerkStan	&	193MB	&  &	291.3MB	&	21.6	&	206.5MB	&	64.3	&  &	1.7	\\	\hline
Youtube	&	217.2MB	&  &	756.5MB	&	38.9	&	503.1MB	&	100.8	& &	66	\\	\hline
As-skitter	&	391.3MB	&  &	1.2GB	&	101.9	&	268.3MB	&	109.9	&	& 31.7	\\	\hline
Flickr	&	626.7MB	&  &	1.5GB	&	232	&	344.5MB	&	163.8	&	& 202.5	\\	\hline
Flickr-growth	  &	1003.9MB &	&	4.3GB	&	315.9	&	338.7MB	&	242.8	& &	363.5	\\	\hline
WikiTalk	&	-	&  &	481.1MB	&	2.5	&	446.9MB	&	-	&	& 41.2	\\	\hline
Orkut	&	8.2GB	&  &	13.2GB	&	749.3	&	312.0MB	&	773.2	&	& 1431.6	\\	\hline
LiveJournal	&	2.3GB	&  &	17.2GB	&	621.7	&	443.0MB	&	707.3	&	& 693.3	\\	\hline

\end{tabular}
}
\vspace{-2.0ex}
\caption{{\small Preprocessing Cost on Random Query \textcolor{red}{please update HN} }}
\label{tab:precomp}
\vspace*{-1.0ex}
\end{table*}



\comment{

\begin{figure*}[!htbp]
\resizebox{7.5in}{!} {
   \hspace{0.02cm}
   \begin{minipage}[c]{3.8in}
    {\scriptsize
    \begin{tabular}{|l|r|r|r|r|r|r|r|}
    \hline
    \multirow{2}{*}{Dataset}&  \multicolumn{ 4}{c|}{Indexing Cost } & \multicolumn{2}{c|}{Preproc.Time(min)} \\
    \cline{2-7}
    &
     \multicolumn{1}{c|}{Sketch-path} & \multicolumn{1}{c|}{HL-total}
    & \multicolumn{1}{c|}{{\small avg.$|L_H(v)|$}} & \multicolumn{1}{c|}{Hub$^2$} &
    \multicolumn{1}{c|}{Sketch} & \multicolumn{1}{c|}{HL} \\ \hline

Facebook	&	10.2MB	&	955.2MB	&	8.2	&	953.0MB	&	3.2	&	1.4	\\	\hline
Slashdot	&	26.1MB	&	496.3MB	&	11.1	&	491.4MB	&	6.5	&	4.3	\\	\hline
BerkStan	&	193MB	&	291.3MB	&	21.6	&	206.5MB	&	64.3	&	1.7	\\	\hline
Youtube	&	217.2MB	&	756.5MB	&	38.9	&	503.1MB	&	100.8	&	66	\\	\hline
As-skitter	&	391.3MB	&	1.2GB	&	101.9	&	268.3MB	&	109.9	&	31.7	\\	\hline
Flickr	&	626.7MB	&	1.5GB	&	232	&	344.5MB	&	163.8	&	202.5	\\	\hline
Flickr-growth	&	1003.9MB	&	4.3GB	&	315.9	&	338.7MB	&	242.8	&	363.5	\\	\hline
WikiTalk	&	-	&	481.1MB	&	2.5	&	446.9MB	&	-	&	41.2	\\	\hline
Orkut	&	8.2GB	&	13.2GB	&	749.3	&	312.0MB	&	773.2	&	1431.6	\\	\hline
LiveJournal	&	2.3GB	&	17.2GB	&	621.7	&	443.0MB	&	707.3	&	693.3	\\	\hline


    \end{tabular}
    }
    %\vspace*{-0.1cm}
    \label{tab:precomp}
    \captionof{table}{Preprocessing Cost on Random Query}
   \end{minipage}

   \hspace{-0.1cm}
   \begin{minipage}[c]{3.6in}
   \centering
   \psfig{figure=Figures/landmarksize_precomptime_part_results.eps,height=1.8in,width=3.6in}
   \vspace*{-3.0ex}
   \captionof{figure}{{\small Preprocessing Time (sec.) on Diff. Sizes of Hub-Set}}
   \label{fig:sizevarprecomptime}
   \end{minipage}
   \hspace{0.02cm}
}
\end{figure*}


\begin{figure*}[!htbp]
\resizebox{7.5in}{!} {
   \hspace{0.02cm}
   \begin{minipage}[c]{3.5in}
    {\scriptsize
    \begin{tabular}{|l|r|r|r|r|r|r|r|}
    \hline
    Dataset &  BFS  & BiBFS & HL-5K  & HL-8K & HL-10K & HL-12K & HL-15K \\ \hline

Facebook	&	0.76	&	0.03	&	0.002 	&	0.003 	&	0.003 	&	0.004 	&	0.015 	\\	\hline
Slashdot	&	2.04	&	0.05	&	0.005 	&	0.004 	&	0.004 	&	0.005 	&	0.024 	\\	\hline
BerkStan	&	0.66	&	0.1	&	0.014 	&	0.009 	&	0.009 	&	0.005 	&	0.005 	\\	\hline
Youtube	&	52.64	&	0.37	&	0.058 	&	0.016 	&	0.017 	&	0.020 	&	0.016 	\\	\hline
As-skitter	&	17.62	&	0.29	&	0.078 	&	0.044 	&	0.037 	&	0.025 	&	0.023 	\\	\hline
Flickr	&	187.3	&	1.45	&	0.342 	&	0.307 	&	0.338 	&	0.174 	&	0.161 	\\	\hline
Flickr-growth	&	249.27	&	0.95	&	0.338 	&	0.312 	&	0.191 	&	0.270 	&	0.245 	\\	\hline
WikiTalk	&	40.41	&	0.34	&	0.002 	&	0.002 	&	0.003 	&	0.001 	&	0.001 	\\	\hline
Orkut	&	862.39	&	16.89	&	1.091 	&	1.314 	&	1.438 	&	1.458 	&	2.190 	\\	\hline
LiveJournal	&	586.95	&	2.93	&	0.524 	&	0.618 	&	0.686 	&	0.741 	&	2.318 	\\	\hline





   \end{tabular}
    }
    %\vspace*{-0.1cm}
    \label{tab:sizevarquerytime}
    \captionof{table}{{\small Avg. Query Time (ms) of Rand. Queries using Diff. Sizes of Hub-Set}}
   \end{minipage}

   \hspace{-0.25cm}
   \begin{minipage}[c]{4in}
   \centering
   \psfig{figure=Figures/landmarksize_indexsize_part_results.eps,height=1.9in,width=3.8in}
   \vspace*{-3.0ex}
   \captionof{figure}{{\small Avg. \#core-hubs for Each Vertex using Diff. Sizes of Hub-set}}
   \label{fig:sizevarindex}
   \end{minipage}
   \hspace{0.02cm}
}
\end{figure*}

}











%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\comment{
\begin{figure*}[!htbp]
\resizebox{7.5in}{!} {
   \hspace{0.02cm}
   \begin{minipage}[c]{4in}
    {\scriptsize
    \begin{tabular}{|l|r|r|r|r|r|r|r|}
    \hline
    \multirow{2}{*}{Dataset}&  \multicolumn{ 5}{c|}{Indexing Cost (MB)} & \multicolumn{2}{c|}{Preproc.Time(min)} \\
    \cline{2-8}
    &
    \multicolumn{1}{c|}{Sketch-db} & \multicolumn{1}{c|}{Sketch-path}
    & \multicolumn{1}{c|}{CL-index} & \multicolumn{1}{c|}{CL-path} & \multicolumn{1}{c|}{CL-total} &
    \multicolumn{1}{c|}{Sketch} & \multicolumn{1}{c|}{CL} \\ \hline

    Facebook    &   10.2    &   107.2   &   20.5    &   1174.2  &   1194.7  &   3.2 &   1.4 \\  \hline
    Slashdot    &   26.1    &   171.6   &   38.5    &   491.4   &   529.9   &   6.5 &   4.3 \\  \hline
    BerkStan    &   193 &   2035    &   386.4   &   217.4   &   603.8   &   64.3    &   1.7 \\  \hline
    Youtube &   217.2   &   2575.6  &   656.8   &   503.1   &   1159.9  &   100.8   &   66  \\  \hline
    As-skitter  &   391.3   &   2897.5  &   965 &   268.3   &   1233.3  &   109.9   &   31.7    \\  \hline
    Flickr  &   626.7   &   4641.2  &   1059.3  &   344.5   &   1403.7  &   163.8   &   202.5   \\  \hline
    Flickr-growth    &   1003.9  &   6608.3  &   1312    &   338.7   &   1650.7  &   242.8   &   363.5   \\  \hline
    WikiTalk    &   -   &   -   &   1364.4  &   446.9   &   1811.2  &   -   &   41.2    \\  \hline
    Orkut   &   6608.3  &   8363.6  &   13173.3 &   312 &   13485.4 &   773.2   &   1431.6  \\  \hline
    cit-Patents &   793.2   &   2897.5  &   2154.2  &   2.6 &   2156.8  &   115.9   &   1   \\  \hline
    LiveJournal   &   2289.4  &   19074.8 &   17244.3 &   443 &   17687.3 &   707.3   &   693.3   \\  \hline
    topology &   6608.3  &   30554   &   9769.7  &   274 &   10043.8 &   1494.4  &   1322.6  \\  \hline

    \end{tabular}
    }
    %\vspace*{-0.1cm}
    \label{tab:precomp}
    \captionof{table}{Preprocessing Cost on Random Query}
   \end{minipage}

   \hspace{-0.05cm}
   \begin{minipage}[c]{4in}
   \centering
   \psfig{figure=Figures/landmarksize_precomptime_results1.eps,height=1.8in,width=4in} %scale=0.65
   \vspace*{-3.0ex}
   \captionof{figure}{{\small Preprocessing time (min.) on different landmark size}}
   \label{fig:sizevarprecomptime}
   \end{minipage}
   \hspace{0.02cm}
}
\end{figure*}


    Facebook    &   0.76    &   0.03    &   0.0022  &   0.0007  &   0.0005  &   0.0005  &   0.0148  \\  \hline
    Slashdot    &   2.04    &   0.05    &   0.0045  &   0.0011  &   0.0006  &   0.0005  &   0.0242  \\  \hline
    BerkStan    &   0.66    &   0.1 &   0.0138  &   0.0094  &   0.0071  &   0.0052  &   0.0048  \\  \hline
    Youtube &   52.64   &   0.37    &   0.0583  &   0.0157  &   0.0277  &   0.0196  &   0.0161  \\  \hline
    As-skitter  &   17.62   &   0.29    &   0.0784  &   0.0442  &   0.0348  &   0.0254  &   0.0226  \\  \hline
    Flickr  &   187.3   &   0.74    &   0.2317  &   0.2063  &   0.1844  &   0.1738  &   0.1609  \\  \hline
    Flickr-growth    &   249.27  &   0.95    &   0.3384  &   0.3116  &   0.2755  &   0.2697  &   0.2447  \\  \hline
    WikiTalk    &   40.41   &   0.17    &   0.0018  &   0.0009  &   0.0007  &   0.0007  &   0.0006  \\  \hline
    Orkut   &   862.39  &   16.89   &   1.0911  &   1.3141  &   1.4383  &   1.4582  &   2.1896  \\  \hline
%    cit-Patents &   0.19    &   0.11    &   0.0838  &   0.0814  &   0.0875  &   0.0787  &   0.0832  \\  \hline
    LiveJournal &   586.95  &   2.93    &   0.5236  &   0.6177  &   0.6863  &   0.7413  &   2.3184  \\  \hline
%    topology &   1490.63 &   8.44    &   0.5782  &   0.5003  &   0.4095  &   0.4189  &   0.3814  \\  \hline



}


==> Figures/query.tex <==
\begin{algorithm}[!htp]
	\caption{Hierarchical Query}
	\label{query}

	\begin{algorithmic}[1]
		\REQUIRE $G=(V,E),K,H,G=(V^*,E^*),s,t$
		\STATE $Q_f^R \leftarrow \{s\}$; $Q_f^H \leftarrow \emptyset$; $level_f(s) = 0$;
		\STATE $Q_b^R \leftarrow \{t\}$; $Q_b^H \leftarrow \emptyset$; $level_b(t) = 0$;
		\STATE $dist \leftarrow K$; $current\_level \leftarrow 0$; $forward \leftarrow true$;
		\WHILE{either $Q_f^R, Q_f^H, Q_b^R, Q_b^H$ is non-empty}
			\IF{$forward = true$}
				\STATE $forwardSearch()$;
				\STATE $forward \leftarrow false$;
			\ELSE
				\STATE $backwardSearch()$;
				\STATE $forward \leftarrow true$;
				\STATE $current\_level \leftarrow current\_level + 1$;
			\ENDIF
			%\STATE \COMMENT{The distance to hub nodes are always correct,
				%so once the two directions meet inside the extracted subgraph, no further expand inside the subgraph is needed}
			%\STATE \COMMENT{But the distance to regular nodes might be incorrect, so we need to compare the lower bound of those paths against the current result}
			\IF{$subgraph\_met \land
				level\_b[Q_f^R.\mathrm{top}()] >= dist - d(s,H) -1 \land
				level\_f[Q_b^R.\mathrm{top}()] >= dist - d(H,t) - 1$}
				\STATE break;
			\ENDIF
		\ENDWHILE
	\end{algorithmic}
\end{algorithm}


\begin{algorithm}[!htp]
	\caption{Forward Search for Hierarchical Query}
	\label{query_forward}

	\begin{algorithmic}[1]
		\IF{$\lnot subgraph\_met$}
			\WHILE{$Q_f^H \neq \emptyset \land level_f(Q_f^H.\mathrm{top}()) = current\_level$}
				\STATE $u \leftarrow Q_f^H.\mathrm{pop}()$;
				%\STATE \COMMENT{The expand is constrained inside the subgraph}
				\FORALL{$v \in neighbour(u) \cap V^*$}
					\IF{$v$ has not been visited}
						\IF{$v$ is reached in the other direction}
							\STATE $dist = \min(dist, d(s,v) + d(v,t))$;
							\STATE $subgraph\_met \leftarrow true$;
							\STATE break while;
						\ENDIF
						\STATE $Q_f^H.\mathrm{push}(v)$;
						\STATE $level_f(v) \leftarrow level_f(u) + 1$;
					\ENDIF
				\ENDFOR
			\ENDWHILE
		\ENDIF
		\WHILE{$Q_f^R \neq \emptyset \land level(Q_f^R.top()) = current\_level$}
			\STATE $u = Q_f^R.\mathrm{pop}()$;
			\FORALL{$v \in neighbours$}
				\IF{$v$ has not been visited}
					\IF{$v$ is reached in the other direction}
						\STATE $dist = \min(dist, d(s,v) + d(v,t))$
					\ENDIF
					\STATE append $v$ to either $Q_f^R$ or $Q_f^H$;
					\STATE $level_f(v) \leftarrow level_f(u) + 1$;
				\ENDIF
			\ENDFOR
		\ENDWHILE
	\end{algorithmic}
\end{algorithm}


==> HubLabeling.tex <==
\section{Indexing  Approach for Hub$^{\textstyle 2}$-Labeling}
\label{hubsetselectionandlabeling}

In this section, we will discuss how to construct the hub-set $\mathcal{H}$ (Subsection~\ref{hubsetselection}), and how to compute the core-hub labeling $L_H$ for each vertex $v$ efficiently (Subsection~\ref{indexingalgo}). 

\subsection{Hub-Set Construction}
\label{hubsetselection}

The vertices in hub-set have similar functionality to the landmarks, which aim to maximally {\em cover} the shortest paths in the graph. 
Intuitively, a  shortest path is covered by the hub-set if it consists of at least one vertex in the hub-set. 
Formally, we define the goodness of a hub-set using the {\em coverage} criterion: 

\bdefin{\bf (Hub-Set Coverage)}
Given a hub-set $\mathcal{H}$ and vertex pair $(s,t)$, if the estimated shortest distance using hub-set indexing scheme is {\em exact} distance (i.e., $d(s,t)=$ \\ $min_{x \in L_{H}(s) \wedge y \in L_{H}(t)} (d(s,x)+d(x,y)+d(y,t))$),
we say vertex pair $(s,t)$ is covered by hub-set $\mathcal{H}$.
Let $C(\mathcal{H})$ be the number of (unique) vertex pairs covered by the hub-set $\mathcal{H}$. 
\edefin

Given this,  we are interested in maximally covering the shortest path distance using a limited number of vertices in the hub-set (in order to hold the distance matrix Hub$^2$). 
This can be formally described as follows: 

\bdefin{\bf (Optimal Hub-Set Selection Problem)}
Given graph $G=(V,E)$ and parameter $K$, we would like to find $\mathcal{H} \in V$,
such that $|\mathcal{H}|=K$ and the number of vertex pairs $(s,t) \in V \times V$ covered by $L$ is maximized ($\max{C(\mathcal{H})}$).
\edefin

Unfortunately, this problem is NP-hard. 
\bthm
The  optimal hub-set selection problem is NP-hard and it is also equivalent to the $k$-landmark-cover problem~\cite{Potamias09}. 
\ethm

The proof is in the appendix. 
Given this, we consider how to heuristically select vertices in the hub-set. It is quite similar to the landmark selection though here we focus on the coverage criterion on the social network. 
Let us start from the most simple scenario to gain a better intuition of good hub-set in social networks.
Intuitively, the best hub-set vertices should be the one in the very {\em central} position of graph since they tend to cover a large number of shortest paths~\cite{Potamias09}.
This high-level understanding suggests two concepts of {\em central} vertex from different perspectives:
1) it is a vertex lying on many shortest paths, which can be measured by vertex betweenness centrality;
2) it is a vertex close to other vertices in the graph, which can be measured by closeness centrality.
In the optimized scenario, the best {\em central} vertex based on first concept is referred to as the vertex with largest vertex betweenness~\cite{citeulike:1025135},
while second one refers to the vertex with optimal closeness centrality.
We generalize both concepts to hub-set selections in social networks.

\noindent{\bf Vertex Betweenness Criterion: }
The vertex betweenness firstly introduced by Freeman~\cite{citeulike:1025135} in the context of social science:
\[  C_B(v) = \sum_{u,w \in V \wedge u\neq w \neq v} \frac{\sigma_{uw}(v)}{\sigma_{uw}} \]
where $\sigma_{uw}(v)$ is the total number of shortest paths between $u$ and $w$ that pass through $v$,
and $\sigma_{uw}$ is the total number of shortest paths between $u$ and $w$.

We sort all vertices based on their vertex betweenness centrality in descending order and pick top $K$ vertices as hub-set.
To achieve this goal, we need to precompute vertex betweenness centrality for every vertex.
However, the fastest (exact) algorithm to compute every vertex betweenness centrality is $O(|V||E|)$~\cite{Brandes2001}, which is still rather expensive for massive networks. 

\noindent{\bf Closeness Betweenness Criterion: }
The closeness of a vertex is evaluated by the inverse of its total distance to all other vertices in the graph~\cite{citeulike:7062391}.
The vertex is the more central the lower its total distance to the remaining vertices. That is,
\[ C_C(v) = \frac{|V|-1}{ \sum_{u \in V \wedge u \neq v} d(v,u) }  \]

The intuition of using this criterion is that, a vertex closer to all other vertices are very likely to be part of many shortest paths.
Therefore, we select top $K$ vertices with largest closeness centrality to be hub-set.
Similar to computing vertex betweenness, calculating closeness betweenness involving pairwise shortest paths computation is an expensive task,
taking $O(|V|(|V|+|E|))$ time in unweighted graph setting.

\noindent{\bf Hub-Set=\{Hub\}:} 
Although it is costly to select $K$ hub-set vertices strictly following aforementioned criteria, 
we are able to adopt {\em the vertices with high vertex degree}, i.e., the {\em hubs}, as their effective proxies in social networks.
This is based on key observations on how high-degree vertices (hubs) contribute social networks' connectivity and small path length. 
The empirical study on several well-known social networks (i.e., Flickr, LiveJournal, Orkut and Youtube) reported in~\cite{Mislove07}
clearly demonstrates the presence of densely connected {\em core} comprising of a small portion of vertices with highest degree.
The removal of this {\em core} dramatically disconnects entire graph, implying that most of pairwise connections rely on few high-degree vertices (hubs).
In other words, few high degree vertices serve as key intermediates in most of shortest paths, thus are qualified to be the hub-set vertices under vertex betweenness criterion.
In addition, this study ~\cite{Mislove07} also analyzes the average shortest path length in the core containing only highest-degree vertices. 
As core grows, the average shortest path length increases sub-logarithmically.
Since average shortest path length of entire graph is very small, this phenomenon suggests that the lower degree vertices that constitute the majority of the network are very close to the high degree vertices in the core.
In this sense, high-degree vertices (hubs) are also qualified under the closeness betweenness criterion.

To sum, we simply select the top $K$ high-degree vertices (hubs) in the original graph $G$ as the hub-set ($\mathcal{H}$) (That is also the reason why we refer to $\mathcal{H}$ as the hub-set). 
In addition, we note that another advantage of using the hubs in the hub-set is to reduce the search space. 
Recall that in the bidirectional search (the query processing step), any vertices in the hub-set do not need to be expanded. 
In this way, we can effectively avoid those high-degree vertices (hubs), which form the very reason for search space explosion. 
Finally, in the rest of the paper, we will also use  the hub-set vertices and the hubs exchangeably. 


\subsection{Core-Hub Labeling}
\label{indexingalgo}

In this subsection, we present an efficient algorithm to assign each vertex $u$ its core hubs $L_{H}(u)$.  
The goal of $6$-degree shortest path is to compute the shortest path with length no greater than $6$ (or $k$ in general).
Given this, it is easy to see that {\em for any hub $h$ in $\mathcal{H}$ to be assigned to $L_H(u)$, their distance has to be no greater than $6$ ($d(h,u) \leq 6$). }
This is because for any vertex pair $(s,t)$, the estimation using the hub-set is to provide an upper-bound  for the bidirectional search, which is also constrained by $6$. 
Thus, if the upper-bound is greater than $6$, it becomes useless.


Now, let us consider the straightforward approach based on the core-hub definition (Definition~\ref{corehubdef}) for labeling.
In this case, we need  first precompute all pairwise distances among hubs and materialize all distances between hubs and other vertices if they are no greater than $6$. 
Since the size of hub-set $\mathcal{H}$ is quite large, the materialization cost of $|V||\mathcal{H}|$ is too high. 

Here, we introduce an efficient procedure which only performs one local breadth-first traversal (BFS) for each hub in $\mathcal{H}$ to visit its $6$-degree neighbors(i.e., the vertices with distance to the hub no more than $6$) and no additional distance-matrix materialization is needed. 
In addition, this procedure also construct the distance matrix Hub$^2$ during the labeling process. 
Given this, for each BFS starting from a hub $h \in \mathcal{H}$, two tasks need to be performed: 
1) it needs to find out all other hubs whose distance to $u$ is no more than $6$, and record one shortest path between them (distance matrix construction);
2) for each visited non-hub vertex $v$ during BFS, we need to quickly check whether $h$ is $v$'s core hub, i.e., whether $u \in L_H(v)$.
This is equivalent to determine whether there is other hubs appearing in a shortest path between $u$ and $v$.
The first task can be easily achieved by introducing an extra integer for each vertex, which is used to record the previous vertex on the shortest path from hub $h$ to current vertex along shortest path.
The first task is relatively straightforward as a basic BFS process can easily accomplish that. 
The second task is non-trivial and is the main focus.

To quickly determine whether $h \in L_H(v)$ during the BFS process, we utilize the following observation:
{\em Let vertex $y$ lies on a shortest path from hub $h$ to non-hub vertex $v$ with distance $d(h,v)-1$ (i.e., $y$ is one hop closer than $v$ with respect to $h$). 
If there is a hub $h^\prime$ appearing in a shortest path from $h$ to $y$ ($h^\prime$ and $y$ may not be distinct),
$h^\prime$ definitely lies on a shortest path from $h$ to $v$ and $h$ cannot be core hub of $v$.}
Based on this observation, we simply maintain a binary flag $b(v)$ to denote whether there is another hub appearing in a shortest path between $h$ and $v$.
Specifically, its update rule is as follows: $b(v)=1$ if $v$ itself is hub or $b(y)=1$ where $d(h,y)=d(h,v)-1$ and $d(y,v)=1$.
Thus, during BFS traversal, when we visit vertex $v$, if its flag $b(v) \neq 1$ meaning there is no other hubs lying on the shortest path between $h$ and $v$, we add $h$ and the corresponding shortest path $SP(h,v)$ to its $L_{H}(v)$.

\begin{example}
Figure~\ref{fig:bfsindexexample} shows an example of core-hub labeling. 
The value attached to each vertex $v$ is its binary flag $b(v)$, such as $b(1)=0$ and $b(2)=1$.
As we know, BFS process visits vertices in levelwise manner with the help of queue. 
We start from hub $h$ to visit its neighbors $1$, $2$ and $3$ in level $1$ and push them ino queue.
When vertex $2$ is popped from queue, its binary flag $b(2)$ is set to be $1$ since it belongs to hub-set.
Afterward, the flags of its immediate neighbors in level $2$ (i.e., vertices $5$ and $7$) are all set to be $1$,
because their neighbor $2$ in level $1$ is hub and lies on shortest paths from hub $h$ to them.
Therefore, hub $h$ cannot be core-hub of $5$ and $7$.
However, the flag of vertex $6$ is $0$ since flags of all its immediate neighbors in level $1$ are $0$,
meaning no hub lying on shortest paths from $h$ to $6$,
thus $h \in L_H(6)$.
%In this sense, binary flag is used to efficiently check whether $h$ is its 6-neighborhood's core-hub. 
\end{example}


\begin{figure}
\centering
\begin{tabular}{c}
\psfig{figure=Figures/bfsindexexample.eps,scale=0.65}
\end {tabular}
\caption{Example for Core-hub Labeling (only consider 3 hops)}
\label{fig:bfsindexexample}
\end{figure}


\input{Figures/BFSIndexing.tex}

The outline of BFS-based procedure for generating core-hubs indices is described in Algorithm~\ref{alg:bfsindex}.
The flag $b(v)$ for each vertex $v$ is updated when $v$ is hub or the flag of its previous vertex in $SP(h,v)$ is one (Line 6 and Line 18).
When vertex $u$ is popped from queue and its flag $b(u)=0$, hub $s$ is assigned to $L_{H}(u)$ (Line 10).
This procedure will be invoked for each hub.
In total, this procedure takes $O(\sum_{h \in \mathcal{H}} (|N_6(h)|+|E_6(h)|))$ time, where $L$ is hub-set, $N_6(h)$ ($E_6(h)$) is the number of vertices (edges) in $u$'s 6-degree neighborhood.

































%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Given a vertex pair $(s,t)$, if their $L^c_{out}(s)$ and $L^c_{in}(t)$ are able to recover the {\em exact} shortest path,
%this shortest path also can be recovered by using traditional indices $L_{out}(s)$ and $L_{in}(t)$,
%because $L^c_{out}(s) \subseteq L_{out}(s)=Succ(s|L)$ and $L^c_{in}(t) \subseteq L_{in}(t)=Pred(t|L)$.
%Essentially, core landmark indexing is the generalization of traditional landmark indexing,
%because it can not only utilize single landmarks, but also a pair of landmarks to estimate shortest path.

\comment{
\section{Local Landmark Framework}
\label{landmark}

In this section, we describe a new indexing scheme using landmarks to effectively encode the shortest path information.
Given a landmark set, new indexing scheme not only provides much compact indices, but also guarantees the resulting shortest path no long than the one by traditional landmark approach.
We formally define the optimal landmark selection problem based on new indexing scheme.
Then, we show that this problem is NP-hard and propose a greedy solution based on set-cover-with-pair framework to achieve logarithmic approximation.


To facilitate our discussion, we begin with defining some nation and terminology used in the rest of paper.
Let $G=(V,E)$ be an unweighted graph where $V=\{1,2,...n\}$ is the vertex set and $E \subseteq V \times V$ is edge set.
The edge from vertex $u$ and $v$ is denoted by $(u,v)$, and we use $P(v_0, v_p) = (v_0, v_1, ..., v_p)$ to denote a simple path from $v_0$ to $v_p$.
The length of a simple path in unweighted graph is the number of edges in the path.
Given two vertices $u$ and $v$, their shortest path $SP(u,v)$ is the path between them with minimal length.
The distance from vertex $u$ to $v$ is the length of shortest path $SP(u,v)$ from $u$ to $v$, denoted by $d(u,v)$.
For each vertex $u$, its $\epsilon$-neighbors, denoted as $N_{\epsilon}(u)$ is a set of vertices such that their distance to $u$ is no greater than $\epsilon$, i.e., $N_{\epsilon}(u) = \{v \in V | 0 < d(u,v) \le \epsilon\}$.
Given a vertex set $V^\ast$, for each each vertex $u \notin V^\ast$,
$Succ(u|V^\ast)$ is a subset of $V^\ast$ which can be reached from $u$ and $Pred(u|V^\ast)$ is a subset of $V^\ast$ which can reach $u$.
Due to the popularity of directed graphs in social networks, we focus on the undirected and unweighted graphs in the paper.
Taking a undirected graph as a bidirected graph, all techniques discussed in the paper can be easily extended to undirected setting.


\subsection{Global Landmark Indexing}
\label{globalindex}

Given graph $G=(V,E)$, suppose a subset of ordered vertices $V^\ast=\{x_1,x_2,...,x_k\} \subseteq V$ has been selected to be {\em landmarks}.
For each landmark $x_i$, we need to precompute and explicitly store the shortest path to all vertices in the graph $G$.
Then, we distribute these shortest path information to every vertex, such that each vertex $u$ is associated with two vectors:
{\small
\beqnarr
L_{in}(u)  = (<x_1: d(x_1,u),SP(x_1,u)>...,<x_p: d(x_p,u),SP(x_p,u)>)  \nonumber \\
L_{out}(u) = (<y_1: d(u,y_1),SP(u,y_1)>...,<y_q: d(u,y_q),SP(u,y_q)>) \nonumber
\eeqnarr
}
where $x_i \in Pred(u|V^\ast)$ ($1 \le i \le p$) and $y_j \in Succ(u|V^\ast)$ ($1 \le j \le q$).
Since all landmark information are propagated to entire graph, we refer to this traditional indexing scheme as {\em Global Landmark Indexing} scheme.
Given this, for a pair of vertices $s$ and $t$, their {\em landmark distance $d(s,t|V^\ast)$} and {\em landmark shortest path $SP(s,t|V^\ast)$} are defined based on triangle inequality:
{\small
\beqnarr
d(s,t|V^\ast) = min_{x \in L_{out}(s) \cap L_{in}(t)} \{ d(s,x)+d(x,t) \} \nonumber \\
SP(s,t|V^\ast) = SP(s,x^\ast) \circ SP(x^\ast,t) \nonumber \\
 \text{ where } x^\ast = \underset{x \in L_{out}(s) \cap L_{in}(t)}{\operatorname{argmin}} d(s,x)+d(x,t) \nonumber
\eeqnarr
}
where $\circ$ is the concatenation operator for two paths by connecting the first path's ending node and second path's starting node.
Clearly, given landmark set $V^\ast$, the landmark index size of total graph is $\sum_{u \in V} |L_{out}(u)|+|L_{in}(u)| = \sum_{u \in V} |Pred(u|V^\ast)| + |Succ(u|V^\ast)|$.

When landmark distance is equivalent to distance in the graph $G$, the landmark shortest path is actually the exact shortest path for a pair of vertices.
We say a set of vertices are {\em exact landmarks} if the landmark distance of any pair of vertices is exact distance in the graph $G$.
Simply speaking, for any two reachable vertices, there always exists one vertex from {\em exact landmarks} appearing in one of the shortest paths between them.
The problem of discovering exact landmarks with smallest cardinality has been proved to be NP-hard~\cite{Potamias:2009:FSP:1645953.1646063}.
Due to the hardness of selecting exact landmarks, most of existing works concentrate on developing different heuristics utilizing certain graph properties, such as vertex centrality, degree distribution or graph diameter.
Few of them attempt to improve the accuracy from indexing perspective.


\begin{figure}
\centering
\begin{tabular}{c}
\psfig{figure=Figures/indexexample.eps,scale=0.6}
\end {tabular}
\caption {Indexing Example}
\label{fig:indexexample}
\end{figure}

\begin{figure}
\centering
\begin{tabular}{c}
\psfig{figure=Figures/proofcases.eps,scale=0.65}
\end {tabular}
\caption {Cases in proof of Lemma~\ref{localgoodpath}}
\label{fig:proofcases}
\end{figure}



\subsection{Local Landmark Indexing}
\label{localindex}

In global landmark indexing scheme, each vertex is required to explicitly record all shortest distance and shortest path to (from) the landmarks which is reachable (can be reached).
However, we observe that many landmarks are redundant for each specific vertex under certain condition.
More specifically, each vertex only needs to record a subset of {\em essential} landmarks such that on other landmarks appear in the shortest path between them.
Using a slightly modified shortest path computation strategy, the recorded landmarks guarantee to generate a path which is no longer than the one produced by global indexing scheme.
Before we formally introduce new indexing scheme, let us go over a simple example to gain intuitive understanding.

\begin{example}
\label{indexexamp}
Figure~\ref{fig:indexexample} shows a shortest path from $s$ to $t$ while three landmarks $v_1$, $v_2$ and $v_3$ lie in this shortest path.
In global landmark indexing, both outgoing indices of source $s$ and incoming indices of destination $t$ need to record all three landmarks.
If shortest path $SP(v_1,v_3)$ between two landmarks $v_1$ and $v_3$ is known beforehand,
landmark $v_1$ included in $L_{out}(s)$ and landmark $v_3$ included in $L_{in}(t)$ are sufficient to recover the shortest path $SP(s,t)$,
i.e., $SP(s,t)= SP(s,v_1) \circ SP(v_1,v_3) \circ SP(v_3,t)$.
We can see that, the shortest path $SP(v_1,v_3)$ between two landmarks are implicitly recorded twice in $SP(s,v_3)$ and $SP(v_1,t)$,
thus materializing $SP(v_1,v_3)$ does not introduce any extra index cost.
\end{example}

In the example, we actually represent the shortest path $SP(s,t)$ by three segments:
1) $SP(s,v_1)$, from source $s$ to one close landmark $v_1$; 2) $SP(v_1,v_3)$, from landmark $v_1$ to another landmark $v_3$ close to destination $t$;
and 3) $SP(v_3,t)$, from landmark $v_3$ to destination $t$.
To some extent, two intermediate landmarks in the shortest path mimic the highway entrances or exits of transportation network.
In order to find the shortest path from starting point to destination, one simply find the shortest path from starting to the appropriate entrance of highway,
and then get off the correct exit of highway which leads to the remaining shortest path to the destination.
The shortest paths among landmarks serve as {\em shortest path oracle} which can answer the shortest path queries quickly, such as in constant time.

Now, given a landmark set $V^\ast$, we formally define {\em incoming essential landmarks} and {\em outgoing essential landmarks} for each vertex $u$:

\bdefin{\bf (Essential Landmarks)}
Given graph $G=(V,E)$ and a landmark set $V^\ast$, for each vertex $u$, its outgoing essential landmarks $L^e_{out}(u)$ contains landmark $x$,
if there does not exist $x^\prime \in V^\ast$ satisfying $d(u,x)=d(u,x^\prime)+d(x^\prime,x)$.
Simply speaking, no other landmarks appear in one of shortest path from $u$ to $x$.
Similarly, its incoming essential landmarks $L^e_{in}(u)$ contains landmark $y$,
if there is no $y^\prime \in V^\ast$ satisfying $d(y,u)=d(y,y^\prime)+d(y^\prime,u)$.
\edefin

The exclusion of a landmark $x$ in the essential landmarks with respect to vertex $u$ means there exists other landmark appear in the shortest path $SP(u,x)$ and closer to $u$ than $x$.
Recalling example~\ref{indexexamp}, $v_3$ is non-essential for source $s$, since the shortest path from $s$ to $v_3$ can be ``blocked'' by $v_1$.
The {\em incoming essential landmarks} and {\em outgoing essential landmarks} of each vertex constitute the indices of new landmark indexing scheme.
Opposing to global landmark indexing which needs to store all reachable (can be reached) landmarks, we refer to this indexing scheme as {\em local landmark indexing}.
Based on local indexing, we are able to compute its corresponding {\em landmark distance $d^e(s,t|V^\ast)$} and {\em landmark shortest path $SP^e(s,t|V^\ast)$} are defined as:
\beqnarr
d^e(s,t|V^\ast) = min_{x \in L^e_{out}(s) \wedge y \in L^e_{in}(t)} \{ d(s,x)+d(x,y)+d(y,t) \} \nonumber \\
SP^e(s,t|V^\ast) = SP(s,x^\ast) \circ SP(x^\ast,y^\ast) \circ SP(y^\ast,t) \nonumber \\
\text{ where } x^\ast = \underset{x \in L^e_{out}(s) \wedge y \in L^e_{in}(t)}{\operatorname{argmin}} d(s,x)+d(x,y)+d(x,t) \nonumber
\eeqnarr
In this sense, we need to materialize the pairwise shortest path among landmarks.
However, this materialization does not impose burden on the memory cost due to two reasons.
First, the length of shortest path in the social networks we focus on in this work is typically rather small~\cite{Mislove07}.
In our experiments, we observe that the length of most shortest paths between landmarks is no more than 3.
Second, lots of shortest paths between landmarks are implicitly encoded multiple times in global landmark indexing (e.g., Figure~\ref{fig:indexexample}, $SP(v_1,v_3)$ is contained in $SP(s,v_3)$ and $SP(v_1,t)$).

In addition, it is not hard to see that, local landmark indexing is a generalization of global landmark indexing.
In other words, if there is no shortest path from non-landmark vertex to landmark (or from landmark to non-landmark vertex) is ``blocked'' by some landmarks,
local landmark indexing degrades to global landmark indexing.
Hence, the index size of local landmark indexing $\sum_{u \in V} (|L^e_{out}(u)| + |L^e_{in}(u)|)$ is no larger that of global indexing.
More importantly, we have following observation:

\blemma
\label{localgoodpath}
The shortest path generated by local landmark indexing is no longer than the best one generated by global landmark indexing.
\elemma

\bproof
We want to prove that, for any path generated by global landmark indexing, we are able to find a path no longer that it based on local landmark indexing.
Without loss of generality, consider reachable vertex pair $(s,t)$, let us denote one path obtained by global landmark indexing as $SP(s,x) \circ SP(x,t)$,
where $x$ is the intermediate landmark in the path (i.e., $x \in L_{out}(s)$ and $x \in L_{in}(t)$.
Now, we try to find a path based on local landmark indexing which is not longer than $SP(s,x) \circ SP(x,t)$ in the following cases:
%we consider the outgoing indices $L^e_{out}(s)$ of source and incoming indices $L^e_{in}(t)$ of destination with respect to $x$ based on local landmark indexing:

\noindent 1) $x \in L^e_{out}(s)$ and $x \in L^e_{in}(t)$. It is trivial to generate the same path $P(s,x) \circ P(x,t)$.

\noindent 2) $x \in L^e_{out}(s)$ and $x \notin L^e_{in}(t)$. According to the definition of {\em essential landmarks}, there is some landmark $y \in L^e_{in}(t)$ appear in the shortest path from $x$ to $t$, i.e., $d(x,t)=d(x,y)+d(y,t)$ (case $2$ shown in Figure~\ref{fig:proofcases}).
Since the shortest path $SP(x,y)$ from landmark $x$ to $y$ is available beforehand, we are able to generate the path $SP(s,x) \circ SP(x,y) \circ SP(y,t)$ with the same length as $SP(s,x) \circ SP(x,t)$.

\noindent 3) $x \notin L^e_{out}(s)$ and $x \in L^e_{in}(t)$. Follow the similar logic in case 2 (case 3 in Figure~\ref{fig:proofcases}). We guarantee to have $y \in L^e_{out}(s)$ appear in $SP(s,x)$. Thus, we can generate path $SP(s,y) \circ SP(y,x) \circ SP(x,t)$ which is no longer than $SP(s,x) \circ SP(x,t)$.

\noindent 4) $x \notin L^e_{out}(s)$ and $x \notin L^e_{in}(t)$. That is, there are some other landmarks $y_1 \in L^e_{out}(s)$ and $y_2 \in L^e_{in}(t)$ appear in the shortest paths $SP(s,x)$ and $SP(x,t)$, respectively (case 4 shown in Figure~\ref{fig:proofcases}).
Moreover the shortest path $SP(y_1,y_2)$ between landmarks $y_1$ and $y_2$ are known.
Due to triangle inequality $d(y_1,y_2) \le d(y_1,x)+d(x,y_2)$, we are able to generate the shorter path $SP(s,y_1) \circ SP(y_1,y_2) \circ SP(y_2,t)$
compared to $SP(s,x) \circ SP(x,t)$.

Putting those together, in any case, we can find a path based on local landmark indexing no worse than the one generated by global landmark indexing.
Therefore, the statement follows.
\eproof

Local landmark indexing scheme not only provides much compact index size, but also guarantees the resulting shortest path no long than the one by global landmark indexing scheme.
On the other hand, due to the properties of social networks, such as small diameter and massive size,
the desired landmarks should be able to provide exact shortest path using compact index size.
Motivated by this requirement, we formally define the concept of landmark coverage and following exact landmark discovery problem:

\bdefin{\bf (Landmark Coverage)}
Given graph $G=(V,E)$ and landmark set $V^\ast \subseteq V$, for a vertex pair $(s,t)$,
we say $V^\ast$ {\em covers} vertex pair $(s,t)$ if there exists two landmarks $x,y \in V^\ast$ appearing in the shortest path from $s$ to $t$.
Note that, two landmarks may not be distinct, i.e., $x$ may be the same with $y$.
\edefin

\bdefin{\bf (Exact Landmark Set Discovery Problem)}
Given an unweighted and directed graph $G=(V,E)$, the exact landmark set discovery problem tries to find a set of landmarks $V^\ast \in V$
which can cover any pair of reachable vertices and the local landmark index size is minimized.
\edefin

\comment{
\bdefin{\bf (Exact Landmark Set Discovery Problem)}
Given an unweighted and directed graph $G=(V,E)$, the exact landmark set discovery problem tries to find a set of landmarks $V^\ast \in V$,
such that for any pair of reachable vertices $(s,t)$, their corresponding local indices satisfy:
\[ d^e(s,t|V^\ast) = d(s,t) \]
where the local landmark index size is minimized.
\edefin
}


\subsection{Transform to Set-Cover-with-Pairs}
\label{scpsolution}

In this section, we transform the exact landmark set discovery problem to set-cover-with-pair instance.
To be self-contained, we first briefly introduce the set-cover-with-pair problem~\cite{HS05}.

\bdefin{\bf (Set-Cover-with-Pairs Problem ~\cite{HS05})}
Let $U$ be the ground set and let $S = \{1, \ldots, M\}$ be a set of objects, where each object $i\in S$ has a non-negative cost $w_i$.
For every $\{i,j\}\subseteq S$, let $\mathcal{C}(i, j)$ be the collection of elements in $U$ covered by the pair $\{i, j\}$.
The objective of the set cover with pairs (SCP) problem is to find a subset $S^\prime \subseteq S$ such that
$\mathcal{C}(S^\prime) =\bigcup_{\{i,j\}\subseteq S^\prime} \mathcal{C}(i, j) = U$ with a minimum covering cost $\sum_{i\in S} w_i$.
We refer to the special case in which each object has a unit weight ($w_i=1$) as the \textbf{cardinality SCP} problem.
\edefin

Now we transform our exact landmark set discovery problem to the Set-Cover-with-Pairs problem as follows.
Let the ground set $U=TC(G)$, i.e., it contains any vertex pair $(u,v)$ in $G$, such that $u \rightarrow v$.
To cover a pair $(u,v)$ means we can recover one of their shortest paths in the new landmark indexing scheme.

In our directed graph setting, we categorize objects in $Q$ into two types: starting objects $Q^s$ and ending objects $Q^e$ with respect to two endpoints of each shortest path.
Each starting object $O^s_{u,x_i}$ in $Q$ corresponds to a tuple $(u,(x_i: d_{x_i}, SP_{x_i}))$, where $u$ is a starting vertex and $x_i$ is a candidate landmark can be reached from $u$.
Note that, $d_{x_i}= d(u,x_i)$ and $SP_{x_i}=SP(u x_i)$ are shortest distance and one shortest path from $u$ to $x_i$, respectively.
Similarly, each ending object $O^e_{y_j,v}$ in $Q$ corresponds to a tuple $((y_j: d_{y_j}, SP_{y_j}),v)$, where $v$ is ending vertex and $y_j$ is a candidate landmark can reach $v$.
Here, $d_{y_j}= d(y_j,v)$ and $SP_{y_j}=SP(y_j, v)$ are shortest distance and one shortest path from $y_j$ to $v$, respectively.
Now, we define $\mathcal(O_{u,x_i}, O_{y_j,v})$ for each pair of objects $O_{u,x_i}$ and $O(y_j,v)$.
Given any four vertices $(u,x_i,y_j,v)$, if $d(u,x_i)+d(x_i,y_j)+d(y_j,v)=d(u,v)$, then vertex pair $(u,v)$ is covered by objects pair $\{O^s_{u,x_i}, O^e_{y_j,v}\}$.
That is, $\mathcal{C}(O^s_{u,x_i}, O^e_{y_j,v})$ contains vertex pair $(u,v)$.
Otherwise, $\mathcal{C}(O_{u,x}, O_{y,v})=\emptyset$.
Note that, aforementioned four vertices may not be distinct, i.e., $u$ may be the same with $x_i$, $x_i$ may be the same with $y_j$, etc.
%From the viewpoint of restoring shortest paths, that vertex pair $(u,v)$ is covered by objects pair $\{O^s_{u,x_i}, O^e_{y_j,v}\}$ means there exists one shortest path from $u$ to $v$ going through two landmarks $x_i \in L^\prime_{out}(u)$ and $y_j \in L^\prime_{in}(v)$.
%In this sense,
It is not hard to see that each $\mathcal{C}(O_{u,x_i}, O_{y_j,v})$ at most contains one vertex pair.


Further, we assign a unit cost to each object, i.e., $w(O_{u,x})=1$.
Then, if we can find a set of objects $Q^\prime \subseteq Q$ such that $\mathcal{C}(Q^\prime)$ covers the ground set,
we are able to recover all shortest path for any pair of reachable vertices in the graph.
Therefore, the union of landmark indices $\cup_{u\in V} (L^e_{out}(u) \cup L^e_{in}(u))$ is the exact landmarks with smallest local landmark index size.
By applying the best available algorithm for SCP proposed in~\cite{HS05}, we obtains a $O(\sqrt{N\log N})$ approximation ratio to exact landmark set discovery problem,
where $N$ is the cardinality of the ground set $N=|U|$, for the cardinality SCP problem.


However, in our problem setting, the ground set is $U=TC(G)$ and $N=|TC(G)|$, which in the worst case is $\frac{n(n-1)}{2}$.
Thus, the approximation bound is $O(n\sqrt{\log n})$, which is meaningless.
Furthermore, without any prior knowledge, any vertex can be candidate of landmarks, in order to construct the set-cover-with-pair instance,
we need to precompute and explicitly record the distance and shortest path between any pair of vertices.
Both running time and memory cost are prohibitively expensive for most of graphs.
}












\comment{
For the traditional landmark indexing, each vertex $u$ in directed graph is assigned with two lists $L_{out}(u)=(<d(u,v_1),SP_{u,v_1}>,<d(u,v_2),SP_{u,v_2}>,...,<d(u,v_k),SP_{u,v_k}>)$ and
$L_{in}(u)=(<d(v_1,u),SP_{v_1,u}>,<d(v_2,u),SP_{v_2,u}>,...,<d(v_k,u),SP_{v_k,u}>)$.
Note that, if some landmarks are not reachable from (or cannot reach) specific vertex, the corresponding distance and shortest path is set to be null.

All landmark selection strategies are motivated by the important observation:
for one vertex pair $u$ and $v$, if there exists one of shortest path between them going through one of landmarks, this shortest path can be recovered by these landmarks.
The ideal landmark set, refer to as {\em landmark cover}, are able to recover exact shortest path for any pair of vertices in the graph.
Although it is computationally intractable, most of landmark selection heuristics are still proposed to target this goal by utilizing graph's underlying properties.
In this section, we focus on investigating the essence of landmark cover which is able to guide us to the practical landmark selection.
Especially, we first describe a new landmark indexing scheme resulting in much compact index size compared to traditional landmark indices.
We formally define the optimal landmark cover discovery problem based on this indexing scheme, and show that this problem is NP-hard.
To address it, we propose an effective algorithm based on set-cover-with-pair (SCP) framework to discover landmark cover with logarithmic bound.

\subsection{Notation}
\label{notation}

To facilitate our discussion, we begin with defining some nation and terminology used in the rest of paper.
Let $G=(V,E)$ be an unweighted and directed graph where $V=\{1,2,...n\}$ is the vertex set and $E \subseteq V \times V$ is edge set.
The edge from vertex $u$ and $v$ is denoted by $(u,v)$, and we use $P_{v_0, v_p} = (v_0, v_1, ..., v_p)$ to denote a simple path from $v_0$ to $v_p$.
The length of a simple path in unweighted graph is the number of edges in the path.
Given two vertices $u$ and $v$, their shortest path $SP_{u,v}$ is the path between them with minimal length.
The distance from vertex $u$ to $v$ is the length of shortest path $SP_{u,v}$ from $u$ to $v$, denoted by $d(u,v)$.
For each vertex $u$, its $\epsilon$-neighbors, denoted as $N_{\epsilon}(u)$ is a set of vertices such that their distance to $u$ is no greater than $\epsilon$, i.e., $N_{\epsilon}(u) = \{v \in V | 0 < d(u,v) \le \epsilon\}$.

Suppose a subset of vertices $V^\ast=\{v_1,v_2,...,v_k\} \subseteq V$ has been selected as landmarks.
For the traditional landmark indexing, each vertex $u$ in directed graph is assigned with two lists $L_{out}(u)=(<d(u,v_1),SP_{u,v_1}>,<d(u,v_2),SP_{u,v_2}>,...,<d(u,v_k),SP_{u,v_k}>)$ and
$L_{in}(u)=(<d(v_1,u),SP_{v_1,u}>,<d(v_2,u),SP_{v_2,u}>,...,<d(v_k,u),SP_{v_k,u}>)$.
Note that, if some landmarks are not reachable from (or cannot reach) specific vertex, the corresponding distance and shortest path is set to be null.

For any vertex pair $(s,t)$, the traditional landmark scheme approximate the shortest path by concatenating shortest paths $SP_{s,v^\prime}$ and $SP_{v^\prime,t}$ where $v^\prime \in V^\ast$ achieves minimal $d(s,v^\prime)+d(v^\prime,t)$.
Clearly, if $v^\prime$ lies in one of shortest path from $s$ to $t$, the estimated shortest path is exact one.
In ideal situation, for any vertex pair $(s,t)$, we can always find a landmark $x$ from landmark set $V^\ast$ such that $d(s,v)+d(v,t)=d(s,t)$.
We refer to such landmark set as {\em landmark cover}.
%That is, there always exists a landmark from {\em landmark cover} appearing in one of shortest paths from $s$ to $t$.
Furthermore, 2hop labels are essentially a {\em landmark cover},
because for any pair of vertices, there always exists one common vertex in their corresponding label such that at least one of their shortest paths goes through it.
These common vertices serves as {\em landmark cover} in our scenario.

\comment{
Here, we formally define the {\em landmark cover} and {\em optimal landmark cover discovery problem} based above indexing scheme as follows:

\bdefin{\bf (Landmark Cover)}
Given unweighted and directed graph $G=(V,E)$, and a subset of vertices $V^\ast \subseteq V$, we say $V^\ast$ is a landmark cover if and only for any vertex pair $(s,t)$,
there exists a landmark $v \in V^\ast$
\edefin

\bdefin{(\bf (Optimal Landmark Cover Discovery Problem)}
Given unweighted and directed graph $G=(V,E)$, we would like to seek a landmark cover with smallest number of vertices.
\edefin
}

\begin{figure}
\centering
\begin{tabular}{c}
\psfig{figure=Figures/indexexample.eps,scale=0.65}
\end {tabular}
\caption {Indexing Example}
\label{fig:indexexample}
\end{figure}



\subsection{New Landmark Indexing Scheme}
\label{landmarkindex}

Considering a traditional landmark cover $V^\ast$ with $k$ landmarks, each vertex is required to explicitly maintain two $k$-element lists for the shortest path to (from) all landmarks.
Given a graph $G=(V,E)$, the total index size is clearly $2k|V|$.
However, we observe that many unnecessary landmarks are recorded for each specific vertex pair when one of their shortest paths goes through several landmarks.
%This is essentially caused by the query procedure which needs to find out a exact intermediate vertex in the shortest path.
%Simply speaking, the shortest path is expressed as two segments: the path from source to intermediate and the path from intermediate to destination.
In order to gain more compact index size,
we represent each shortest path as three segments instead of two segments in traditional methods: 1) the path from source to appropriate landmark close to it; 2) the path from current landmark to another landmark close to destination;
3) and the path between destination and above nearby landmarks.

We note that the functionality of these landmarks in this scenario is analogous to the highway entrances or exits of transportation network.
In order to find the shortest path from starting point to destination, one simply find the shortest path from starting to the appropriate entrance of highway,
and then get off the correct exit of highway which leads to the remaining shortest path to the destination.
Based on 3-segment expression, for any pair of vertices $(s,t)$, if there are many landmarks from one landmark cover appear in one of shortest path,
both $s$ and $t$ only need to store the {\em essential} landmark, i.e., the nearest one.
To facilitate the exact shortest path query, the middle segment connecting two landmarks are required to be available during online query.
As we discussed in section~\ref{contribution}, the landmark size is rather small and the shortest path among them is almost constant (no more than 3 in large social network),
thus the benefit from index size reduction would easily pay off the cost of materializing pairwise shortest path among landmarks.
This materialization essentially serves as {\em shortest path oracle} which is able to answer shortest path queries between any two landmarks in constant time.


\begin{example}
Figure~\ref{fig:indexexample} shows two different indexing schemes for vertex pair $(s,t)$ given that $3$ landmarks $v_1$, $v_2$ and $v_3$ appear in one of shortest path between them.
As we can see from traditional indexing, the shortest paths from $s$ to all landmarks and from landmarks to $t$ are all recorded.
According to 3-segment representation of shortest path, we only need to record one nearest landmark for each vertex, i.e., $v_1$ for source $s$ and $v_3$ for destination $t$.
The traditional landmark index size is reduced from $6$ to $2$.
Given the shortest path from $v_1$ to $v_3$, the shortest path $SP_{st}$ is easily recovered by $SP_{sv_1}+SP_{v_1 v_3}+SP_{v_3 t}$.
\end{example}


Our new landmark indexing scheme assigns each vertex $u$ two lists, $L^\prime_{out}(u)$ and $L^\prime_{in}(u)$.
$L^\prime_{out}(u)$ records the {\em essential} list of landmarks which is reachable from $u$, including their respective distance and shortest path,
i.e., $L^\prime_{out}(u)=(<x_1:d_{x_1},SP_{x_1}>,...,<x_p:d_{x_p},SP_{x_p}>)$, where $d_{x_i}=d(u,x_i)$ and $SP_{x_i} = SP_{u x_i}$.
Similarly, $L^\prime_{in}(u)$ records the {\em essential} list of landmarks which can reach $u$, including their respective distance and shortest path,
i.e., $L^\prime_{in}(u)=(<y_1:d_{y_1},SP_{y_1}>,...,<y_p:d_{y_p},SP_{y_q}>)$, where $d_{y_i}=d(y_i,u)$ and $SP_{y_i} = SP_{y_i u}$.
Both $x_i$ ($1 \le i \le p$) and $y_j$ ($1 \le j \le q$) are landmarks.
Given a shortest path query $(s,t)$, let $x_i \in L^\prime_{out}(s)$ and $y_i \in L^\prime_{in}(t)$.
We define the {\em landmark distance} from $s$ to $t$:
\beqnarr
d(s,t|L^\prime_{out}(s),L^\prime_{in}(t)) =  \nonumber \\
min_{x_i \in L^\prime_{out}(s), y_j \in L^\prime_{in}(t)} d(s,x_i)+d(x_i,y_j)+d(y_j,t) \nonumber
\eeqnarr
Corresponding {\em landmark shortest path} is the concatenation of $SP_{s x_i}$, $SP_{x_i y_j}$ and $SP_{y_j t}$.
Note that, the pairwise distance and shortest path among landmarks $d_(x_i y_j)$ and $SP_{x_i y_j}$ are materialized.
In addition, the index size is defined to be $\sum_{u \in V} (|L^\prime_{out}(u)| + |L^\prime_{in}(u)|)$.

If {\em landmark distance} by landmark set $V^\ast$ is exactly shortest distance for any pair of vertices,
we refer to $V^\ast$ as {\em landmark cover} in this setting.
Formally, we define {\em landmark cover} and {\em optimal landmark cover discovery problem} based new indexing scheme as follows:

\bdefin{\bf (Landmark Cover)}
Given unweighted and directed graph $G=(V,E)$, and a subset of vertices $V^\ast \subseteq V$, we say $V^\ast$ is a landmark cover if and only for any vertex pair $(s,t)$,
there exists two landmarks $x, y \in V^\ast$ such that $d(s,x)+d(x,y)+d(y,t)=d(s,t)$.
That is, there always exists two landmarks appearing in one of shortest paths from $s$ to $t$.
\edefin

When $x$ is the same with $y$, the landmark cover based on new indexing scheme is degraded to the one based on traditional indexing scheme,
which is also equivalent to the aforementioned 2-hop labels.

\bdefin{(\bf (Optimal Landmark Cover Discovery Problem)}
Given unweighted and directed graph $G=(V,E)$, we would like to seek a landmark cover such that its total index size based on new indexing scheme
$\sum_{u \in V} (|L^\prime_{out}(u)| + |L^\prime_{in}(u)|)$ is minimized.
\edefin


Since 2hop labeling problem can be treated as special case of Optimal Landmark Cover Discovery Problem, where two landmarks that serve as meeting point become only one.
we can easily derive following result:

\bthm
Given unweighted and directed graph $G=(V,E)$, Optimal Landmark Cover Discovery Problem is NP-hard problem.
\ethm

}



==> Intro.1.tex <==
\section{Introduction}
\label{intro}

Social networks are becoming ubiquitous and their data volume is increasing dramatically.
The popular online social network websites, such as Facebook, Twitter, and LinkedIn, all have hundreds of millions of active users nowadays. 
Google's new social network Google+ attracted 25 million unique users and was growing at a rate of roughly one million visitor per day in the first month after launch.
Enabling online and interactive query processing of
these massive graphs, especially to quickly capture/discover the relationship between entities,  is becoming an indispensable component for emerging applications from the social sciences, to advertisement and marketing research, as well as homeland security.  

Among them,  shortest path computation is the most basic, yet critical problem, for managing and querying social networks.
Social network website, LinkedIn,  pioneered the most well-known shortest-path service ``How you're connected to A'', which offers a precise description of friendship chain between you and  a user A within $3$ steps.
Microsoft's Renlifang (EntityCube) ~\cite{entitycube}, which records over a billion relationships for over
10 million entities (people, locations, organizations), allows users to retrieve the shortest path between two entities if their distance is smaller or equal to $6$. 
The newly emerged online application ``Six Degrees''~\footnote{http://www.6-degreesonline.com} provides an interactive way to demonstrate how you connect to other people in your Facebook network.
In addition, shortest path computation is also useful in determining the trust and discovering friends in online games~\cite{citeulike:7372248,zhao2011}. 

In all these emerging social network applications, (one) shortest path between two users needs to be computed generally only if their distance is less than a certain threshold (such as $6$). 
Such a focus directly resonates with the {\em small-world} phenomenon being observed in these massive social networks. 
For instance, the average pairwise distance distance on a large sample of Facebook users ~\footnote{http://www.6-degreesonline.com} has shown to be only $5.73$; also around half of users on Twitter are on average $4$ steps away from another while nearly everyone is $5$ steps away ~\footnote{http://www.sysomos.com/insidetwitter/sixdegrees/}. 
Not only most of the users in large social networks are separated by less than $6$ steps, the longer connections or paths in social networks are also less meaningful and/or useful. 
Therefore, computing shortest path within $6$-steps (or less) is the focus of these emerging applications, which can be formally described as the {\bf $k$-degree shortest path} query ($k \leq 6$ in general): 
{\em Given two vertices (users) $s$ and $t$ in a large (social) network, what is the shortest path from $s$ to $t$ if their distance is less than or equal to $k$?}
%In this paper, we will focus on {\em $6$-degree shortest path}, which is the most commonly used shortest path query in social network. 

Computing $k$-degree shortest path in large social network is surprisingly challenging, especially when $k$ is relatively large, such as $k=6$. 
A single BFS can easily visit more than a million vertices in $6$ steps in a large network with a few million of vertices. 
Though existing techniques~\cite{Jing98,Jung02,Shekhar97,Sanders05,BastFSS07,Gutman04,GoldbergSODA05,HananSA08,Sankaranarayanan:2009,Kriegel:2008:HGE,Geisberger:2008:CHF,Tao11,Bauer:2010:CHG} are very successful for finding the shortest path on large but sparse road networks,
these massive social graphs have quite different characteristics.
Instead of being spatial, with edge weight, and having low vertex degree, social networks are generally {\em non-spatial}, {\em non-weighted}, {\em scale-free} (especially consisting vertices with high-degree connections), and {\em small-world}  in addition to their massive size.
Indeed, due to the difficulty in finding the shortest path in social network,  the recent studies~\cite{Gubichev:2010:FAE:1871437.1871503,citeulike:7372248,zhao2011} all focus on discovering only the approximate ones (longer than the true shortest path). 
Furthermore, even with the approximation, the fastest methods, such as {\em Sketch}~\cite{Gubichev:2010:FAE:1871437.1871503}, {\em TreeSketch}~\cite{Gubichev:2010:FAE:1871437.1871503}, and {\em RigelPaths}~\cite{zhao2011}, still needs tens or hundreds of milliseconds ($10^{-6}$ second) to compute an approximate shortest path in a social network with a few million vertices. 


In this paper, we introduce a new {\bf Hub$^{\bf 2}$-Labeling} approach for computing the shortest path in large social networks. 
%Effectively leveraging the scale-free property in social network, 
The  Hub$^2$-Labeling approach is on average  over $2000$ times faster than the BFS in answering 
the {\em exact} $6$-degree shortest-path (or $k$-degree shortest-path) query. 
It effectively reduces the BFS search space by an average of more than three orders of magnitude. 
The Hub$^2$-Labeling  is also at least two orders of magnitude faster than the state-of-art approximate shortest path methods, including {\em Sketch}~\cite{Gubichev:2010:FAE:1871437.1871503}, {\em TreeSketch}~\cite{Gubichev:2010:FAE:1871437.1871503}, and {\em RigelPaths}~\cite{zhao2011}. 
In a single computation server with $24$GB memory, our approach can find the exact  $6$-degree shortest path  on average within tens of microseconds ($10^{-9}$) in a large social network with millions of vertices. 
The index size and index construction cost  of Hub$^2$-Labeling are also rather moderate and better than or comparable to the light approximation indexing {\em Sketch}~\cite{Gubichev:2010:FAE:1871437.1871503} method. 

The rest of papers are organized as follows. 
We first review the related works on shortest path computation (Section~\ref{related}). 
Then, we introduce the  Hub$^2$-Labeling framework (Section~\ref{framework}) and the indexing method (Section~\ref{hubsetselectionandlabeling}). 
We discuss the query algorithm in Section~\ref{}.
We present the detailed experimental evaluation  in Section~\ref{} and conclude the paper in Section~\ref{}. 


\section{Related Work}
\label{related}

In the following, we will review the existing methods on shortest path computation, especially related to social networks. 
Throughout our discussion, we use $n$ and $m$ to denote the number of nodes and edges in the graph $G$, respectively.

\noindent{\bf Online Shortest Path Computation:}
One of the most well-known methods for shortest path computation is Dijkstra's algorithm~\cite{Dijkstra59}.
It computes the single source shortest paths in a weighted graph and can be implemented with $O(m+n\log n)$ time. 
If the graph is unweighted (such as the social network), 
a Breadth-First Search (BFS) procedure can compute the shortest path in $O(m+n)$. 
However, it is prohibitively expensive to apply these methods to a social network with millions of vertices even for expending BFS up to $6$ steps. 
First, the average degree in the social network is relatively high. For instance, each user in Facebook on average has about $130$ friends. The straightforward BFS can easily scan one million vertices within $6$ steps. 
A simple strategy is to employ bidirectional search to reduce the search space. 
However,  the main difficulty is that the social networks are generally  scale-free and consist of some very high-degree vertices (often referred to as {\em hubs}). Each hub  can directly links to tens of thousands of friends (neighbors). 
Due to the small-world property, a large number of hubs may be traversed in bidirectional BFS (within three steps of 
the start $s$ or end $t$ of the shortest path query). 
For instance, in the Orkut graph (a frequently used benchmarking social network), which consists of over $3$ million vertices and $220$ million edges, a bidirectional BFS still needs to access almost $200K$ of vertices per query while the traditional BFS needs to access almost $1.6$ million of vertices per query. 

\noindent{\bf Shortest Path Computation on Road Networks:}
Computing shortest path on road networks has been widely studied~\cite{Jing98,Jung02,Shekhar97,Sanders05,BastFSS07,Gutman04,GoldbergSODA05,HananSA08,Sankaranarayanan:2009,Kriegel:2008:HGE,Geisberger:2008:CHF,Tao11,Bauer:2010:CHG}. Here we only provide a short review (More detailed review on this topic can be found in ~\cite{Delling:2009}).
Several early studies~\cite{Jing98,Jung02,Shekhar97}, such as {\em HEPV}~\cite{Jing98} and {\em HiTi}~\cite{Jung02},  utilize the decomposition of a topological map to speed up shortest path search.  
%For instance, in {\em HEPV}~\cite{Jing98} and {\em HiTi}~\cite{Jung02},  they first decompose the entire map into fragments (subgraphs), then they extract the {\em border nodes} (nodes in fragments directly adjacent to nodes in other fragments), and finally the relationship of these border nodes form a new graph to express the high level structure of the graphs.
Recently, a variety of techniques~\cite{Delling:2009}, such as $A^\ast$~\cite{GoldbergSODA05},  Arc-flag (directing the search towards the goal)~\cite{Bauer:2010:CHG}, highway hierarchies (building shortcuts to reduce search space)~\cite{Gutman04,Sanders05}, transit node routing (using a small set of vertices to relay the shortest path computation)~\cite{BastFSS07}, and utilizing spatial data structures to aggressively compress the distance matrix~\cite{HananSA08,Sankaranarayanan:2009}, have been developed.
However, the effectiveness of these approaches rely on the essential properties of road networks, such as almost planar, low vertex degree, weighted, spatial, and existence of hierarchical structure~\cite{Gubichev:2010:FAE:1871437.1871503}.
As we mentioned before, the social networks have different properties, such as non-spatial, unweighted, scale-free (existence of hubs), and small-world. 
For instance, those techniques utilizing spatial properties (triangle inequality) for pruning the search space immediately become infeasible in the social network. 
Also, the high vertex degree (hubs) easily lead to the explosion of search space. 

\noindent{\bf Theoretical Distance Labeling and Landmarking:} 
There have been several studies on estimating the distance between any vertices in large (social) networks~\cite{Potamias09,SarmaSMR10,Gubichev:2010:FAE:1871437.1871503, citeulike:7372248,zhao2011,DBLP:conf/icde/Qiao12}.
These methods in general belong to distance-labeling~\cite{DBLP:journals/jal/GavoillePPR04}, which assigns each vertex $u$ a label (for instance, a set of vertices and the distances from $u$ to each of them) and then estimate the shortest path distance between two vertices using the assigned labels.
The seminal work, referred to as the distance oracle~\cite{DBLP:journals/jacm/ThorupZ05},  by Thorup and Zwick shows a $(2k-1)$-multiplicative distance labeling scheme (the approximate distance is no more than $2k-1$ times the exact distance), for each integer $k\geq 1$, with labels of $O(n^{1/k} \log^2n)$ bits.
However, as Potamias {\em et al.}~\cite{Potamias09} argued, for practical purposes,
even $k=2$ is unacceptable (due to small-world phenomenon).
Recently, Sarma {\em et al.}~\cite{SarmaSMR10} study Thorup and Zwick's distance oracle method on real Web graphs and they found this method can provide fairly accurate estimation. 

The pioneering $2$-hop distance method by Cohen {\em et al.}~\cite{cohen2hop} provides exact distance labeling on directed graphs (which is very similar to the $2$-hop reachability indexing).
Specifically, each vertex $u$ records a list of intermediate vertices $L_{out}(u)$ it can reach along with their (shortest) distances, and a list of intermediate vertices $L_{in}(u)$ which can reach it along with their distances.
To find the distance from $u$ to $v$, the $2$-hop method simply checks all the common intermediate vertices between $L_{out}(u)$ and $L_{in}(v)$ and choose the vertex $p$, such that $dist(u,p)+dist(p,v)$ is minimized for all $p \in L_{out}(u) \cap L_{in}(v)$. However, the computational cost to construct an optimal $2$-hop labeling is prohibitively expensive~\cite{hopiedbt,DBLP:conf/sigmod/JinXRF09}. 

Several works uses {\em landmarks} to approximate the shortest path distance ~\cite{Ng01predictinginternet,Kleinberg04,Potamias09,citeulike:7372248,zhao2011,DBLP:conf/icde/Qiao12}.
Here, each vertex precomputes the shortest distance to a set of landmarks and thus the landmark approach can be viewed as a special case of $2$-hop and distance labeling where each vertex can record the distance to different vertices. 
Specifically, Potamias {\em et al.}~\cite{Potamias09} investigates the selection of the optimal set of landmarks to estimate the shortest path distance; Qiao {\em et al.} ~\cite{DBLP:conf/icde/Qiao12} observe that globally selected landmark set introduces too large error, especially for some vertex pairs with small distance, and propose a query-load aware landmark selection method; Zhao {\em et al.}~\cite{zhao2011} introduces Rigel, which utilizes the hyperbolic space embedding on top of the landmark to improve the estimation accuracy. 

\noindent{\bf Approximate Shortest Path Computation in Social Networks:} 
A few recent studies aim to compute the shortest path in large social networks.  They extend the distance-labeling or the landmarking approach to approximate the shortest paths. 
Gubichev {\em et al.}  propose {\em Sketch}, which generalizes the distance oracle method~\cite{DBLP:journals/jacm/ThorupZ05,SarmaSMR10} to discover the shortest path (not only the distance) in large graphs~\cite{Gubichev:2010:FAE:1871437.1871503}.
They observe that the path lengths are small enough to be considered as almost constant and therefore store a set of precomputed shortest path in addition to the distance labeling. 
They also propose several improvements, such as {\em cycle elimination} (SketchCE), {\em tree-based search} (TreeSketch), to boost the shortest path accuracy (their length closer to the exact shortest path). 
Zhao {\em et al.}~\cite{zhao2011} develops {\em RigelPath} to approximate the shortest path in social network on top of their distance estimation method, Rigel. 
Their basic idea is to use the distance estimation to help determine the search direction and prune search space. 
The Sketch is the fastest approximate shortest path method, though the RigelPath and TreeSketch can be more accurate. 
In addition, the RigelPath mainly focuses on the undirected graph, while the Sketch based method can handle both directed and undirected graphs. 



==> Labeling.tex <==
\section{Indexing  Approach for Hub$^{\textstyle 2}$-Labeling}
\label{hubsetselectionandlabeling}

In this section, we will discuss how to construct the hub-set $\mathcal{H}$ (Subsection~\ref{hubsetselection}), and how to compute the core-hub labeling $L_H$ for each vertex $v$ efficiently (Subsection~\ref{indexingalgo}). 

\subsection{Hub-Set Construction}
\label{hubsetselection}

The vertices in hub-set have similar functionality to the landmarks, which aim to maximally {\em cover} the shortest paths in the graph. 
Intuitively, a  shortest path is covered by the hub-set if it consists of at least one vertex in the hub-set. 
Formally, we define the goodness of a hub-set using the {\em coverage} criterion: 

\bdefin{\bf (Hub-Set Coverage)}
Given a hub-set $\mathcal{H}$ and vertex pair $(s,t)$, if the estimated shortest distance using hub-set indexing scheme is {\em exact} distance (i.e., $d(s,t)=$ \\ $min_{x \in L_{H}(s) \wedge y \in L_{H}(t)} (d(s,x)+d(x,y)+d(y,t))$),
we say vertex pair $(s,t)$ is covered by hub-set $\mathcal{H}$.
Let $C(\mathcal{H})$ be the number of (unique) vertex pairs covered by the hub-set $\mathcal{H}$. 
\edefin

Given this,  we are interested in maximally covering the shortest path distance using a limited number of vertices in the hub-set (in order to hold the distance matrix Hub$^2$). 
This can be formally described as follows: 

\bdefin{\bf (Optimal Hub-Set Selection Problem)}
Given graph $G=(V,E)$ and parameter $K$, we would like to find $\mathcal{H} \in V$,
such that $|\mathcal{H}|=K$ and the number of vertex pairs $(s,t) \in V \times V$ covered by $L$ is maximized ($\max{C(\mathcal{H})}$).
\edefin

Unfortunately, this problem is NP-hard. 
\bthm
The  optimal hub-set selection problem is NP-hard and it is also equivalent to the $k$-landmark-cover problem~\cite{Potamias09}. 
\ethm

The proof is in the appendix. 
Given this, we consider how to heuristically select vertices in the hub-set. It is quite similar to the landmark selection though here we focus on the coverage criterion on the social network. 
Let us start from the most simple scenario to gain a better intuition of good hub-set in social networks.
Intuitively, the best hub-set vertices should be the one in the very {\em central} position of graph since they tend to cover a large number of shortest paths~\cite{Potamias09}.
This high-level understanding suggests two concepts of {\em central} vertex from different perspectives:
1) it is a vertex lying on many shortest paths, which can be measured by vertex betweenness centrality;
2) it is a vertex close to other vertices in the graph, which can be measured by closeness centrality.
In the optimized scenario, the best {\em central} vertex based on first concept is referred to as the vertex with largest vertex betweenness~\cite{citeulike:1025135},
while second one refers to the vertex with optimal closeness centrality.
We generalize both concepts to hub-set selections in social networks.

\noindent{\bf Vertex Betweenness Criterion: }
The vertex betweenness firstly introduced by Freeman~\cite{citeulike:1025135} in the context of social science:
\[  C_B(v) = \sum_{u,w \in V \wedge u\neq w \neq v} \frac{\sigma_{uw}(v)}{\sigma_{uw}} \]
where $\sigma_{uw}(v)$ is the total number of shortest paths between $u$ and $w$ that pass through $v$,
and $\sigma_{uw}$ is the total number of shortest paths between $u$ and $w$.

We sort all vertices based on their vertex betweenness centrality in descending order and pick top $K$ vertices as hub-set.
To achieve this goal, we need to precompute vertex betweenness centrality for every vertex.
However, the fastest (exact) algorithm to compute every vertex betweenness centrality is $O(|V||E|)$~\cite{Brandes2001}, which is still rather expensive for massive networks. 

\noindent{\bf Closeness Betweenness Criterion: }
The closeness of a vertex is evaluated by the inverse of its total distance to all other vertices in the graph~\cite{citeulike:7062391}.
The vertex is the more central the lower its total distance to the remaining vertices. That is,
\[ C_C(v) = \frac{|V|-1}{ \sum_{u \in V \wedge u \neq v} d(v,u) }  \]

The intuition of using this criterion is that, a vertex closer to all other vertices are very likely to be part of many shortest paths.
Therefore, we select top $K$ vertices with largest closeness centrality to be hub-set.
Similar to computing vertex betweenness, calculating closeness betweenness involving pairwise shortest paths computation is an expensive task,
taking $O(|V|(|V|+|E|))$ time in unweighted graph setting.

\noindent{\bf Hub-Set=\{Hub\}:} 
Although it is costly to select $K$ hub-set vertices strictly following aforementioned criteria, 
we are able to adopt {\em the vertices with high vertex degree}, i.e., the {\em hubs}, as their effective proxies in social networks.
This is based on key observations on how high-degree vertices (hubs) contribute social networks' connectivity and small path length. 
The empirical study on several well-known social networks (i.e., Flickr, LiveJournal, Orkut and Youtube) reported in~\cite{Mislove07}
clearly demonstrates the presence of densely connected {\em core} comprising of a small portion of vertices with highest degree.
The removal of this {\em core} dramatically disconnects entire graph, implying that most of pairwise connections rely on few high-degree vertices (hubs).
In other words, few high degree vertices serve as key intermediates in most of shortest paths, thus are qualified to be the hub-set vertices under vertex betweenness criterion.
In addition, this study ~\cite{Mislove07} also analyzes the average shortest path length in the core containing only highest-degree vertices. 
As core grows, the average shortest path length increases sub-logarithmically.
Since average shortest path length of entire graph is very small, this phenomenon suggests that the lower degree vertices that constitute the majority of the network are very close to the high degree vertices in the core.
In this sense, high-degree vertices (hubs) are also qualified under the closeness betweenness criterion.

To sum, we simply select the top $K$ high-degree vertices (hubs) in the original graph $G$ as the hub-set ($\mathcal{H}$) (That is also the reason why we refer to $\mathcal{H}$ as the hub-set). 
In addition, we note that another advantage of using the hubs in the hub-set is to reduce the search space. 
Recall that in the bidirectional search (the query processing step), any vertices in the hub-set do not need to be expanded. 
In this way, we can effectively avoid those high-degree vertices (hubs), which form the very reason for search space explosion. 
Finally, in the rest of the paper, we will also use  the hub-set vertices and the hubs exchangeably. 


\subsection{Core-Hub Labeling}
\label{indexingalgo}

In this subsection, we present an efficient algorithm to assign each vertex $u$ its core hubs $L_{H}(u)$.  
The goal of $6$-degree shortest path is to compute the shortest path with length no greater than $6$ (or $k$ in general).
Given this, it is easy to see that {\em for any hub $h$ in $\mathcal{H}$ to be assigned to $L_H(u)$, their distance has to be no greater than $6$ ($d(h,u) \leq 6$). }
This is because for any vertex pair $(s,t)$, the estimation using the hub-set is to provide an upper-bound  for the bidirectional search, which is also constrained by $6$. 
Thus, if the upper-bound is greater than $6$, it becomes useless.


Now, let us consider the straightforward approach based on the core-hub definition (Definition~\ref{corehubdef}) for labeling.
In this case, we need  first precompute all pairwise distances among hubs and materialize all distances between hubs and other vertices if they are no greater than $6$. 
Since the size of hub-set $\mathcal{H}$ is quite large, the materialization cost of $|V||\mathcal{H}|$ is too high. 

Here, we introduce an efficient procedure which only performs one local breadth-first traversal (BFS) for each hub in $\mathcal{H}$ to visit its $6$-degree neighbors(i.e., the vertices with distance to the hub no more than $6$) and no additional distance-matrix materialization is needed. 
In addition, this procedure also construct the distance matrix Hub$^2$ during the labeling process. 
Given this, for each BFS starting from a hub $h \in \mathcal{H}$, two tasks need to be performed: 
1) it needs to find out all other hubs whose distance to $u$ is no more than $6$, and record one shortest path between them (distance matrix construction);
2) for each visited non-hub vertex $v$ during BFS, we need to quickly check whether $h$ is $v$'s core hub, i.e., whether $u \in L_H(v)$.
This is equivalent to determine whether there is other hubs appearing in a shortest path between $u$ and $v$.
The first task can be easily achieved by introducing an extra integer for each vertex, which is used to record the previous vertex on the shortest path from hub $h$ to current vertex along shortest path.
The first task is relatively straightforward as a basic BFS process can easily accomplish that. 
The second task is non-trivial and is the main focus.

To quickly determine whether $h \in L_H(v)$ during the BFS process, we utilize the following observation:
{\em Let vertex $y$ lies on a shortest path from hub $h$ to non-hub vertex $v$ with distance $d(h,v)-1$ (i.e., $y$ is one hop closer than $v$ with respect to $h$). 
If there is a hub $h^\prime$ appearing in a shortest path from $h$ to $y$ ($h^\prime$ and $y$ may not be distinct),
$h^\prime$ definitely lies on a shortest path from $h$ to $v$ and $h$ cannot be core hub of $v$.}
Based on this observation, we simply maintain a binary flag $b(v)$ to denote whether there is another hub appearing in a shortest path between $h$ and $v$.
Specifically, its update rule is as follows: $b(v)=1$ if $v$ itself is hub or $b(y)=1$ where $d(h,y)=d(h,v)-1$ and $d(y,v)=1$.
Thus, during BFS traversal, when we visit vertex $v$, if its flag $b(v) \neq 1$ meaning there is no other hubs lying on the shortest path between $h$ and $v$, we add $h$ and the corresponding shortest path $SP(h,v)$ to its $L_{H}(v)$.

\begin{example}
Figure~\ref{fig:bfsindexexample} shows an example of core-hub labeling. 
The value attached to each vertex $v$ is its binary flag $b(v)$, such as $b(1)=0$ and $b(2)=1$.
As we know, BFS process visits vertices in levelwise manner with the help of queue. 
We start from hub $h$ to visit its neighbors $1$, $2$ and $3$ in level $1$ and push them ino queue.
When vertex $2$ is popped from queue, its binary flag $b(2)$ is set to be $1$ since it belongs to hub-set.
Afterward, the flags of its immediate neighbors in level $2$ (i.e., vertices $5$ and $7$) are all set to be $1$,
because their neighbor $2$ in level $1$ is hub and lies on shortest paths from hub $h$ to them.
Therefore, hub $h$ cannot be core-hub of $5$ and $7$.
However, the flag of vertex $6$ is $0$ since flags of all its immediate neighbors in level $1$ are $0$,
meaning no hub lying on shortest paths from $h$ to $6$,
thus $h \in L_H(6)$.
%In this sense, binary flag is used to efficiently check whether $h$ is its 6-neighborhood's core-hub. 
\end{example}


\begin{figure}
\centering
\begin{tabular}{c}
\psfig{figure=Figures/bfsindexexample.eps,scale=0.65}
\end {tabular}
\caption{Example for Core-hub Labeling (only consider 3 hops)}
\label{fig:bfsindexexample}
\end{figure}


\input{Figures/BFSIndexing.tex}

The outline of BFS-based procedure for generating core-hubs indices is described in Algorithm~\ref{alg:bfsindex}.
The flag $b(v)$ for each vertex $v$ is updated when $v$ is hub or the flag of its previous vertex in $SP(h,v)$ is one (Line 6 and Line 18).
When vertex $u$ is popped from queue and its flag $b(u)=0$, hub $s$ is assigned to $L_{H}(u)$ (Line 10).
This procedure will be invoked for each hub.
In total, this procedure takes $O(\sum_{h \in \mathcal{H}} (|N_6(h)|+|E_6(h)|))$ time, where $L$ is hub-set, $N_6(h)$ ($E_6(h)$) is the number of vertices (edges) in $u$'s 6-degree neighborhood.

































%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Given a vertex pair $(s,t)$, if their $L^c_{out}(s)$ and $L^c_{in}(t)$ are able to recover the {\em exact} shortest path,
%this shortest path also can be recovered by using traditional indices $L_{out}(s)$ and $L_{in}(t)$,
%because $L^c_{out}(s) \subseteq L_{out}(s)=Succ(s|L)$ and $L^c_{in}(t) \subseteq L_{in}(t)=Pred(t|L)$.
%Essentially, core landmark indexing is the generalization of traditional landmark indexing,
%because it can not only utilize single landmarks, but also a pair of landmarks to estimate shortest path.

\comment{
\section{Local Landmark Framework}
\label{landmark}

In this section, we describe a new indexing scheme using landmarks to effectively encode the shortest path information.
Given a landmark set, new indexing scheme not only provides much compact indices, but also guarantees the resulting shortest path no long than the one by traditional landmark approach.
We formally define the optimal landmark selection problem based on new indexing scheme.
Then, we show that this problem is NP-hard and propose a greedy solution based on set-cover-with-pair framework to achieve logarithmic approximation.


To facilitate our discussion, we begin with defining some nation and terminology used in the rest of paper.
Let $G=(V,E)$ be an unweighted graph where $V=\{1,2,...n\}$ is the vertex set and $E \subseteq V \times V$ is edge set.
The edge from vertex $u$ and $v$ is denoted by $(u,v)$, and we use $P(v_0, v_p) = (v_0, v_1, ..., v_p)$ to denote a simple path from $v_0$ to $v_p$.
The length of a simple path in unweighted graph is the number of edges in the path.
Given two vertices $u$ and $v$, their shortest path $SP(u,v)$ is the path between them with minimal length.
The distance from vertex $u$ to $v$ is the length of shortest path $SP(u,v)$ from $u$ to $v$, denoted by $d(u,v)$.
For each vertex $u$, its $\epsilon$-neighbors, denoted as $N_{\epsilon}(u)$ is a set of vertices such that their distance to $u$ is no greater than $\epsilon$, i.e., $N_{\epsilon}(u) = \{v \in V | 0 < d(u,v) \le \epsilon\}$.
Given a vertex set $V^\ast$, for each each vertex $u \notin V^\ast$,
$Succ(u|V^\ast)$ is a subset of $V^\ast$ which can be reached from $u$ and $Pred(u|V^\ast)$ is a subset of $V^\ast$ which can reach $u$.
Due to the popularity of directed graphs in social networks, we focus on the undirected and unweighted graphs in the paper.
Taking a undirected graph as a bidirected graph, all techniques discussed in the paper can be easily extended to undirected setting.


\subsection{Global Landmark Indexing}
\label{globalindex}

Given graph $G=(V,E)$, suppose a subset of ordered vertices $V^\ast=\{x_1,x_2,...,x_k\} \subseteq V$ has been selected to be {\em landmarks}.
For each landmark $x_i$, we need to precompute and explicitly store the shortest path to all vertices in the graph $G$.
Then, we distribute these shortest path information to every vertex, such that each vertex $u$ is associated with two vectors:
{\small
\beqnarr
L_{in}(u)  = (<x_1: d(x_1,u),SP(x_1,u)>...,<x_p: d(x_p,u),SP(x_p,u)>)  \nonumber \\
L_{out}(u) = (<y_1: d(u,y_1),SP(u,y_1)>...,<y_q: d(u,y_q),SP(u,y_q)>) \nonumber
\eeqnarr
}
where $x_i \in Pred(u|V^\ast)$ ($1 \le i \le p$) and $y_j \in Succ(u|V^\ast)$ ($1 \le j \le q$).
Since all landmark information are propagated to entire graph, we refer to this traditional indexing scheme as {\em Global Landmark Indexing} scheme.
Given this, for a pair of vertices $s$ and $t$, their {\em landmark distance $d(s,t|V^\ast)$} and {\em landmark shortest path $SP(s,t|V^\ast)$} are defined based on triangle inequality:
{\small
\beqnarr
d(s,t|V^\ast) = min_{x \in L_{out}(s) \cap L_{in}(t)} \{ d(s,x)+d(x,t) \} \nonumber \\
SP(s,t|V^\ast) = SP(s,x^\ast) \circ SP(x^\ast,t) \nonumber \\
 \text{ where } x^\ast = \underset{x \in L_{out}(s) \cap L_{in}(t)}{\operatorname{argmin}} d(s,x)+d(x,t) \nonumber
\eeqnarr
}
where $\circ$ is the concatenation operator for two paths by connecting the first path's ending node and second path's starting node.
Clearly, given landmark set $V^\ast$, the landmark index size of total graph is $\sum_{u \in V} |L_{out}(u)|+|L_{in}(u)| = \sum_{u \in V} |Pred(u|V^\ast)| + |Succ(u|V^\ast)|$.

When landmark distance is equivalent to distance in the graph $G$, the landmark shortest path is actually the exact shortest path for a pair of vertices.
We say a set of vertices are {\em exact landmarks} if the landmark distance of any pair of vertices is exact distance in the graph $G$.
Simply speaking, for any two reachable vertices, there always exists one vertex from {\em exact landmarks} appearing in one of the shortest paths between them.
The problem of discovering exact landmarks with smallest cardinality has been proved to be NP-hard~\cite{Potamias:2009:FSP:1645953.1646063}.
Due to the hardness of selecting exact landmarks, most of existing works concentrate on developing different heuristics utilizing certain graph properties, such as vertex centrality, degree distribution or graph diameter.
Few of them attempt to improve the accuracy from indexing perspective.


\begin{figure}
\centering
\begin{tabular}{c}
\psfig{figure=Figures/indexexample.eps,scale=0.6}
\end {tabular}
\caption {Indexing Example}
\label{fig:indexexample}
\end{figure}

\begin{figure}
\centering
\begin{tabular}{c}
\psfig{figure=Figures/proofcases.eps,scale=0.65}
\end {tabular}
\caption {Cases in proof of Lemma~\ref{localgoodpath}}
\label{fig:proofcases}
\end{figure}



\subsection{Local Landmark Indexing}
\label{localindex}

In global landmark indexing scheme, each vertex is required to explicitly record all shortest distance and shortest path to (from) the landmarks which is reachable (can be reached).
However, we observe that many landmarks are redundant for each specific vertex under certain condition.
More specifically, each vertex only needs to record a subset of {\em essential} landmarks such that on other landmarks appear in the shortest path between them.
Using a slightly modified shortest path computation strategy, the recorded landmarks guarantee to generate a path which is no longer than the one produced by global indexing scheme.
Before we formally introduce new indexing scheme, let us go over a simple example to gain intuitive understanding.

\begin{example}
\label{indexexamp}
Figure~\ref{fig:indexexample} shows a shortest path from $s$ to $t$ while three landmarks $v_1$, $v_2$ and $v_3$ lie in this shortest path.
In global landmark indexing, both outgoing indices of source $s$ and incoming indices of destination $t$ need to record all three landmarks.
If shortest path $SP(v_1,v_3)$ between two landmarks $v_1$ and $v_3$ is known beforehand,
landmark $v_1$ included in $L_{out}(s)$ and landmark $v_3$ included in $L_{in}(t)$ are sufficient to recover the shortest path $SP(s,t)$,
i.e., $SP(s,t)= SP(s,v_1) \circ SP(v_1,v_3) \circ SP(v_3,t)$.
We can see that, the shortest path $SP(v_1,v_3)$ between two landmarks are implicitly recorded twice in $SP(s,v_3)$ and $SP(v_1,t)$,
thus materializing $SP(v_1,v_3)$ does not introduce any extra index cost.
\end{example}

In the example, we actually represent the shortest path $SP(s,t)$ by three segments:
1) $SP(s,v_1)$, from source $s$ to one close landmark $v_1$; 2) $SP(v_1,v_3)$, from landmark $v_1$ to another landmark $v_3$ close to destination $t$;
and 3) $SP(v_3,t)$, from landmark $v_3$ to destination $t$.
To some extent, two intermediate landmarks in the shortest path mimic the highway entrances or exits of transportation network.
In order to find the shortest path from starting point to destination, one simply find the shortest path from starting to the appropriate entrance of highway,
and then get off the correct exit of highway which leads to the remaining shortest path to the destination.
The shortest paths among landmarks serve as {\em shortest path oracle} which can answer the shortest path queries quickly, such as in constant time.

Now, given a landmark set $V^\ast$, we formally define {\em incoming essential landmarks} and {\em outgoing essential landmarks} for each vertex $u$:

\bdefin{\bf (Essential Landmarks)}
Given graph $G=(V,E)$ and a landmark set $V^\ast$, for each vertex $u$, its outgoing essential landmarks $L^e_{out}(u)$ contains landmark $x$,
if there does not exist $x^\prime \in V^\ast$ satisfying $d(u,x)=d(u,x^\prime)+d(x^\prime,x)$.
Simply speaking, no other landmarks appear in one of shortest path from $u$ to $x$.
Similarly, its incoming essential landmarks $L^e_{in}(u)$ contains landmark $y$,
if there is no $y^\prime \in V^\ast$ satisfying $d(y,u)=d(y,y^\prime)+d(y^\prime,u)$.
\edefin

The exclusion of a landmark $x$ in the essential landmarks with respect to vertex $u$ means there exists other landmark appear in the shortest path $SP(u,x)$ and closer to $u$ than $x$.
Recalling example~\ref{indexexamp}, $v_3$ is non-essential for source $s$, since the shortest path from $s$ to $v_3$ can be ``blocked'' by $v_1$.
The {\em incoming essential landmarks} and {\em outgoing essential landmarks} of each vertex constitute the indices of new landmark indexing scheme.
Opposing to global landmark indexing which needs to store all reachable (can be reached) landmarks, we refer to this indexing scheme as {\em local landmark indexing}.
Based on local indexing, we are able to compute its corresponding {\em landmark distance $d^e(s,t|V^\ast)$} and {\em landmark shortest path $SP^e(s,t|V^\ast)$} are defined as:
\beqnarr
d^e(s,t|V^\ast) = min_{x \in L^e_{out}(s) \wedge y \in L^e_{in}(t)} \{ d(s,x)+d(x,y)+d(y,t) \} \nonumber \\
SP^e(s,t|V^\ast) = SP(s,x^\ast) \circ SP(x^\ast,y^\ast) \circ SP(y^\ast,t) \nonumber \\
\text{ where } x^\ast = \underset{x \in L^e_{out}(s) \wedge y \in L^e_{in}(t)}{\operatorname{argmin}} d(s,x)+d(x,y)+d(x,t) \nonumber
\eeqnarr
In this sense, we need to materialize the pairwise shortest path among landmarks.
However, this materialization does not impose burden on the memory cost due to two reasons.
First, the length of shortest path in the social networks we focus on in this work is typically rather small~\cite{Mislove07}.
In our experiments, we observe that the length of most shortest paths between landmarks is no more than 3.
Second, lots of shortest paths between landmarks are implicitly encoded multiple times in global landmark indexing (e.g., Figure~\ref{fig:indexexample}, $SP(v_1,v_3)$ is contained in $SP(s,v_3)$ and $SP(v_1,t)$).

In addition, it is not hard to see that, local landmark indexing is a generalization of global landmark indexing.
In other words, if there is no shortest path from non-landmark vertex to landmark (or from landmark to non-landmark vertex) is ``blocked'' by some landmarks,
local landmark indexing degrades to global landmark indexing.
Hence, the index size of local landmark indexing $\sum_{u \in V} (|L^e_{out}(u)| + |L^e_{in}(u)|)$ is no larger that of global indexing.
More importantly, we have following observation:

\blemma
\label{localgoodpath}
The shortest path generated by local landmark indexing is no longer than the best one generated by global landmark indexing.
\elemma

\bproof
We want to prove that, for any path generated by global landmark indexing, we are able to find a path no longer that it based on local landmark indexing.
Without loss of generality, consider reachable vertex pair $(s,t)$, let us denote one path obtained by global landmark indexing as $SP(s,x) \circ SP(x,t)$,
where $x$ is the intermediate landmark in the path (i.e., $x \in L_{out}(s)$ and $x \in L_{in}(t)$.
Now, we try to find a path based on local landmark indexing which is not longer than $SP(s,x) \circ SP(x,t)$ in the following cases:
%we consider the outgoing indices $L^e_{out}(s)$ of source and incoming indices $L^e_{in}(t)$ of destination with respect to $x$ based on local landmark indexing:

\noindent 1) $x \in L^e_{out}(s)$ and $x \in L^e_{in}(t)$. It is trivial to generate the same path $P(s,x) \circ P(x,t)$.

\noindent 2) $x \in L^e_{out}(s)$ and $x \notin L^e_{in}(t)$. According to the definition of {\em essential landmarks}, there is some landmark $y \in L^e_{in}(t)$ appear in the shortest path from $x$ to $t$, i.e., $d(x,t)=d(x,y)+d(y,t)$ (case $2$ shown in Figure~\ref{fig:proofcases}).
Since the shortest path $SP(x,y)$ from landmark $x$ to $y$ is available beforehand, we are able to generate the path $SP(s,x) \circ SP(x,y) \circ SP(y,t)$ with the same length as $SP(s,x) \circ SP(x,t)$.

\noindent 3) $x \notin L^e_{out}(s)$ and $x \in L^e_{in}(t)$. Follow the similar logic in case 2 (case 3 in Figure~\ref{fig:proofcases}). We guarantee to have $y \in L^e_{out}(s)$ appear in $SP(s,x)$. Thus, we can generate path $SP(s,y) \circ SP(y,x) \circ SP(x,t)$ which is no longer than $SP(s,x) \circ SP(x,t)$.

\noindent 4) $x \notin L^e_{out}(s)$ and $x \notin L^e_{in}(t)$. That is, there are some other landmarks $y_1 \in L^e_{out}(s)$ and $y_2 \in L^e_{in}(t)$ appear in the shortest paths $SP(s,x)$ and $SP(x,t)$, respectively (case 4 shown in Figure~\ref{fig:proofcases}).
Moreover the shortest path $SP(y_1,y_2)$ between landmarks $y_1$ and $y_2$ are known.
Due to triangle inequality $d(y_1,y_2) \le d(y_1,x)+d(x,y_2)$, we are able to generate the shorter path $SP(s,y_1) \circ SP(y_1,y_2) \circ SP(y_2,t)$
compared to $SP(s,x) \circ SP(x,t)$.

Putting those together, in any case, we can find a path based on local landmark indexing no worse than the one generated by global landmark indexing.
Therefore, the statement follows.
\eproof

Local landmark indexing scheme not only provides much compact index size, but also guarantees the resulting shortest path no long than the one by global landmark indexing scheme.
On the other hand, due to the properties of social networks, such as small diameter and massive size,
the desired landmarks should be able to provide exact shortest path using compact index size.
Motivated by this requirement, we formally define the concept of landmark coverage and following exact landmark discovery problem:

\bdefin{\bf (Landmark Coverage)}
Given graph $G=(V,E)$ and landmark set $V^\ast \subseteq V$, for a vertex pair $(s,t)$,
we say $V^\ast$ {\em covers} vertex pair $(s,t)$ if there exists two landmarks $x,y \in V^\ast$ appearing in the shortest path from $s$ to $t$.
Note that, two landmarks may not be distinct, i.e., $x$ may be the same with $y$.
\edefin

\bdefin{\bf (Exact Landmark Set Discovery Problem)}
Given an unweighted and directed graph $G=(V,E)$, the exact landmark set discovery problem tries to find a set of landmarks $V^\ast \in V$
which can cover any pair of reachable vertices and the local landmark index size is minimized.
\edefin

\comment{
\bdefin{\bf (Exact Landmark Set Discovery Problem)}
Given an unweighted and directed graph $G=(V,E)$, the exact landmark set discovery problem tries to find a set of landmarks $V^\ast \in V$,
such that for any pair of reachable vertices $(s,t)$, their corresponding local indices satisfy:
\[ d^e(s,t|V^\ast) = d(s,t) \]
where the local landmark index size is minimized.
\edefin
}


\subsection{Transform to Set-Cover-with-Pairs}
\label{scpsolution}

In this section, we transform the exact landmark set discovery problem to set-cover-with-pair instance.
To be self-contained, we first briefly introduce the set-cover-with-pair problem~\cite{HS05}.

\bdefin{\bf (Set-Cover-with-Pairs Problem ~\cite{HS05})}
Let $U$ be the ground set and let $S = \{1, \ldots, M\}$ be a set of objects, where each object $i\in S$ has a non-negative cost $w_i$.
For every $\{i,j\}\subseteq S$, let $\mathcal{C}(i, j)$ be the collection of elements in $U$ covered by the pair $\{i, j\}$.
The objective of the set cover with pairs (SCP) problem is to find a subset $S^\prime \subseteq S$ such that
$\mathcal{C}(S^\prime) =\bigcup_{\{i,j\}\subseteq S^\prime} \mathcal{C}(i, j) = U$ with a minimum covering cost $\sum_{i\in S} w_i$.
We refer to the special case in which each object has a unit weight ($w_i=1$) as the \textbf{cardinality SCP} problem.
\edefin

Now we transform our exact landmark set discovery problem to the Set-Cover-with-Pairs problem as follows.
Let the ground set $U=TC(G)$, i.e., it contains any vertex pair $(u,v)$ in $G$, such that $u \rightarrow v$.
To cover a pair $(u,v)$ means we can recover one of their shortest paths in the new landmark indexing scheme.

In our directed graph setting, we categorize objects in $Q$ into two types: starting objects $Q^s$ and ending objects $Q^e$ with respect to two endpoints of each shortest path.
Each starting object $O^s_{u,x_i}$ in $Q$ corresponds to a tuple $(u,(x_i: d_{x_i}, SP_{x_i}))$, where $u$ is a starting vertex and $x_i$ is a candidate landmark can be reached from $u$.
Note that, $d_{x_i}= d(u,x_i)$ and $SP_{x_i}=SP(u x_i)$ are shortest distance and one shortest path from $u$ to $x_i$, respectively.
Similarly, each ending object $O^e_{y_j,v}$ in $Q$ corresponds to a tuple $((y_j: d_{y_j}, SP_{y_j}),v)$, where $v$ is ending vertex and $y_j$ is a candidate landmark can reach $v$.
Here, $d_{y_j}= d(y_j,v)$ and $SP_{y_j}=SP(y_j, v)$ are shortest distance and one shortest path from $y_j$ to $v$, respectively.
Now, we define $\mathcal(O_{u,x_i}, O_{y_j,v})$ for each pair of objects $O_{u,x_i}$ and $O(y_j,v)$.
Given any four vertices $(u,x_i,y_j,v)$, if $d(u,x_i)+d(x_i,y_j)+d(y_j,v)=d(u,v)$, then vertex pair $(u,v)$ is covered by objects pair $\{O^s_{u,x_i}, O^e_{y_j,v}\}$.
That is, $\mathcal{C}(O^s_{u,x_i}, O^e_{y_j,v})$ contains vertex pair $(u,v)$.
Otherwise, $\mathcal{C}(O_{u,x}, O_{y,v})=\emptyset$.
Note that, aforementioned four vertices may not be distinct, i.e., $u$ may be the same with $x_i$, $x_i$ may be the same with $y_j$, etc.
%From the viewpoint of restoring shortest paths, that vertex pair $(u,v)$ is covered by objects pair $\{O^s_{u,x_i}, O^e_{y_j,v}\}$ means there exists one shortest path from $u$ to $v$ going through two landmarks $x_i \in L^\prime_{out}(u)$ and $y_j \in L^\prime_{in}(v)$.
%In this sense,
It is not hard to see that each $\mathcal{C}(O_{u,x_i}, O_{y_j,v})$ at most contains one vertex pair.


Further, we assign a unit cost to each object, i.e., $w(O_{u,x})=1$.
Then, if we can find a set of objects $Q^\prime \subseteq Q$ such that $\mathcal{C}(Q^\prime)$ covers the ground set,
we are able to recover all shortest path for any pair of reachable vertices in the graph.
Therefore, the union of landmark indices $\cup_{u\in V} (L^e_{out}(u) \cup L^e_{in}(u))$ is the exact landmarks with smallest local landmark index size.
By applying the best available algorithm for SCP proposed in~\cite{HS05}, we obtains a $O(\sqrt{N\log N})$ approximation ratio to exact landmark set discovery problem,
where $N$ is the cardinality of the ground set $N=|U|$, for the cardinality SCP problem.


However, in our problem setting, the ground set is $U=TC(G)$ and $N=|TC(G)|$, which in the worst case is $\frac{n(n-1)}{2}$.
Thus, the approximation bound is $O(n\sqrt{\log n})$, which is meaningless.
Furthermore, without any prior knowledge, any vertex can be candidate of landmarks, in order to construct the set-cover-with-pair instance,
we need to precompute and explicitly record the distance and shortest path between any pair of vertices.
Both running time and memory cost are prohibitively expensive for most of graphs.
}












\comment{
For the traditional landmark indexing, each vertex $u$ in directed graph is assigned with two lists $L_{out}(u)=(<d(u,v_1),SP_{u,v_1}>,<d(u,v_2),SP_{u,v_2}>,...,<d(u,v_k),SP_{u,v_k}>)$ and
$L_{in}(u)=(<d(v_1,u),SP_{v_1,u}>,<d(v_2,u),SP_{v_2,u}>,...,<d(v_k,u),SP_{v_k,u}>)$.
Note that, if some landmarks are not reachable from (or cannot reach) specific vertex, the corresponding distance and shortest path is set to be null.

All landmark selection strategies are motivated by the important observation:
for one vertex pair $u$ and $v$, if there exists one of shortest path between them going through one of landmarks, this shortest path can be recovered by these landmarks.
The ideal landmark set, refer to as {\em landmark cover}, are able to recover exact shortest path for any pair of vertices in the graph.
Although it is computationally intractable, most of landmark selection heuristics are still proposed to target this goal by utilizing graph's underlying properties.
In this section, we focus on investigating the essence of landmark cover which is able to guide us to the practical landmark selection.
Especially, we first describe a new landmark indexing scheme resulting in much compact index size compared to traditional landmark indices.
We formally define the optimal landmark cover discovery problem based on this indexing scheme, and show that this problem is NP-hard.
To address it, we propose an effective algorithm based on set-cover-with-pair (SCP) framework to discover landmark cover with logarithmic bound.

\subsection{Notation}
\label{notation}

To facilitate our discussion, we begin with defining some nation and terminology used in the rest of paper.
Let $G=(V,E)$ be an unweighted and directed graph where $V=\{1,2,...n\}$ is the vertex set and $E \subseteq V \times V$ is edge set.
The edge from vertex $u$ and $v$ is denoted by $(u,v)$, and we use $P_{v_0, v_p} = (v_0, v_1, ..., v_p)$ to denote a simple path from $v_0$ to $v_p$.
The length of a simple path in unweighted graph is the number of edges in the path.
Given two vertices $u$ and $v$, their shortest path $SP_{u,v}$ is the path between them with minimal length.
The distance from vertex $u$ to $v$ is the length of shortest path $SP_{u,v}$ from $u$ to $v$, denoted by $d(u,v)$.
For each vertex $u$, its $\epsilon$-neighbors, denoted as $N_{\epsilon}(u)$ is a set of vertices such that their distance to $u$ is no greater than $\epsilon$, i.e., $N_{\epsilon}(u) = \{v \in V | 0 < d(u,v) \le \epsilon\}$.

Suppose a subset of vertices $V^\ast=\{v_1,v_2,...,v_k\} \subseteq V$ has been selected as landmarks.
For the traditional landmark indexing, each vertex $u$ in directed graph is assigned with two lists $L_{out}(u)=(<d(u,v_1),SP_{u,v_1}>,<d(u,v_2),SP_{u,v_2}>,...,<d(u,v_k),SP_{u,v_k}>)$ and
$L_{in}(u)=(<d(v_1,u),SP_{v_1,u}>,<d(v_2,u),SP_{v_2,u}>,...,<d(v_k,u),SP_{v_k,u}>)$.
Note that, if some landmarks are not reachable from (or cannot reach) specific vertex, the corresponding distance and shortest path is set to be null.

For any vertex pair $(s,t)$, the traditional landmark scheme approximate the shortest path by concatenating shortest paths $SP_{s,v^\prime}$ and $SP_{v^\prime,t}$ where $v^\prime \in V^\ast$ achieves minimal $d(s,v^\prime)+d(v^\prime,t)$.
Clearly, if $v^\prime$ lies in one of shortest path from $s$ to $t$, the estimated shortest path is exact one.
In ideal situation, for any vertex pair $(s,t)$, we can always find a landmark $x$ from landmark set $V^\ast$ such that $d(s,v)+d(v,t)=d(s,t)$.
We refer to such landmark set as {\em landmark cover}.
%That is, there always exists a landmark from {\em landmark cover} appearing in one of shortest paths from $s$ to $t$.
Furthermore, 2hop labels are essentially a {\em landmark cover},
because for any pair of vertices, there always exists one common vertex in their corresponding label such that at least one of their shortest paths goes through it.
These common vertices serves as {\em landmark cover} in our scenario.

\comment{
Here, we formally define the {\em landmark cover} and {\em optimal landmark cover discovery problem} based above indexing scheme as follows:

\bdefin{\bf (Landmark Cover)}
Given unweighted and directed graph $G=(V,E)$, and a subset of vertices $V^\ast \subseteq V$, we say $V^\ast$ is a landmark cover if and only for any vertex pair $(s,t)$,
there exists a landmark $v \in V^\ast$
\edefin

\bdefin{(\bf (Optimal Landmark Cover Discovery Problem)}
Given unweighted and directed graph $G=(V,E)$, we would like to seek a landmark cover with smallest number of vertices.
\edefin
}

\begin{figure}
\centering
\begin{tabular}{c}
\psfig{figure=Figures/indexexample.eps,scale=0.65}
\end {tabular}
\caption {Indexing Example}
\label{fig:indexexample}
\end{figure}



\subsection{New Landmark Indexing Scheme}
\label{landmarkindex}

Considering a traditional landmark cover $V^\ast$ with $k$ landmarks, each vertex is required to explicitly maintain two $k$-element lists for the shortest path to (from) all landmarks.
Given a graph $G=(V,E)$, the total index size is clearly $2k|V|$.
However, we observe that many unnecessary landmarks are recorded for each specific vertex pair when one of their shortest paths goes through several landmarks.
%This is essentially caused by the query procedure which needs to find out a exact intermediate vertex in the shortest path.
%Simply speaking, the shortest path is expressed as two segments: the path from source to intermediate and the path from intermediate to destination.
In order to gain more compact index size,
we represent each shortest path as three segments instead of two segments in traditional methods: 1) the path from source to appropriate landmark close to it; 2) the path from current landmark to another landmark close to destination;
3) and the path between destination and above nearby landmarks.

We note that the functionality of these landmarks in this scenario is analogous to the highway entrances or exits of transportation network.
In order to find the shortest path from starting point to destination, one simply find the shortest path from starting to the appropriate entrance of highway,
and then get off the correct exit of highway which leads to the remaining shortest path to the destination.
Based on 3-segment expression, for any pair of vertices $(s,t)$, if there are many landmarks from one landmark cover appear in one of shortest path,
both $s$ and $t$ only need to store the {\em essential} landmark, i.e., the nearest one.
To facilitate the exact shortest path query, the middle segment connecting two landmarks are required to be available during online query.
As we discussed in section~\ref{contribution}, the landmark size is rather small and the shortest path among them is almost constant (no more than 3 in large social network),
thus the benefit from index size reduction would easily pay off the cost of materializing pairwise shortest path among landmarks.
This materialization essentially serves as {\em shortest path oracle} which is able to answer shortest path queries between any two landmarks in constant time.


\begin{example}
Figure~\ref{fig:indexexample} shows two different indexing schemes for vertex pair $(s,t)$ given that $3$ landmarks $v_1$, $v_2$ and $v_3$ appear in one of shortest path between them.
As we can see from traditional indexing, the shortest paths from $s$ to all landmarks and from landmarks to $t$ are all recorded.
According to 3-segment representation of shortest path, we only need to record one nearest landmark for each vertex, i.e., $v_1$ for source $s$ and $v_3$ for destination $t$.
The traditional landmark index size is reduced from $6$ to $2$.
Given the shortest path from $v_1$ to $v_3$, the shortest path $SP_{st}$ is easily recovered by $SP_{sv_1}+SP_{v_1 v_3}+SP_{v_3 t}$.
\end{example}


Our new landmark indexing scheme assigns each vertex $u$ two lists, $L^\prime_{out}(u)$ and $L^\prime_{in}(u)$.
$L^\prime_{out}(u)$ records the {\em essential} list of landmarks which is reachable from $u$, including their respective distance and shortest path,
i.e., $L^\prime_{out}(u)=(<x_1:d_{x_1},SP_{x_1}>,...,<x_p:d_{x_p},SP_{x_p}>)$, where $d_{x_i}=d(u,x_i)$ and $SP_{x_i} = SP_{u x_i}$.
Similarly, $L^\prime_{in}(u)$ records the {\em essential} list of landmarks which can reach $u$, including their respective distance and shortest path,
i.e., $L^\prime_{in}(u)=(<y_1:d_{y_1},SP_{y_1}>,...,<y_p:d_{y_p},SP_{y_q}>)$, where $d_{y_i}=d(y_i,u)$ and $SP_{y_i} = SP_{y_i u}$.
Both $x_i$ ($1 \le i \le p$) and $y_j$ ($1 \le j \le q$) are landmarks.
Given a shortest path query $(s,t)$, let $x_i \in L^\prime_{out}(s)$ and $y_i \in L^\prime_{in}(t)$.
We define the {\em landmark distance} from $s$ to $t$:
\beqnarr
d(s,t|L^\prime_{out}(s),L^\prime_{in}(t)) =  \nonumber \\
min_{x_i \in L^\prime_{out}(s), y_j \in L^\prime_{in}(t)} d(s,x_i)+d(x_i,y_j)+d(y_j,t) \nonumber
\eeqnarr
Corresponding {\em landmark shortest path} is the concatenation of $SP_{s x_i}$, $SP_{x_i y_j}$ and $SP_{y_j t}$.
Note that, the pairwise distance and shortest path among landmarks $d_(x_i y_j)$ and $SP_{x_i y_j}$ are materialized.
In addition, the index size is defined to be $\sum_{u \in V} (|L^\prime_{out}(u)| + |L^\prime_{in}(u)|)$.

If {\em landmark distance} by landmark set $V^\ast$ is exactly shortest distance for any pair of vertices,
we refer to $V^\ast$ as {\em landmark cover} in this setting.
Formally, we define {\em landmark cover} and {\em optimal landmark cover discovery problem} based new indexing scheme as follows:

\bdefin{\bf (Landmark Cover)}
Given unweighted and directed graph $G=(V,E)$, and a subset of vertices $V^\ast \subseteq V$, we say $V^\ast$ is a landmark cover if and only for any vertex pair $(s,t)$,
there exists two landmarks $x, y \in V^\ast$ such that $d(s,x)+d(x,y)+d(y,t)=d(s,t)$.
That is, there always exists two landmarks appearing in one of shortest paths from $s$ to $t$.
\edefin

When $x$ is the same with $y$, the landmark cover based on new indexing scheme is degraded to the one based on traditional indexing scheme,
which is also equivalent to the aforementioned 2-hop labels.

\bdefin{(\bf (Optimal Landmark Cover Discovery Problem)}
Given unweighted and directed graph $G=(V,E)$, we would like to seek a landmark cover such that its total index size based on new indexing scheme
$\sum_{u \in V} (|L^\prime_{out}(u)| + |L^\prime_{in}(u)|)$ is minimized.
\edefin


Since 2hop labeling problem can be treated as special case of Optimal Landmark Cover Discovery Problem, where two landmarks that serve as meeting point become only one.
we can easily derive following result:

\bthm
Given unweighted and directed graph $G=(V,E)$, Optimal Landmark Cover Discovery Problem is NP-hard problem.
\ethm

}



==> Landmark.tex <==
\section{Hub$^{\textstyle 2}$-Labeling Framework}
\label{framework}

In this section, we overview the Hub$^2$-Labeling framework and discuss the selection of {\em hub-set}. 
To facilitate our discussion, we introduce the following notation. 
Let $G=(V,E)$ be an undirected graph where $V=\{1,2,...n\}$ is the vertex set and $E \subseteq V \times V$ is the edge set.
The edge from vertex $u$ and $v$ is denoted by $(u,v)$, and we use $P(v_0, v_p) = (v_0, v_1, ..., v_p)$ to denote a simple path between $v_0$ and $v_p$.
The length of a simple path is the number of edges in the path, denoted by $|P(v_0,v_p)|$.
Given two vertices $u$ and $v$, their shortest path $SP(u,v)$ is the path between them with the minimal length.
The distance from vertex $u$ to $v$ is the length of shortest path $SP(u,v)$ between $u$ and $v$, denoted by $d(u,v)$.

To compute the $k$-degree shortest-path in large social network, we develop three new and complementary techniques, {\em Hub$^2$}, {\em Hub-Labeling}, and  {\em Hub-avoidance Bidirectional BFS} (HBBFS). 
They work in harmony and form the Hub$^{2}$-Labeling approach. 

\benum
\item({\bf Hub-Set and Hub$^2$})  A set of vertices, referred to as the {\em hub-set} ($\mathcal{H}$),  are selected from the original graph and their pair-wise distance matrix (referred to as   Hub$^2$) along with the corresponding shortest paths are precomputed and stored in the main memory. The vertices in hub-set have similar functionality to the landmarks, which aim to maximally {\em cover} the shortest paths in the graph (a shortest path is covered by the hub-set if it consists of at least one vertex in the hub-set). However, the size of hub-set is much larger than the number of landmarks: the latter is maximally in the order of tens or hundreds since each vertex in the original graph need to record their distance to the landmarks. Here, the size of the hub-set is constrained by the size of distance matrix (Hub$^2$) since it needs to be held in the main memory. However, nowadays a desktop computer with moderate memory size can easily hold a hub-set with  $10K$ (or more) of vertices. 

\item({\bf Hub-Labeling}) Each vertex $v$ in the graph records only a small portion of hub-set ($L_H(v) \subseteq \mathcal{H}$), referred to as the {\em core-hubs}, along with the distances and the corresponding shortest path. Unlike the landmarking method, where each vertex needs to record their distance to all the landmarks, the hub-labeling in some sense is more close to the $2$-hop labeling as each vertex can record different core-hubs. 
Since the number of core-hubs is much smaller than the cardinality of the entire hub-set (no more than $2\%$ of $|H|$ in the real social networks), the index size scales almost linearly with respect to the graph size (the number of vertices). 
Furthermore, a pairwise computation between each vertex in $L_H(s)$ and each vertex in $L_H(t)$ can be quickly performed to estimate the upper-bound between the distance from $s$ to $t$. 

\item({\bf Hub-avoidance Bidirectional BFS (HBBFS)}) A bidirectional BFS from $s$ and $t$ is performed and the search step is constrained by the minimum between $k$ (for $k$-degree shortest path) and the distance upper-bound computed using the hub-labeling. In particular, none of the vertices in the hub-set $\mathcal{H}$ need to be expanded during the bidirectional search. 
Thus, if the hub-set contains the high-degree vertices, then the bidirectional BFS search can effectively prune the search space.
\eenum 


In the following, we provide an in-depth discussion of the hub-set and core-hubs by comparing them with the classical landmark approach. Especially, we will discuss why we can afford a large hub-set and why the hub-set (along with the distance matrix, hub$^2$) and core-hubs can provide more accurate estimation than the landmark approach (even assuming every vertex records their distance to each vertex in the hub-set). 


\subsection{Hub-Set, Hub$^{\bf 2}$, and Core-Hubs} 
The hub-set $\mathcal{H}$ contains a subset of vertices $\mathcal{H}=\{h_1,h_2,...,h_D\} \subseteq V$. 
(In next section, we will discuss how we select the vertices in hub-set.)
Further, to facilitate our discussion,  we also assume each vertex $h$ in the hub-set can be also considered as a landmark.
Given this, using the traditional landmark index, each vertex $v$ in the original graph records their distance to every landmark $h$ in $\mathcal{H}$. 
To compute the actual shortest path,  we may also record the corresponding shortest path from each vertex $v$ to landmark  $h$.  
Thus, in the traditional landmark approach, each vertex $v$ is indexed by a $D$-dimensional vector:
{\small
\beqnarr
L(v)  = (<h_1: d(h_1,v),SP(h_1,v)>,\cdots,<h_D: d(h_D,v),SP(h_D,v)>)  \nonumber
\eeqnarr
}
Given a vertex pair $(s,t)$, based on the traditional landmark approach, the distance $d(s,t|\mathcal{H})$ and corresponding shortest path $SP(s,t|\mathcal{H})$ can be approximated as:
\beqnarr
d(s,t|\mathcal{H}) &=& min_{h \in \mathcal{H}} \{d(s,h)+d(h,t) \} \nonumber \\
SP(s,t|\mathcal{H}) &=& SP(s,h^\ast) \circ SP(h^\ast,t) \nonumber,  \nonumber \\
\text{ where } h^\ast &=& \underset{h \in L}{\operatorname{argmin}} \{d(s,h)+d(h,t)\} \nonumber
\eeqnarr
Here, $\circ$ is the concatenation operator for two paths by connecting first path's ending node and second path's starting node. Also, $d(s,t|\mathcal{H})=|SP(s,t|\mathcal{H})|$. 

Note that the total index size for the landmark approach is $O(|V| \times |\mathcal{H}|)$. 
Clearly, to hold the index in the main memory, for a graph with millions of vertices, the number of landmark vertices has to be relatively small (in the order of tens or a few hundreds). 
However, in the new Hub$^{2}$-Labeling approach, we can afford to utilize a much larger number of hub-set vertices (or landmarks). 
To achieve that, the Hub$^{2}$-Labeling approach materializes the distance-matrix (Hub$^2$) between vertices in the hub-set and more important, introduces the concept of {\em core-hubs}. 

\bdefin{\bf (Core-Hubs)}
Given graph $G=(V,E)$ and the hub-set $\mathcal{H} \subseteq V$, for each vertex $v$,
we say vertex $h \in \mathcal{H}$ is a core-hub for $v$ (denoted as $L_{H}(v)$)
if there is no other $h^\prime \in \mathcal{H}$ such that $d(v,h)=d(v,h^\prime)+d(h^\prime,h)$.
Formally, $L_H(v)=\{h \in \mathcal{H}: \nexists h^\prime \in \mathcal{H}, d(v,h)=d(v,h^\prime)+d(h^\prime,h)\}$. 
\edefin

\begin{figure}
\centering
\begin{tabular}{c}
\psfig{figure=Figures/coreindexexample.eps,scale=0.65}
\end {tabular}
\caption{Examples of Hub-Set, Hub$^2$, and Core-Hubs}
\label{fig:coreindexexample}
\end{figure}

\begin{example}
Simply speaking, if no other vertex $h^\prime$ appear in any shortest path between $v$ and $h$, $h$ is $v$'s core-hub. 
Figure~\ref{fig:coreindexexample} illustrates the core-hubs for the given hub-set $\{3,5,8\}$. 
%(we omit the distance and shortest path in indices for simplification).
Vertex $1$ only needs to record landmark $3$ in $L_{H}(1)$ since there are shortest path $(1,3,5)$ and $(1,3,8)$ passing through $3$ to reach landmarks $5$ and $8$.
However, there are unique shortest paths between vertex $10$ and all three landmarks, thus $L_H(10)$ should record all of them.
\end{example}

Using the core-hubs  ($L_H$) and distance-matrix (Hub$^2$) on the hub-set, we can approximate the distance and the shortest path for vertex pair $(s,t)$ in the following fashion: 
\beqnarr
\label{corepath}
d_H(s,t|\mathcal{H}) = min_{x \in L_{H}(s) \wedge y \in L_{H}(t)} \{ d(s,x)+d(x,y)+d(y,t) \}  \nonumber \\
SP_H(s,t|\mathcal{H}) = SP(s,x^\ast) \circ SP(x^\ast,y^\ast) \circ SP(y^\ast,t)  \nonumber  \\
\text{ where } x^\ast = \underset{x \in L_H(s) \wedge y \in L_{H}(t)}{\operatorname{argmin}} d(s,x)+d(x,y)+d(y,t) \nonumber
\eeqnarr
Here, $d(x,y)$ ($SP(x,y)$) is the exact distance (shortest path) recorded in the distance-matrix Hub$^2$. 

\noindent{\bf Index Size:}
The over index size of Hub$^2$-Labeling is the sum of the size of distance-matrix (Hub$^2$) together with the core-hub labeling for each vertex ($L_H(v)$): $\sum_{v \in V} O(|L_{H}(v)|\times k) + O(|\mathcal{H}|^2\times k )$, where $k$ is the longest shortest path needs to be stored  in order to answer the $k$-degree shortest path. 
Since $k$ is quite small (no greater than $6$ in general), we can treat it as a constant. 
Thus, the overall index size is $\sum_{v \in V} O(|L_{H}(v)|) + O(|\mathcal{H}|^2)$. 
In the experimental study, we found that for most of the real social networks, the core-hubs of each vertex $v$ is only a small portion of the hub-set (in most case, less than or close to $2\%$). 
Therefore, the  Hub$^2$-Labeling can easily utilize more than $10K$ of landmarks (hub-set vertices). 
Furthermore, since the second term (the size of the distance matrix) is stable, as the number of vertices increases in the original graph, the first term will scale linearly with respect to $|V|$. 


\begin{example}
Now, let us take the Flicker as an example  network we used in experiments as example to get in-depth understanding.
The network contains around $9.4$ millions vertices and $222$ millions edges and we select $10K$ highest degree vertices as landmarks.
Using core landmark indexing scheme, each vertex only needs to record around $180$ landmarks (i.e., no more than $2\%$ of entire landmarks), and total number of entries for pairwise shortest paths among landmarks is at most $100$ millions.
Distributing materialization cost of shortest paths among landmark to each vertex, each vertex at most needs to record around $190$ ($=180+\frac{100M}{9.4M}$) entries, which is still significantly smaller than $10K$ in traditional landmark indexing scheme.
\end{example}

\comment{
Utilizing core landmark indexing, the capacity of $10K$ landmarks is preserved at the expense of index cost equivalent to that using $190$ landmarks.
As we know, the average index cost for each vertex is $\frac{\sum_{u \in V \setminus L} |L_{H}(u)| }{|V|} + \frac{|L|\times |L|}{|V|}$.
Intuitively, as graph size increases, the second term would be much smaller,
and core landmark indexing would bring more benefit regarding index size compared to traditional one.}

\noindent{\bf Advantage over Landmark:} 
In the following, we introduce the following the key observation on the new estimation approach based on the hub-set, hub$^2$, and core-hubs. 
We compare its estimation accuracy with the traditional landmark approach (assuming it can utilizes all the vertices in the hub-set as the landmarks) but with the distance matrix hub$^2$. 

\begin{figure}
\centering
\begin{tabular}{c}
\psfig{figure=Figures/proofcases.eps,scale=0.65}
\end {tabular}
\caption {Cases in proof of Lemma~\ref{goodcorepath}}
\label{fig:proofcases}
\end{figure}

\blemma
\label{goodcorepath}
Given a set of landmarks $L \in V$ in the graph $G=(V,E)$,
the shortest path estimated by using core landmark indexing is not longer than the one obtained by using traditional landmark indexing scheme,
i.e., $d_H(s,t|L) \le d(s,t|L)$ for any reachable vertex pair $(s,t)$.
\elemma

\bproof
Without loss of generality, we want to prove that, for any path generated by traditional landmark indexing, we can find one path no longer that that using core landmark indexing.
Considering reachable vertex pair $(s,t)$, let us denote one path obtained by traditional landmark indexing to be $SP(s,x) \circ SP(x,t)$,
where $x$ is one intermediate landmark between $s$ and $t$.
Now, we seek one path based on core landmark indexing which is not longer than $SP(s,x) \circ SP(x,t)$ in the following cases:

\noindent 1) $x \in L_{H}(s)$ and $x \in L_{H}(t)$. It is trivial to generate the same path $SP(s,x) \circ SP(x,t)$.

\noindent 2) $x \in L_{H}(s)$ and $x \notin L_{H}(t)$.
According to the definition of {\em core landmarks}, there is some landmark $y \in L_{H}(t)$ lying on the shortest path between $x$ and $t$, i.e., $d(x,t)=d(x,y)+d(y,t)$ (case $2$ shown in Figure~\ref{fig:proofcases}).
Since the shortest path $SP(x,y)$ has been materialized beforehand, we can obtain the path $SP(s,x) \circ SP(x,y) \circ SP(y,t)$ with the same length as $SP(s,x) \circ SP(x,t)$.

\noindent 3) $x \notin L_{H}(s)$ and $x \in L_{H}(t)$. Follow the similar logic in case 2 (case 3 in Figure~\ref{fig:proofcases}).
We guarantee to have $y \in L_{H}(s)$ appearing in $SP(s,x)$.
Thus, we have path $SP(s,y) \circ SP(y,x) \circ SP(x,t)$ which is no longer than $SP(s,x) \circ SP(x,t)$.

\noindent 4) $x \notin L_{H}(s)$ and $x \notin L_{H}(t)$. That is, there are some other landmarks $y_1 \in L_{H}(s)$ and $y_2 \in L_{H}(t)$ appearing in shortest paths $SP(s,x)$ and $SP(x,t)$, respectively (case 4 shown in Figure~\ref{fig:proofcases}).
According to triangle inequality, we have $d(y_1,x) + d(x,y_2) \ge d(y_1,y_2)$.
Also, shortest path $SP(y_1,y_2)$ has been precomputed before,
thus we can have the path $SP(s,y_1) \circ SP(y_1,y_2) \circ SP(y_2,t)$ which guarantees to be no longer than $SP(s,x) \circ SP(x,t)$.

Therefore, in any case, the lemma follows.
\eproof


\subsection{Core Landmark Selection}
\label{landmarkselection}

In the previous subsections, we assume that landmarks are given.
Here, we consider how to select a set of good landmarks which are able to greatly preserve pairwise shortest path information.
%In this subsection, we study the problem: {\em how to select good core landmarks to accurately estimate the shortest path?}
%As we know, landmark selection strategies greatly influence the estimation accuracy and performance of query processing.
In ideal case, we wish landmarks are able to perfectly approximate the shortest path for any reachable vertex pair, i.e., estimated shortest path is {\em exact shortest path}.
Additionally, the efficiency of query processing relies on the average number of landmarks each vertex needs to record,
such that estimating the shortest path of vertex pair $(s,t)$ basically requires $|L_H(s)| \times |L_{H}(t)|$ times pairwise computation.
Therefore, smallest number of landmarks encapsulating maximum shortest path information naturally becomes the goal of landmark selection.
We first define the following concept to evaluate a set of landmarks' ability:
%all exiting landmark selection strategies based on traditional indexing scheme target at finding the smallest number of landmarks which can recover all shortest path, although it is computational intractable.

\bdefin{\bf (Core Landmark Coverage)}
Given core landmarks $L$ and vertex pair $(s,t)$, if the estimated shortest distance using core landmark indexing scheme is {\em exact} distance (i.e., $d(s,t)=min_{x \in L_{H}(s) \wedge y \in L_{H}(t)} (d(s,x)+d(x,y)+d(y,t))$),
we say vertex pair $(s,t)$ is covered by core landmarks $L$.
\edefin

This motivates our problem definition of optimal core landmark selection:

\bdefin{\bf (Optimal Core Landmark Selection Problem)}
Given an unweighted and directed graph $G=(V,E)$, optimal landmark selection problem tries to find minimum number of landmarks $L \in V$,
such that $L$ is able to cover any reachable vertex pair $(s,t) \in V \times V$.
\edefin

We build an interesting connections between optimal core landmark selection problem and landmark-cover problem stated in~\cite{Potamias:2009:FSP:1645953.1646063}, which aims at finding a minimum number landmarks to recover any vertex pair using traditional landmark indices.

\blemma
\label{equal}
Optimal core landmark selection problem is equivalent to landmark-cover problem~\cite{Potamias:2009:FSP:1645953.1646063}.
\elemma
\bproof
Let us use $L$ to denote the optimal solution for landmark cover problem, and use $L_H$ to the solution for optimal core landmark selection problem.
On the one hand, given landmarks $L_H$, for any vertex pair $(s,t)$, if we can find two landmarks $x,y \in L_H$ to cover it (i.e., $d(s,t)=d(s,x)+d(x,y)+d(y,t)$, $x \in L_{H}(s)$ and $y \in L_{H}(t)$),
we are also able to restore their distance using one of landmarks based on traditional indexing scheme (i.e., $d(s,t)=d(s,x)+d(x,t)$ and $x \in L(s)$).
In other words, $L_H$ is a feasible solution for landmark cover problem.
Therefore, $|L_H| \ge |L|$.

On the other hand, given landmarks $L$, according to lemma~\ref{goodcorepath},
we are able to assign each vertex $u$ indices $L_{H}(u) \subseteq L$.
These core landmark indices are sufficient to recover shortest paths of all vertex pairs that can be recovered by $L$ based on traditional landmark indexing scheme.
Therefore, $\cup_{u \in V \setminus L} L_{H}(u)  \subseteq L$ is a feasible solution for optimal core landmark selection problem.
Moreover, since $L_H$ is optimal solution, meaning $|\cup_{u \in V \setminus L} L_{H}(u)| \ge |L_H|$,
thus $|L_H| \le |L|$.

Putting both together, we have $|L|=|L_H|$ following the statement in the lemma.
\eproof

Since landmark cover problem~\cite{Potamias:2009:FSP:1645953.1646063} has been proved to be NP-hard, we easily establish following result:

\blemma
Optimal core landmark selection problem is NP-hard.
\elemma

Due to the hardness of optimal core landmark selection, we consider an variant by fixing the number of landmarks.
This is more practical in many applications with limited memory resource,
because the number of landmarks $K$ indeed offers a upper bound for landmark indexing size, i.e., $K \times |V|$.
In addition, by changing the number of landmarks, we are able to trade off landmark index size and query performance.
We will empirically study this trade-off in the experimental evaluation.


\bdefin{\bf (Optimal $K$ Core Landmark Selection Problem)}
Given an unweighted and directed graph $G=(V,E)$, we try to find $L \in V$,
such that $|L|=K$ and  the number of vertex pairs $(s,t) \in V \times V$ covered by $L$ is maximized.
\edefin

Following the similar idea in the proof of lemma~\ref{equal}, our optimal $K$ core landmark selection problem is also equivalent to $Landmark_d$ problem in~\cite{Potamias:2009:FSP:1645953.1646063}, which is still NP-hard.
In this case, we need to select landmarks in a more practical and efficient manner for massive social networks.

We start from most simple scenario to gain a better intuition of good landmarks in social networks.
Intuitively, the best landmark should be the one in the very {\em central} position of graph~\cite{Potamias:2009:FSP:1645953.1646063}.
This high-level understanding suggests two concepts of {\em central} vertex (i.e., landmark) from different perspectives:
1) it is a vertex lying on many shortest paths, which can be measured by vertex betweenness centrality;
2) it is a vertex close to other vertices in the graph, which can be measured by closeness centrality.
In the optimized scenario, the best {\em central} vertex based on first concept is referred to as the vertex with largest vertex betweenness~\cite{citeulike:1025135},
while second one refers to the vertex with optimal closeness centrality.
We generalize both concepts to $K$ landmarks selections in social networks.

%To be self-contained, we rephrase both definitions first.
\noindent{\bf Vertex Betweenness Criterion: }
The vertex betweenness firstly introduced by Freeman~\cite{citeulike:1025135} in the context of social science:
\[  C_B(v) = \sum_{u,w \in V \wedge u\neq w \neq v} \frac{\sigma_{uw}(v)}{\sigma_{uw}} \]
where $\sigma_{uw}(v)$ is the total number of shortest path between $u$ and $w$ that pass through $v$,
and $\sigma_{uw}$ is the total number of shortest path between $u$ and $w$.

We sort all vertices based on their vertex betweenness centrality in descending order and pick top $K$ vertices as landmarks.
To achieve this goal, we need to precompute vertex betweenness centrality for every vertex.
However, to our knowledge, the fastest algorithm to compute every vertex betweenness centrality in unweighted and directed graph is $O(|V||E|)$~\cite{Brandes2001}, which is still rather expensive for massive networks.

\noindent{\bf Closeness Betweenness Criterion: }
The closeness of a vertex is evaluated by the inverse of its total distance to all other vertices in the graph~\cite{citeulike:7062391}.
The vertex is the more central the lower its total distance to the remaining vertices. That is,
\[ C_C(v) = \frac{|V|-1}{ \sum_{u \in V \wedge u \neq v} d(v,u) }  \]

The intuition of using this criterion is that, a vertex closer to all other vertices are very likely to part of many shortest paths.
Therefore, we select top $K$ vertices with largest closeness centrality to be landmarks.
Analogous to computing vertex betweenness, calculating closeness betweenness involving pairwise shortest paths computation is an expensive task,
taking $O(|V|(|V|+|E|))$ time in unweighted graph setting.

Although it is costly to select $K$ landmarks strictly following aforementioned criteria,
we are able to adopt the vertices with high vertex degree as their effective proxies in social networks.
This is based on key observations on how high-degree vertices contribute social networks' connectivity and small path length.
The empirical study on several well-known social networks (i.e., Flickr, LiveJournal, Orkut and Youtube) reported in~\cite{Mislove07}
clearly demonstrates the presence of densely connected {\em core} comprising of a small portion of vertices with highest degree.
The removal of this {\em core} dramatically disconnects entire graph, implying that most of pairwise connections rely on few high-degree vertices.
In other words, few high degree vertices serve as key intermediates in most of shortest paths, thus are qualified to be landmarks under vertex betweenness criterion.

In addition, they also analyze the average shortest path length in the core containing only highest-degree vertices.
As core grows, the average shortest path length increases sub-logarithmically.
Since average shortest path length of entire graph is very small, this phenomenon suggests that the lower degree vertices that constitute the majority of the network are very close to the high degree vertices in the core.
In this sense, high-degree vertices are also qualified to be landmarks under closeness betweenness criterion.

\subsection{Efficient Indexing Procedure}
\label{indexingalgo}

In this subsection, we present an efficient algorithm to assign each vertex $u$ its core landmarks $L_{H}(u)$.
Recall that our goal is to compute the shortest path with length no greater than $6$.
For any vertex pair $(s,t)$, the landmark $x$ that is $6$ hops away from both of them is unlikely to offer effective estimation,
because the upper bound $d(s,x)+d(x,t)$ ($\ge 12$) is too relaxed to approximate the shortest path length of social networks which is typically small.
Therefore, each vertex only consider landmarks within $6$ hops to be their core landmarks.
We note that such distance-constrained landmark indexing would make lemma~\ref{goodcorepath} infeasible.
However, recall that our overall goal is to utilize landmark indexing to assist in online query answering.
This distance-constrained indexing offers a practical trade-off between the preprocessing cost and online estimation.

Now, we turn back to landmark indexing.
The straightforward solution is to precompute all pairwise distances among landmarks and materialize all distances between landmarks and non-landmarks vertices.
It is not hard to see that each landmark is very likely to be accessed several times.
Since landmarks are all high degree vertices, such multiple access would make indexing unacceptably long.

To tackle the problem, we introduce an efficient procedure which only performs one local breadth-first traversal (BFS) for each landmark to visit its $6$-neighborhood (i.e., the vertex with distance to landmark no more than 6).
Specifically, for each BFS starting from landmark $u$, two tasks have to be completed:
1) it needs to find out all other landmarks whose distance to $u$ is no more than $6$, and record one shortest path between them for query answering;
2) for each visited non-landmark vertex $v$ during BFS, we need to quickly check whether $u$ is $v$'s core landmarks.
This is equivalent to check if there is other landmarks appearing in a shortest path between $u$ and $v$.
The first task can be easily achieved by introducing an extra integer for each vertex, which is used to record the previous vertex on the shortest path from landmark $u$ to current vertex along shortest path.
In order to achieve second task, we utilize a simple observation:
{\em let vertex $y$ lies on one shortest path from landmark $u$ to non-landmark vertex $v$ with distance $d(u,v)-1$ (i.e., $y$ is one hop closer than $v$ with respect to $u$),
if there is a landmark $x$ appearing in one shortest path from $u$ to $y$ ($x$ and $y$ may not be distinct),
$x$ definitely lies on one shortest path from $u$ to $v$ and $u$ cannot be core landmark of $v$.}
Based on this observation, we maintain a binary flag $b(v)$ to denote if there is another landmark appearing in shortest path between $u$ and $v$.
Specifically, $b(v)=1$ if $v$ is landmark or $b(y)=1$ where $d(u,y)=d(u,v)-1$ and $d(y,v)=1$.
During BFS traversal, when we visit each vertex $v$, if its flag $b(v) \neq 1$ meaning there is no other landmark lying on the shortest path between $u$ and $v$, we append $u$ and shortest path $SP(u,v)$ to its $L_{H}(v)$.
Figure~\ref{fig:bfsindexexample} shows an example of landmark mark indexing.
The value attached to each vertex $v$ is its binary flag $b(v)$, such as $b(1)=0$ and $b(2)=1$.


\begin{figure}
\centering
\begin{tabular}{c}
\psfig{figure=Figures/bfsindexexample.eps,scale=0.65}
\end {tabular}
\caption{Example for Core Landmark Indexing (only consider 3 hops)}
\label{fig:bfsindexexample}
\end{figure}



\input{Figures/BFSIndexing.tex}

The outline of BFS-based procedure for generating core landmark indices is described in Algorithm~\ref{alg:bfsindex}.
The flag $b(v)$ for each vertex $v$ is updated when $v$ is landmark or the flag of its previous vertex in $SP(s,v)$ is one (Line 6 and Line 18).
When vertex $u$ is popped from queue and its flag $b(u)=0$, landmark $s$ is assigned to $L_{H}(u)$ (Line 10).
This procedure will be invoked for each landmark.
In total, this procedure takes $O(\sum_{u \in L} (|N_6(u)|+|E_6(u)|))$ time, where $L$ is landmark set, $N_6(u)$ ($E_6(u)$) is the number of vertices (edges) in $u$'s 6-neighborhood.

































%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Given a vertex pair $(s,t)$, if their $L^c_{out}(s)$ and $L^c_{in}(t)$ are able to recover the {\em exact} shortest path,
%this shortest path also can be recovered by using traditional indices $L_{out}(s)$ and $L_{in}(t)$,
%because $L^c_{out}(s) \subseteq L_{out}(s)=Succ(s|L)$ and $L^c_{in}(t) \subseteq L_{in}(t)=Pred(t|L)$.
%Essentially, core landmark indexing is the generalization of traditional landmark indexing,
%because it can not only utilize single landmarks, but also a pair of landmarks to estimate shortest path.

\comment{
\section{Local Landmark Framework}
\label{landmark}

In this section, we describe a new indexing scheme using landmarks to effectively encode the shortest path information.
Given a landmark set, new indexing scheme not only provides much compact indices, but also guarantees the resulting shortest path no long than the one by traditional landmark approach.
We formally define the optimal landmark selection problem based on new indexing scheme.
Then, we show that this problem is NP-hard and propose a greedy solution based on set-cover-with-pair framework to achieve logarithmic approximation.


To facilitate our discussion, we begin with defining some nation and terminology used in the rest of paper.
Let $G=(V,E)$ be an unweighted graph where $V=\{1,2,...n\}$ is the vertex set and $E \subseteq V \times V$ is edge set.
The edge from vertex $u$ and $v$ is denoted by $(u,v)$, and we use $P(v_0, v_p) = (v_0, v_1, ..., v_p)$ to denote a simple path from $v_0$ to $v_p$.
The length of a simple path in unweighted graph is the number of edges in the path.
Given two vertices $u$ and $v$, their shortest path $SP(u,v)$ is the path between them with minimal length.
The distance from vertex $u$ to $v$ is the length of shortest path $SP(u,v)$ from $u$ to $v$, denoted by $d(u,v)$.
For each vertex $u$, its $\epsilon$-neighbors, denoted as $N_{\epsilon}(u)$ is a set of vertices such that their distance to $u$ is no greater than $\epsilon$, i.e., $N_{\epsilon}(u) = \{v \in V | 0 < d(u,v) \le \epsilon\}$.
Given a vertex set $V^\ast$, for each each vertex $u \notin V^\ast$,
$Succ(u|V^\ast)$ is a subset of $V^\ast$ which can be reached from $u$ and $Pred(u|V^\ast)$ is a subset of $V^\ast$ which can reach $u$.
Due to the popularity of directed graphs in social networks, we focus on the undirected and unweighted graphs in the paper.
Taking a undirected graph as a bidirected graph, all techniques discussed in the paper can be easily extended to undirected setting.


\subsection{Global Landmark Indexing}
\label{globalindex}

Given graph $G=(V,E)$, suppose a subset of ordered vertices $V^\ast=\{x_1,x_2,...,x_k\} \subseteq V$ has been selected to be {\em landmarks}.
For each landmark $x_i$, we need to precompute and explicitly store the shortest path to all vertices in the graph $G$.
Then, we distribute these shortest path information to every vertex, such that each vertex $u$ is associated with two vectors:
{\small
\beqnarr
L_{in}(u)  = (<x_1: d(x_1,u),SP(x_1,u)>...,<x_p: d(x_p,u),SP(x_p,u)>)  \nonumber \\
L_{out}(u) = (<y_1: d(u,y_1),SP(u,y_1)>...,<y_q: d(u,y_q),SP(u,y_q)>) \nonumber
\eeqnarr
}
where $x_i \in Pred(u|V^\ast)$ ($1 \le i \le p$) and $y_j \in Succ(u|V^\ast)$ ($1 \le j \le q$).
Since all landmark information are propagated to entire graph, we refer to this traditional indexing scheme as {\em Global Landmark Indexing} scheme.
Given this, for a pair of vertices $s$ and $t$, their {\em landmark distance $d(s,t|V^\ast)$} and {\em landmark shortest path $SP(s,t|V^\ast)$} are defined based on triangle inequality:
{\small
\beqnarr
d(s,t|V^\ast) = min_{x \in L_{out}(s) \cap L_{in}(t)} \{ d(s,x)+d(x,t) \} \nonumber \\
SP(s,t|V^\ast) = SP(s,x^\ast) \circ SP(x^\ast,t) \nonumber \\
 \text{ where } x^\ast = \underset{x \in L_{out}(s) \cap L_{in}(t)}{\operatorname{argmin}} d(s,x)+d(x,t) \nonumber
\eeqnarr
}
where $\circ$ is the concatenation operator for two paths by connecting the first path's ending node and second path's starting node.
Clearly, given landmark set $V^\ast$, the landmark index size of total graph is $\sum_{u \in V} |L_{out}(u)|+|L_{in}(u)| = \sum_{u \in V} |Pred(u|V^\ast)| + |Succ(u|V^\ast)|$.

When landmark distance is equivalent to distance in the graph $G$, the landmark shortest path is actually the exact shortest path for a pair of vertices.
We say a set of vertices are {\em exact landmarks} if the landmark distance of any pair of vertices is exact distance in the graph $G$.
Simply speaking, for any two reachable vertices, there always exists one vertex from {\em exact landmarks} appearing in one of the shortest paths between them.
The problem of discovering exact landmarks with smallest cardinality has been proved to be NP-hard~\cite{Potamias:2009:FSP:1645953.1646063}.
Due to the hardness of selecting exact landmarks, most of existing works concentrate on developing different heuristics utilizing certain graph properties, such as vertex centrality, degree distribution or graph diameter.
Few of them attempt to improve the accuracy from indexing perspective.


\begin{figure}
\centering
\begin{tabular}{c}
\psfig{figure=Figures/indexexample.eps,scale=0.6}
\end {tabular}
\caption {Indexing Example}
\label{fig:indexexample}
\end{figure}

\begin{figure}
\centering
\begin{tabular}{c}
\psfig{figure=Figures/proofcases.eps,scale=0.65}
\end {tabular}
\caption {Cases in proof of Lemma~\ref{localgoodpath}}
\label{fig:proofcases}
\end{figure}



\subsection{Local Landmark Indexing}
\label{localindex}

In global landmark indexing scheme, each vertex is required to explicitly record all shortest distance and shortest path to (from) the landmarks which is reachable (can be reached).
However, we observe that many landmarks are redundant for each specific vertex under certain condition.
More specifically, each vertex only needs to record a subset of {\em essential} landmarks such that on other landmarks appear in the shortest path between them.
Using a slightly modified shortest path computation strategy, the recorded landmarks guarantee to generate a path which is no longer than the one produced by global indexing scheme.
Before we formally introduce new indexing scheme, let us go over a simple example to gain intuitive understanding.

\begin{example}
\label{indexexamp}
Figure~\ref{fig:indexexample} shows a shortest path from $s$ to $t$ while three landmarks $v_1$, $v_2$ and $v_3$ lie in this shortest path.
In global landmark indexing, both outgoing indices of source $s$ and incoming indices of destination $t$ need to record all three landmarks.
If shortest path $SP(v_1,v_3)$ between two landmarks $v_1$ and $v_3$ is known beforehand,
landmark $v_1$ included in $L_{out}(s)$ and landmark $v_3$ included in $L_{in}(t)$ are sufficient to recover the shortest path $SP(s,t)$,
i.e., $SP(s,t)= SP(s,v_1) \circ SP(v_1,v_3) \circ SP(v_3,t)$.
We can see that, the shortest path $SP(v_1,v_3)$ between two landmarks are implicitly recorded twice in $SP(s,v_3)$ and $SP(v_1,t)$,
thus materializing $SP(v_1,v_3)$ does not introduce any extra index cost.
\end{example}

In the example, we actually represent the shortest path $SP(s,t)$ by three segments:
1) $SP(s,v_1)$, from source $s$ to one close landmark $v_1$; 2) $SP(v_1,v_3)$, from landmark $v_1$ to another landmark $v_3$ close to destination $t$;
and 3) $SP(v_3,t)$, from landmark $v_3$ to destination $t$.
To some extent, two intermediate landmarks in the shortest path mimic the highway entrances or exits of transportation network.
In order to find the shortest path from starting point to destination, one simply find the shortest path from starting to the appropriate entrance of highway,
and then get off the correct exit of highway which leads to the remaining shortest path to the destination.
The shortest paths among landmarks serve as {\em shortest path oracle} which can answer the shortest path queries quickly, such as in constant time.

Now, given a landmark set $V^\ast$, we formally define {\em incoming essential landmarks} and {\em outgoing essential landmarks} for each vertex $u$:

\bdefin{\bf (Essential Landmarks)}
Given graph $G=(V,E)$ and a landmark set $V^\ast$, for each vertex $u$, its outgoing essential landmarks $L^e_{out}(u)$ contains landmark $x$,
if there does not exist $x^\prime \in V^\ast$ satisfying $d(u,x)=d(u,x^\prime)+d(x^\prime,x)$.
Simply speaking, no other landmarks appear in one of shortest path from $u$ to $x$.
Similarly, its incoming essential landmarks $L^e_{in}(u)$ contains landmark $y$,
if there is no $y^\prime \in V^\ast$ satisfying $d(y,u)=d(y,y^\prime)+d(y^\prime,u)$.
\edefin

The exclusion of a landmark $x$ in the essential landmarks with respect to vertex $u$ means there exists other landmark appear in the shortest path $SP(u,x)$ and closer to $u$ than $x$.
Recalling example~\ref{indexexamp}, $v_3$ is non-essential for source $s$, since the shortest path from $s$ to $v_3$ can be ``blocked'' by $v_1$.
The {\em incoming essential landmarks} and {\em outgoing essential landmarks} of each vertex constitute the indices of new landmark indexing scheme.
Opposing to global landmark indexing which needs to store all reachable (can be reached) landmarks, we refer to this indexing scheme as {\em local landmark indexing}.
Based on local indexing, we are able to compute its corresponding {\em landmark distance $d^e(s,t|V^\ast)$} and {\em landmark shortest path $SP^e(s,t|V^\ast)$} are defined as:
\beqnarr
d^e(s,t|V^\ast) = min_{x \in L^e_{out}(s) \wedge y \in L^e_{in}(t)} \{ d(s,x)+d(x,y)+d(y,t) \} \nonumber \\
SP^e(s,t|V^\ast) = SP(s,x^\ast) \circ SP(x^\ast,y^\ast) \circ SP(y^\ast,t) \nonumber \\
\text{ where } x^\ast = \underset{x \in L^e_{out}(s) \wedge y \in L^e_{in}(t)}{\operatorname{argmin}} d(s,x)+d(x,y)+d(x,t) \nonumber
\eeqnarr
In this sense, we need to materialize the pairwise shortest path among landmarks.
However, this materialization does not impose burden on the memory cost due to two reasons.
First, the length of shortest path in the social networks we focus on in this work is typically rather small~\cite{Mislove07}.
In our experiments, we observe that the length of most shortest paths between landmarks is no more than 3.
Second, lots of shortest paths between landmarks are implicitly encoded multiple times in global landmark indexing (e.g., Figure~\ref{fig:indexexample}, $SP(v_1,v_3)$ is contained in $SP(s,v_3)$ and $SP(v_1,t)$).

In addition, it is not hard to see that, local landmark indexing is a generalization of global landmark indexing.
In other words, if there is no shortest path from non-landmark vertex to landmark (or from landmark to non-landmark vertex) is ``blocked'' by some landmarks,
local landmark indexing degrades to global landmark indexing.
Hence, the index size of local landmark indexing $\sum_{u \in V} (|L^e_{out}(u)| + |L^e_{in}(u)|)$ is no larger that of global indexing.
More importantly, we have following observation:

\blemma
\label{localgoodpath}
The shortest path generated by local landmark indexing is no longer than the best one generated by global landmark indexing.
\elemma

\bproof
We want to prove that, for any path generated by global landmark indexing, we are able to find a path no longer that it based on local landmark indexing.
Without loss of generality, consider reachable vertex pair $(s,t)$, let us denote one path obtained by global landmark indexing as $SP(s,x) \circ SP(x,t)$,
where $x$ is the intermediate landmark in the path (i.e., $x \in L_{out}(s)$ and $x \in L_{in}(t)$.
Now, we try to find a path based on local landmark indexing which is not longer than $SP(s,x) \circ SP(x,t)$ in the following cases:
%we consider the outgoing indices $L^e_{out}(s)$ of source and incoming indices $L^e_{in}(t)$ of destination with respect to $x$ based on local landmark indexing:

\noindent 1) $x \in L^e_{out}(s)$ and $x \in L^e_{in}(t)$. It is trivial to generate the same path $P(s,x) \circ P(x,t)$.

\noindent 2) $x \in L^e_{out}(s)$ and $x \notin L^e_{in}(t)$. According to the definition of {\em essential landmarks}, there is some landmark $y \in L^e_{in}(t)$ appear in the shortest path from $x$ to $t$, i.e., $d(x,t)=d(x,y)+d(y,t)$ (case $2$ shown in Figure~\ref{fig:proofcases}).
Since the shortest path $SP(x,y)$ from landmark $x$ to $y$ is available beforehand, we are able to generate the path $SP(s,x) \circ SP(x,y) \circ SP(y,t)$ with the same length as $SP(s,x) \circ SP(x,t)$.

\noindent 3) $x \notin L^e_{out}(s)$ and $x \in L^e_{in}(t)$. Follow the similar logic in case 2 (case 3 in Figure~\ref{fig:proofcases}). We guarantee to have $y \in L^e_{out}(s)$ appear in $SP(s,x)$. Thus, we can generate path $SP(s,y) \circ SP(y,x) \circ SP(x,t)$ which is no longer than $SP(s,x) \circ SP(x,t)$.

\noindent 4) $x \notin L^e_{out}(s)$ and $x \notin L^e_{in}(t)$. That is, there are some other landmarks $y_1 \in L^e_{out}(s)$ and $y_2 \in L^e_{in}(t)$ appear in the shortest paths $SP(s,x)$ and $SP(x,t)$, respectively (case 4 shown in Figure~\ref{fig:proofcases}).
Moreover the shortest path $SP(y_1,y_2)$ between landmarks $y_1$ and $y_2$ are known.
Due to triangle inequality $d(y_1,y_2) \le d(y_1,x)+d(x,y_2)$, we are able to generate the shorter path $SP(s,y_1) \circ SP(y_1,y_2) \circ SP(y_2,t)$
compared to $SP(s,x) \circ SP(x,t)$.

Putting those together, in any case, we can find a path based on local landmark indexing no worse than the one generated by global landmark indexing.
Therefore, the statement follows.
\eproof

Local landmark indexing scheme not only provides much compact index size, but also guarantees the resulting shortest path no long than the one by global landmark indexing scheme.
On the other hand, due to the properties of social networks, such as small diameter and massive size,
the desired landmarks should be able to provide exact shortest path using compact index size.
Motivated by this requirement, we formally define the concept of landmark coverage and following exact landmark discovery problem:

\bdefin{\bf (Landmark Coverage)}
Given graph $G=(V,E)$ and landmark set $V^\ast \subseteq V$, for a vertex pair $(s,t)$,
we say $V^\ast$ {\em covers} vertex pair $(s,t)$ if there exists two landmarks $x,y \in V^\ast$ appearing in the shortest path from $s$ to $t$.
Note that, two landmarks may not be distinct, i.e., $x$ may be the same with $y$.
\edefin

\bdefin{\bf (Exact Landmark Set Discovery Problem)}
Given an unweighted and directed graph $G=(V,E)$, the exact landmark set discovery problem tries to find a set of landmarks $V^\ast \in V$
which can cover any pair of reachable vertices and the local landmark index size is minimized.
\edefin

\comment{
\bdefin{\bf (Exact Landmark Set Discovery Problem)}
Given an unweighted and directed graph $G=(V,E)$, the exact landmark set discovery problem tries to find a set of landmarks $V^\ast \in V$,
such that for any pair of reachable vertices $(s,t)$, their corresponding local indices satisfy:
\[ d^e(s,t|V^\ast) = d(s,t) \]
where the local landmark index size is minimized.
\edefin
}


\subsection{Transform to Set-Cover-with-Pairs}
\label{scpsolution}

In this section, we transform the exact landmark set discovery problem to set-cover-with-pair instance.
To be self-contained, we first briefly introduce the set-cover-with-pair problem~\cite{HS05}.

\bdefin{\bf (Set-Cover-with-Pairs Problem ~\cite{HS05})}
Let $U$ be the ground set and let $S = \{1, \ldots, M\}$ be a set of objects, where each object $i\in S$ has a non-negative cost $w_i$.
For every $\{i,j\}\subseteq S$, let $\mathcal{C}(i, j)$ be the collection of elements in $U$ covered by the pair $\{i, j\}$.
The objective of the set cover with pairs (SCP) problem is to find a subset $S^\prime \subseteq S$ such that
$\mathcal{C}(S^\prime) =\bigcup_{\{i,j\}\subseteq S^\prime} \mathcal{C}(i, j) = U$ with a minimum covering cost $\sum_{i\in S} w_i$.
We refer to the special case in which each object has a unit weight ($w_i=1$) as the \textbf{cardinality SCP} problem.
\edefin

Now we transform our exact landmark set discovery problem to the Set-Cover-with-Pairs problem as follows.
Let the ground set $U=TC(G)$, i.e., it contains any vertex pair $(u,v)$ in $G$, such that $u \rightarrow v$.
To cover a pair $(u,v)$ means we can recover one of their shortest paths in the new landmark indexing scheme.

In our directed graph setting, we categorize objects in $Q$ into two types: starting objects $Q^s$ and ending objects $Q^e$ with respect to two endpoints of each shortest path.
Each starting object $O^s_{u,x_i}$ in $Q$ corresponds to a tuple $(u,(x_i: d_{x_i}, SP_{x_i}))$, where $u$ is a starting vertex and $x_i$ is a candidate landmark can be reached from $u$.
Note that, $d_{x_i}= d(u,x_i)$ and $SP_{x_i}=SP(u x_i)$ are shortest distance and one shortest path from $u$ to $x_i$, respectively.
Similarly, each ending object $O^e_{y_j,v}$ in $Q$ corresponds to a tuple $((y_j: d_{y_j}, SP_{y_j}),v)$, where $v$ is ending vertex and $y_j$ is a candidate landmark can reach $v$.
Here, $d_{y_j}= d(y_j,v)$ and $SP_{y_j}=SP(y_j, v)$ are shortest distance and one shortest path from $y_j$ to $v$, respectively.
Now, we define $\mathcal(O_{u,x_i}, O_{y_j,v})$ for each pair of objects $O_{u,x_i}$ and $O(y_j,v)$.
Given any four vertices $(u,x_i,y_j,v)$, if $d(u,x_i)+d(x_i,y_j)+d(y_j,v)=d(u,v)$, then vertex pair $(u,v)$ is covered by objects pair $\{O^s_{u,x_i}, O^e_{y_j,v}\}$.
That is, $\mathcal{C}(O^s_{u,x_i}, O^e_{y_j,v})$ contains vertex pair $(u,v)$.
Otherwise, $\mathcal{C}(O_{u,x}, O_{y,v})=\emptyset$.
Note that, aforementioned four vertices may not be distinct, i.e., $u$ may be the same with $x_i$, $x_i$ may be the same with $y_j$, etc.
%From the viewpoint of restoring shortest paths, that vertex pair $(u,v)$ is covered by objects pair $\{O^s_{u,x_i}, O^e_{y_j,v}\}$ means there exists one shortest path from $u$ to $v$ going through two landmarks $x_i \in L^\prime_{out}(u)$ and $y_j \in L^\prime_{in}(v)$.
%In this sense,
It is not hard to see that each $\mathcal{C}(O_{u,x_i}, O_{y_j,v})$ at most contains one vertex pair.


Further, we assign a unit cost to each object, i.e., $w(O_{u,x})=1$.
Then, if we can find a set of objects $Q^\prime \subseteq Q$ such that $\mathcal{C}(Q^\prime)$ covers the ground set,
we are able to recover all shortest path for any pair of reachable vertices in the graph.
Therefore, the union of landmark indices $\cup_{u\in V} (L^e_{out}(u) \cup L^e_{in}(u))$ is the exact landmarks with smallest local landmark index size.
By applying the best available algorithm for SCP proposed in~\cite{HS05}, we obtains a $O(\sqrt{N\log N})$ approximation ratio to exact landmark set discovery problem,
where $N$ is the cardinality of the ground set $N=|U|$, for the cardinality SCP problem.


However, in our problem setting, the ground set is $U=TC(G)$ and $N=|TC(G)|$, which in the worst case is $\frac{n(n-1)}{2}$.
Thus, the approximation bound is $O(n\sqrt{\log n})$, which is meaningless.
Furthermore, without any prior knowledge, any vertex can be candidate of landmarks, in order to construct the set-cover-with-pair instance,
we need to precompute and explicitly record the distance and shortest path between any pair of vertices.
Both running time and memory cost are prohibitively expensive for most of graphs.
}












\comment{
For the traditional landmark indexing, each vertex $u$ in directed graph is assigned with two lists $L_{out}(u)=(<d(u,v_1),SP_{u,v_1}>,<d(u,v_2),SP_{u,v_2}>,...,<d(u,v_k),SP_{u,v_k}>)$ and
$L_{in}(u)=(<d(v_1,u),SP_{v_1,u}>,<d(v_2,u),SP_{v_2,u}>,...,<d(v_k,u),SP_{v_k,u}>)$.
Note that, if some landmarks are not reachable from (or cannot reach) specific vertex, the corresponding distance and shortest path is set to be null.

All landmark selection strategies are motivated by the important observation:
for one vertex pair $u$ and $v$, if there exists one of shortest path between them going through one of landmarks, this shortest path can be recovered by these landmarks.
The ideal landmark set, refer to as {\em landmark cover}, are able to recover exact shortest path for any pair of vertices in the graph.
Although it is computationally intractable, most of landmark selection heuristics are still proposed to target this goal by utilizing graph's underlying properties.
In this section, we focus on investigating the essence of landmark cover which is able to guide us to the practical landmark selection.
Especially, we first describe a new landmark indexing scheme resulting in much compact index size compared to traditional landmark indices.
We formally define the optimal landmark cover discovery problem based on this indexing scheme, and show that this problem is NP-hard.
To address it, we propose an effective algorithm based on set-cover-with-pair (SCP) framework to discover landmark cover with logarithmic bound.

\subsection{Notation}
\label{notation}

To facilitate our discussion, we begin with defining some nation and terminology used in the rest of paper.
Let $G=(V,E)$ be an unweighted and directed graph where $V=\{1,2,...n\}$ is the vertex set and $E \subseteq V \times V$ is edge set.
The edge from vertex $u$ and $v$ is denoted by $(u,v)$, and we use $P_{v_0, v_p} = (v_0, v_1, ..., v_p)$ to denote a simple path from $v_0$ to $v_p$.
The length of a simple path in unweighted graph is the number of edges in the path.
Given two vertices $u$ and $v$, their shortest path $SP_{u,v}$ is the path between them with minimal length.
The distance from vertex $u$ to $v$ is the length of shortest path $SP_{u,v}$ from $u$ to $v$, denoted by $d(u,v)$.
For each vertex $u$, its $\epsilon$-neighbors, denoted as $N_{\epsilon}(u)$ is a set of vertices such that their distance to $u$ is no greater than $\epsilon$, i.e., $N_{\epsilon}(u) = \{v \in V | 0 < d(u,v) \le \epsilon\}$.

Suppose a subset of vertices $V^\ast=\{v_1,v_2,...,v_k\} \subseteq V$ has been selected as landmarks.
For the traditional landmark indexing, each vertex $u$ in directed graph is assigned with two lists $L_{out}(u)=(<d(u,v_1),SP_{u,v_1}>,<d(u,v_2),SP_{u,v_2}>,...,<d(u,v_k),SP_{u,v_k}>)$ and
$L_{in}(u)=(<d(v_1,u),SP_{v_1,u}>,<d(v_2,u),SP_{v_2,u}>,...,<d(v_k,u),SP_{v_k,u}>)$.
Note that, if some landmarks are not reachable from (or cannot reach) specific vertex, the corresponding distance and shortest path is set to be null.

For any vertex pair $(s,t)$, the traditional landmark scheme approximate the shortest path by concatenating shortest paths $SP_{s,v^\prime}$ and $SP_{v^\prime,t}$ where $v^\prime \in V^\ast$ achieves minimal $d(s,v^\prime)+d(v^\prime,t)$.
Clearly, if $v^\prime$ lies in one of shortest path from $s$ to $t$, the estimated shortest path is exact one.
In ideal situation, for any vertex pair $(s,t)$, we can always find a landmark $x$ from landmark set $V^\ast$ such that $d(s,v)+d(v,t)=d(s,t)$.
We refer to such landmark set as {\em landmark cover}.
%That is, there always exists a landmark from {\em landmark cover} appearing in one of shortest paths from $s$ to $t$.
Furthermore, 2hop labels are essentially a {\em landmark cover},
because for any pair of vertices, there always exists one common vertex in their corresponding label such that at least one of their shortest paths goes through it.
These common vertices serves as {\em landmark cover} in our scenario.

\comment{
Here, we formally define the {\em landmark cover} and {\em optimal landmark cover discovery problem} based above indexing scheme as follows:

\bdefin{\bf (Landmark Cover)}
Given unweighted and directed graph $G=(V,E)$, and a subset of vertices $V^\ast \subseteq V$, we say $V^\ast$ is a landmark cover if and only for any vertex pair $(s,t)$,
there exists a landmark $v \in V^\ast$
\edefin

\bdefin{(\bf (Optimal Landmark Cover Discovery Problem)}
Given unweighted and directed graph $G=(V,E)$, we would like to seek a landmark cover with smallest number of vertices.
\edefin
}

\begin{figure}
\centering
\begin{tabular}{c}
\psfig{figure=Figures/indexexample.eps,scale=0.65}
\end {tabular}
\caption {Indexing Example}
\label{fig:indexexample}
\end{figure}



\subsection{New Landmark Indexing Scheme}
\label{landmarkindex}

Considering a traditional landmark cover $V^\ast$ with $k$ landmarks, each vertex is required to explicitly maintain two $k$-element lists for the shortest path to (from) all landmarks.
Given a graph $G=(V,E)$, the total index size is clearly $2k|V|$.
However, we observe that many unnecessary landmarks are recorded for each specific vertex pair when one of their shortest paths goes through several landmarks.
%This is essentially caused by the query procedure which needs to find out a exact intermediate vertex in the shortest path.
%Simply speaking, the shortest path is expressed as two segments: the path from source to intermediate and the path from intermediate to destination.
In order to gain more compact index size,
we represent each shortest path as three segments instead of two segments in traditional methods: 1) the path from source to appropriate landmark close to it; 2) the path from current landmark to another landmark close to destination;
3) and the path between destination and above nearby landmarks.

We note that the functionality of these landmarks in this scenario is analogous to the highway entrances or exits of transportation network.
In order to find the shortest path from starting point to destination, one simply find the shortest path from starting to the appropriate entrance of highway,
and then get off the correct exit of highway which leads to the remaining shortest path to the destination.
Based on 3-segment expression, for any pair of vertices $(s,t)$, if there are many landmarks from one landmark cover appear in one of shortest path,
both $s$ and $t$ only need to store the {\em essential} landmark, i.e., the nearest one.
To facilitate the exact shortest path query, the middle segment connecting two landmarks are required to be available during online query.
As we discussed in section~\ref{contribution}, the landmark size is rather small and the shortest path among them is almost constant (no more than 3 in large social network),
thus the benefit from index size reduction would easily pay off the cost of materializing pairwise shortest path among landmarks.
This materialization essentially serves as {\em shortest path oracle} which is able to answer shortest path queries between any two landmarks in constant time.


\begin{example}
Figure~\ref{fig:indexexample} shows two different indexing schemes for vertex pair $(s,t)$ given that $3$ landmarks $v_1$, $v_2$ and $v_3$ appear in one of shortest path between them.
As we can see from traditional indexing, the shortest paths from $s$ to all landmarks and from landmarks to $t$ are all recorded.
According to 3-segment representation of shortest path, we only need to record one nearest landmark for each vertex, i.e., $v_1$ for source $s$ and $v_3$ for destination $t$.
The traditional landmark index size is reduced from $6$ to $2$.
Given the shortest path from $v_1$ to $v_3$, the shortest path $SP_{st}$ is easily recovered by $SP_{sv_1}+SP_{v_1 v_3}+SP_{v_3 t}$.
\end{example}


Our new landmark indexing scheme assigns each vertex $u$ two lists, $L^\prime_{out}(u)$ and $L^\prime_{in}(u)$.
$L^\prime_{out}(u)$ records the {\em essential} list of landmarks which is reachable from $u$, including their respective distance and shortest path,
i.e., $L^\prime_{out}(u)=(<x_1:d_{x_1},SP_{x_1}>,...,<x_p:d_{x_p},SP_{x_p}>)$, where $d_{x_i}=d(u,x_i)$ and $SP_{x_i} = SP_{u x_i}$.
Similarly, $L^\prime_{in}(u)$ records the {\em essential} list of landmarks which can reach $u$, including their respective distance and shortest path,
i.e., $L^\prime_{in}(u)=(<y_1:d_{y_1},SP_{y_1}>,...,<y_p:d_{y_p},SP_{y_q}>)$, where $d_{y_i}=d(y_i,u)$ and $SP_{y_i} = SP_{y_i u}$.
Both $x_i$ ($1 \le i \le p$) and $y_j$ ($1 \le j \le q$) are landmarks.
Given a shortest path query $(s,t)$, let $x_i \in L^\prime_{out}(s)$ and $y_i \in L^\prime_{in}(t)$.
We define the {\em landmark distance} from $s$ to $t$:
\beqnarr
d(s,t|L^\prime_{out}(s),L^\prime_{in}(t)) =  \nonumber \\
min_{x_i \in L^\prime_{out}(s), y_j \in L^\prime_{in}(t)} d(s,x_i)+d(x_i,y_j)+d(y_j,t) \nonumber
\eeqnarr
Corresponding {\em landmark shortest path} is the concatenation of $SP_{s x_i}$, $SP_{x_i y_j}$ and $SP_{y_j t}$.
Note that, the pairwise distance and shortest path among landmarks $d_(x_i y_j)$ and $SP_{x_i y_j}$ are materialized.
In addition, the index size is defined to be $\sum_{u \in V} (|L^\prime_{out}(u)| + |L^\prime_{in}(u)|)$.

If {\em landmark distance} by landmark set $V^\ast$ is exactly shortest distance for any pair of vertices,
we refer to $V^\ast$ as {\em landmark cover} in this setting.
Formally, we define {\em landmark cover} and {\em optimal landmark cover discovery problem} based new indexing scheme as follows:

\bdefin{\bf (Landmark Cover)}
Given unweighted and directed graph $G=(V,E)$, and a subset of vertices $V^\ast \subseteq V$, we say $V^\ast$ is a landmark cover if and only for any vertex pair $(s,t)$,
there exists two landmarks $x, y \in V^\ast$ such that $d(s,x)+d(x,y)+d(y,t)=d(s,t)$.
That is, there always exists two landmarks appearing in one of shortest paths from $s$ to $t$.
\edefin

When $x$ is the same with $y$, the landmark cover based on new indexing scheme is degraded to the one based on traditional indexing scheme,
which is also equivalent to the aforementioned 2-hop labels.

\bdefin{(\bf (Optimal Landmark Cover Discovery Problem)}
Given unweighted and directed graph $G=(V,E)$, we would like to seek a landmark cover such that its total index size based on new indexing scheme
$\sum_{u \in V} (|L^\prime_{out}(u)| + |L^\prime_{in}(u)|)$ is minimized.
\edefin


Since 2hop labeling problem can be treated as special case of Optimal Landmark Cover Discovery Problem, where two landmarks that serve as meeting point become only one.
we can easily derive following result:

\bthm
Given unweighted and directed graph $G=(V,E)$, Optimal Landmark Cover Discovery Problem is NP-hard problem.
\ethm

}


==> LandmarkEst.tex <==
\section{Shortest Path Estimation}
\label{estimation}

In this section, we consider how to approximate the shortest between two vertices using landmark indices.
Before that, we first introduce a compact representation of landmark indices in the implementation,
which not only achieves much memory saving, but also effectively assists in estimating shortest paths.

\subsection{Compact Landmark Indices Representation}
\label{compactrep}

The straightforward 

==> Landmarkindex.tex <==



\section{Local Landmark Selection and Efficient Indexing}
\label{localselection}

According to the discussion in subsection~\ref{scpsolution}, selecting exact landmark set with minimum local index size is really computationally intractable.
By relaxing the requirement of computing exact shortest path by local landmarks, we turn to a similar while more practical problem:
{\em given a specific number $k$, how can we find $k$ {\bf good} landmarks to approximate the shortest paths of most vertex pairs with high accuracy?}
In this section, we first exploit the properties of good landmarks on social networks to compute six-degree shortest paths.
Guided by these properties, effective landmark selection strategy and efficient indexing algorithm are descried later.

%\begin{figure}
%\centering
%\begin{tabular}{c}
%\psfig{figure=Figures/coreexample.eps,scale=0.6}
%\end {tabular}
%\caption {$k$-center in social network}
%\label{fig:coreexample}
%\end{figure}


\subsection{Good Landmarks in Social Networks}
\label{goodlandmark}

We start from most simple scenario to gain a better intuition of good landmarks in social networks.
Suppose we only need to select one landmark to approximate the shortest path computation.
Intuitively, the best landmark should be the one in the very {\em central} position of graph~\cite{Potamias:2009:FSP:1645953.1646063}.
This high-level understanding suggests two concepts of {\em central} vertex (i.e., landmark) from different perspectives:
1) a {\em central} vertex is a vertex lying on many shortest paths;
2) a {\em central} vertex is a vertex close to other vertices in the graph.
In the optimized scenario, the best {\em central} vertex based on first concept is referred to as the vertex with largest vertex betweenness~\cite{citeulike:1025135},
while another one refers to the vertex with minimal radius.
We generalize both concepts to a set of vertices and analyze the relationship to social networks.

\noindent{\bf Vertex betweenness: }
We want to find a set of landmarks which are able to maximally {\em cover} the vertex pairs with distance no greater than $6$ in the graph.
Simply speaking, we wish that most of shortest paths with length no greater than $6$ pass through those landmarks.
The comprehensive empirical study on several well-known social networks (i.e., Flickr, LiveJournal, Orkut and Youtube) in~\cite{Mislove07}
clearly demonstrates the presence of densely connected {\em core} comprising of a small portion of vertices with highest degree.
The removal of the {\em core} dramatically disconnects the entire graph, implying that most of connections between two vertices rely on few high-degree vertices.
In other words, few high degree vertices serve as the key intermediate in most of shortest paths,
thus are qualified to be landmarks under this criterion.

\noindent{\bf $k$-center: }
We want to find $k$ landmarks such that the maximum distance between each vertex and each landmark is minimized.
Since shortest distance is metric measure, this problem is essentially metric $k$-center problem which has been proved to be NP-hard.
This criterion guarantees that each vertex in the graph can find a landmark not far from itself.
Based on local landmark indexing scheme, the shortest path from $s$ to $t$ is estimated by $d(s,x)+d(x,y)+d(y,t)$, where $x$ and $y$ are essential landmarks to $s$ and $t$, respectively.
Under this criterion, both $d(s,x)$ and $d(y,t)$ are effectively constrained, which potentially results in good approximation (i.e., small value of $d(s,x)+d(x,y)+d(y,t)$).
Now, let us consider these landmarks in the social networks exhibiting aforementioned highly connected {\em core}.
It is surprising to see that {\em core} vertices naturally fit this criterion, that is, the distance between core vertex and non-core vertex is rather small.
The length of most of shortest paths between two non-core vertices is typically small in social network,
thus the distance between core vertex and non-core vertex is ever shorter since core vertex is very likely to lie on these shortest paths.


According to above analysis, the high-degree vertices are sufficient to serve as landmarks from different angles due to the characteristics of social networks.
On the other hand, both computing vertex betweenness and $k$-center are very computational costly.
Using high-degree vertices to approximate optimal landmarks under both criteria effectively avoids those cost and can be easily scaled to large social networks.
We will demonstrate the power of high-degree vertices as landmarks in the experiments.


\subsection{Efficient Local Landmark Indexing}
\label{localindexing}

Due the existence of small-world phenomenon in social networks, it is sufficient for each vertex to record the essential landmarks within $6$ steps to approximate the shortest path.
Given a certain portion of high-degree vertices as landmark, in order to assign each vertex $u$ their essential landmarks and compute shortest paths among landmarks, the straightforward solution is to precompute the shortest path (distance) of each pair of vertices with distance no greater than $6$.
For a large social networks with several millions of vertices, such computational cost and memory assumption are not acceptable.

To tackle the problem, we introduce an efficient procedure which perform two local breath-first traversals (BFS) for each landmark to visit only its $6$-neighbors (i.e., the vertex with distance to landmark no more than 6).
That is, one BFS for outgoing essential landmarks while another one for essential incoming landmarks.
Specifically, for each BFS starting from landmark $u$, two tasks have to be completed:
1) it needs to find out all other landmarks whose distance to (from) $u$ is no more than $6$, and record one shortest path between them for query answering;
2) for each visited non-landmark vertex $v$, we need to quickly check whether there is other landmarks appearing in a shortest path from $u$ ($v$) to $v$ ($u$).
The first task can be easily achieved by introducing an extra integer for each vertex, which is used to record the previous vertex on the shortest path from source landmark $u$ to current vertex or from current vertex to source landmark.
To simplify the explanation, we focus on the generation of incoming essential landmark, which can be easily generalized for outoging essential landmark assignment.
In order to achieve second task, we utilize a simple observation:
{\em let vertex $y$ lies on the shortest path from landmark $u$ to non-landmark vertex $v$ with distance $d(u,v)-1$ (i.e., $y$ is one step closer than $v$ with respect to $u$),
if there is a landmark $x$ appearing in one shortest path from $u$ to $y$ ($x$ and $y$ may not be distinct),
$x$ definitely lies on the shortest path from $u$ to $v$ and $u$ will not be essential landmark of $v$.}
Based on this observation, we maintain a flag $b(v)$ for each vertex $v$, such that $b(v)=true$ if $v$ is landmark or $b(y)=true$ when $1 < d(u,v) \le 6$, $d(u,y)=d(u,v)-1$ and $y$ can reach $v$.
During BFS process, when we visit each vertex $v$, if its flag $b(v)$ is not true meaning there is no other landmark lying on the shortest path from $u$ to $v$, we append $u$ and shortest path $SP(u,v)$ to its $L^e_{in}(v)$.

\input{Figures/BFSIndexing.tex}

The outline of BFS-based algorithm for generating incoming landmark indices is described in Algorithm~\ref{alg:bfsindex}.
The flag $b(v)$ for each vertex $v$ is updated when $v$ is landmark or its previous vertex in the shortest path $SP(s,v)$ (Line 6 and Line 16).
When vertex $u$ is accessed from queue and its flag $b(u)$ is false, the source $s$ is assigned to incoming label $L^e_{in}(u)$ of vertex $u$ (Line 10).
This procedure will be invoked for each landmark.
The outgoing landmark indices $L^e_{out}(u)$ for each vertex $u$ can be similarly generated by reverse BFS (change $out\_neighbor$ in Line 12 to $in\_neighbor$).
In total, labeling indexing procedure takes $O(\sum_{u \in V^\ast} (|N_6(u)|+|E_6(u)|))$ time, where $V^\ast$ is landmark set, $N_6(u)$ ($E_6(u)$) is the number of vertices (edges) in the $u$'s 6-neighbors (including incoming neighbors and outgoing neighbors).


==> Prob.tex <==
\section{Overview}
\label{overview}

Social networking is playing more and more important role in our daily life.
Coupling with advance of Internet technology, lots of social networking websites such as Facebook.com, Twitter.com and LinkedIn.com are created to facilitate various social actives.
Many existing research are devoted to study the structural properties of such emerging social networks.
One of the most fundamental properties is ``small-world phenomenon'' revealing the fact that most of persons can be connected by very short paths through social networks.
This property is made well-known by social phycologist Stanley Milgram's famous experiment ``six degrees of separation''.
Besides social science, this phenomena is also explored and confirmed in many areas even gaming field.
The game ``six degree of Kevin Bacon'' relying on the concept of ``small world phenomenon'', asks players to try to connect any actors to Kevin Bacon in smallest number of links.
The phenomena is also observed from the data of Facebook and LinkedIn.
In Facebook, one of its well-known applications, so-called ``Six Degrees'', collects around $5.8$ million users and shows that the average pairwise shortest distance is $5.73$.
Also, the report from Sysomos~\footnote{http://www.sysomos.com/insidetwitter/sixdegrees/} observes that around half of users on Twitter are on average $4$ steps away from another while nearly everyone is $5$ steps away.

The aforementioned applications all relate to the fundamental problem: finding shortest path within $6$ steps. Indeed,
this is also consistent with basic principle of building social connections that people always make new friendship
through some other close acquaintances.
%This is also equivalent to finding the persons in the shortest path from themselves to the targeted person they want to know.
Motivated by the striking observation -- ``six degree of separation'',
many preliminary efforts from industrial perspective have been imposed for finding shortest path between two persons with distance no greater than 6 in social network.
One of most famous applications is the service ``How you're connected to A'' developed by LinkedIn, which offers a precise description of friendship chain between you and friend A within $3$ steps.
In addition, Microsoft's Renlifang~\footnote{http://renlifang.msra.cn/6du.aspx} allows users to retrieve the shortest path between two entities if their distance is smaller or equal to $6$.
The newly emerged online application ``Six Degrees''~\footnote{http://www.6-degreesonline.com} provides an interactive way to demonstrate how you connect to other people in your facebook network.
The efficiency of those applications are far away from the achievement made by real-time routing on road networks.


Recently, the traditional shortest path finding problem has been extensively studied and applied in numerous computing fields.
However, the applicability of existing methods on our six-degree shortest path problem is hindered by the characteristics of social network data.
Unlike the planar network and road network on which most of research focus, social networks have very high vertex degree in addition to their massive size.
The shortest-path processing techniques designed for road networks do not perform well on such massive and dense graphs.
For some methods aiming at estimating exact shortest distance even with guaranteed approximation ratio,
they are still not applicable in our scenario because the length of most shortest paths is very short (no more than $6$ steps) and the involving of small errors will lead to meaningless results.
Indeed, daunting size of dense large-scale networks makes the most simple and basic graph queries extremely difficult and expensive to process.
Consider performing BFS (breath-first search) on Facebook which currently has more than $750$ million active users and average user has $130$ friends.
The number of users needed to be traversed in six-degree shortest path finding procedure can be up to hundreds of billions which is very costly.


\section{Problem Statement}
\label{prob}

Let $G=(V,E)$ be an unweighted and undirected graph where $V=\{1,2,...n\}$ is the vertex set and $E \subseteq V \times V$ is edge set.
The edge from vertex $u$ and $v$ is denoted by $(u,v)$, and we use $P_{v_0, v_p} = (v_0, v_1, ..., v_p)$ to denote a simple path from $v_0$ to $v_p$.
The length of a simple path in unweighted graph is the number of edges in the path.
Given two vertices $u$ and $v$, their shortest path $SP_{u,v}$ is the path between them with minimal length.
The distance from vertex $u$ to $v$ is the length of shortest path $SP_{u,v}$ from $u$ to $v$, denoted by $d(u,v)$.
For each vertex $u$, its $\epsilon$-neighbors, denoted as $N_{\epsilon}(u)$ is a set of vertices such that their distance to $u$ is no greater than $\epsilon$, i.e., $N_{\epsilon}(u) = \{v \in V | 0 < d(u,v) \le \epsilon\}$.
To facilitate our discussion on six-degree shortest path query,
we say vertex $v$ is $6-reachable$ from vertex $u$ if the distance from $u$ to $v$ is no greater than $6$.
If $u$ and $v$ are $6-reachable$ to each other, their shortest paths (maybe more than one) are {\em 6-degree shortest path} $SP_6(u,v)$.


\bdefin{\bf Six-degree Shortest Path Query (6DSP)}
Given a unweighted and undirected graph $G=(V,E)$, and two vertices $u$ and $v$,
if $u$ and $v$ are reachable from each other and their distance $d(u,v) \le 6$ (i.e., $6-reachable$), six-degree shortest path query returns unique shortest path $SP_6(u,v)$ between them.
Otherwise, the query returns null.
\edefin


\section{Search Algorithms without \\ Structural Organization}
\label{searchalgs}

In this section, we adapt existing shortest path computation methods originally on road networks, ALT ($A^\ast$, landmark and triangle inequality) and contraction hierarchy (CH), for our social network searching scenario.
In general, several novel techniques are proposed to incorporate these methods by taking characteristics of social network data into consideration.
Especially, a new landmark selection strategy is introduced for ALT; a novel node ordering scheme and an efficient node contraction method are discussed in CH.


\subsection{ALT}
\label{alt}

ALT is proposed by Goldberg and Harrelson~\cite{GoldbergSODA05} to considerably reduce the search space by combining $A^\ast$ search, landmark technique and triangle inequality.
Generally, landmark and triangle inequality are used to compute the effective lower bound to facilitate bidirectional $A^\ast$ search.
They demonstrate that the performance of bidirectional $A^\ast$ search can be significantly improved by incorporating lower bound computed based on landmarks instead of Euclidean distance.
Analogous to most of online searching algorithms, ALT mainly consists of two steps: preprocessing and online bidirectional $A^\ast$ search.
During preprocessing step, some landmarks are selected according to certain selection strategies.
Then, for each vertex, their distance to landmarks are precomputed and recorded.
When distance queries come, we use the recorded distance to compute lower bounds (one to estimate the distance from current node to destination in forward search, another for the distance from current node to source in backward search),
and apply them in bidirectional $A^\ast$ shortest path algorithm.
The effective lower bound provided by landmarks would allow us to greatly reduce the search space.
In other words, the performance of ALT method largely relies on the effectiveness of landmark selection.

\input{Figures/ALT.tex}

Here, we first revisit ALT framework and then discuss how to select good landmarks in social networks.
The online search procedure is outlined in Algorithm~\ref{alg:altquery}.
Basically, the forward $A^\ast$ search from $s$ and backward $A^\ast$ search from $t$ are performed in an alternative manner.
During bidirectional search, the minimal length of shortest path $\mu$ so far is updated accordingly (Line 13 to 15).
The algorithm terminates when search procedure picks one vertex from priority in one direction which has been scanned in the other direction (Line 9 to 11).
Note that, potential functions $p_f(v)=\frac{1}{2}(\pi_f(v)-\pi_b(v))+\frac{\pi_b(t)}{2}$ and $p_b(v)=\frac{1}{2}(\pi_b(v)-\pi_f(v))+\frac{\pi_f(t)}{2}$,
where $\pi_f(v) = max_{x \in L} |d(v,x)-d(x,t)|$ and $\pi_b(v)=max_{x \in L}|d(v,x)-d(x,s)|$.


Finding good landmarks is critical for the performance of ALT method.
Most straightforward solution is to randomly select a fixed number of vertices as landmarks.
Clearly, we can do much better in landmark selection.
Since the landmark is used to estimate the lower bound, a good landmark tends to lie behind the shortest paths between a pair of vertices.
Some existing empirical studies~\cite{Mislove07} demonstrate the existence of ``core'' structure (highly connected component with small-world phenomena) in large social network.
They demonstrate that ``core'' plays remarkable role in keeping the remainder of social networks connected.
Based on this observation, the boundary nodes whose diameter is rather close to network diameter are able to serve as good landmark
because most of pair of vertices naturally find one vertex in boundary nodes which lies behind one of them.
Our landmark selection procedure extracts the boundary nodes by sampling method.
We sketch the method in Algorithm~\ref{alg:altlandmark}.

\input{Figures/Landmark.tex}

We start the procedure by randomly sampling a set of vertices and generate shortest path tree by performing BFS traversal from those vertices.
For each shortest path tree, we only consider their leaf nodes as landmark candidate and record their distance information $s(w)$ and $c(w)$ (Line 5 to 9).
Intuitively, boundary nodes of social networks frequently appear in the leaves of BFS tree and their distance in corresponding BFS tree is relatively large in general.
Therefore, we rank those landmark candidates by their average distance serving as leaves in BFS trees (Line 11 to 13).
Finally, we pick the top ranked candidates as landmarks.
In order to make landmark uniformly distributed in entire network, the candidates which is close to currently selected landmark is removed from queue (Line 14 to 16).

%\textcolor{blue}{what if consider the combination of average distance and $c(w)$ (frequency serving as leaf nodes)?}

\comment{
general pruning technique, main idea is to compute feasible lower bound by effective landmarks.
how to select good landmarks highly influence the searching performance of ALT.
bidirectional search

basic procedure
1) landmark selection and landmark distance computation for each vertex;
2) compute consistent feasible function value for each vertex;
3) for $(u,v)$ shortest path query, alternatively run forward search and backward search until certain stopping condition is satisfied (make it clear why they are correct).

landmark selection procedure (main spirit: boundary nodes tend to generate good lower bound since it potentially on left side of source or right side of destination)
1) randomly sample a set of nodes as roots, perform BFS from those root nodes, rank the farthest nodes they can reached based on their average distance to those starting nodes;
2) select $5\%$ top ranked nodes as landmarks (boundary nodes, it is defined as a set of vertices whose diameters are very large);
}


\subsection{Contraction Hierarchy}
\label{ch}

Contraction hierarchies~\cite{Geisberger:2008} is one of techniques exploring highway nature of road network to speedup Dijkstra algorithm.
The basic idea is to construct some short cuts which able to skip traversing ``unimportant'' nodes during online search procedure.
As ALT method, it is made up of two steps: node contraction step and query procedure.
In the first step, nodes are firstly ordered according to their ``importance'' (node importance is heuristically evaluated by linear combination of several factors).
We now create the short cut by contracting the nodes following this order and preserve the shortest path information for remaining vertices.
For each vertex $v$, if there is a unique shortest path $P=(u,v,w)$ such that order of both $u$ and $w$ are higher than $v$,
a shortcut edge $(u,w)$ is introduced to graph.
After that, vertex $v$ and all its incident edges are removed from graph.
Eventually, shortcut edges with edges in original graph constitute overlay graph which will be used for online query.
To answer shortest path queries, bidirectional Dijkstra algorithm is adopted in overlay graph from source and from destination respectively.
For forward search, we only relax the edge $(v,w)$ such that order of $w$ is higher than that of $v$.
Similarly, we only relax the edge $(w,v)$ such that the order of $w$ is higher than that of $v$.
The intuition is that both searches from source and from destination ``climb'' toward and meet at more ``important'' vertex (peaks).


\begin{figure}
\centering
\begin{tabular}{c}
\psfig{figure=Figures/ncexample.eps,scale=0.5}
\end {tabular}
\caption {Generating shortcut with length $3$}
\label{fig:ncexample}
\end{figure}

In the following, we describe the node contraction in six-degree shortest path query context provided that node ordering is given.
Afterward, we discuss how to obtain ``good'' node ordering which potentially reduces the number of added shortcut edges.

\input{Figures/NodeContraction.tex}

\noindent {\bf Node Contraction: }
Since we focus on the shortest path with length no greater than $6$,
the length of shortcut edges which are needed in bidirectional search stage should be no more than $6$.
Therefore, instead of generating the shortcut with arbitrary length, we are able to introduce shortcuts in batch based on exiting shortcuts with smaller length.
Generally, according to node ordering, we firstly scan all vertices to generate the shortcut edges with length 2 and record those shortcuts.
In order to generate shortcuts with length $3$, we only need to consider the endpoints of shortcuts with length 2.
In figure~\ref{fig:ncexample}, edge $(4,1)$ is existing shortcut with length $2$.
To generate shortcut with length $3$, we only consider vertex $1$ and its incident vertices like $5$ with higher order, and check if there is alternate shortest path between $4$ and $5$.
For shortcuts with length $4$, there are two combinations: concatenation of $2$ shortcuts with length $2$, or one with length $1$ and another is shortcut with length $3$.
Theoretically, we can repeat this process until shortcut edges with length $6$.
Due to the consideration of reducing preprocessing time, we only generate the shortcut edges with length no more than $4$.
Even for shortest path with length $6$, those shortcuts can help considerably reduce the search space.
The advantage of this algorithm is that we generate the shortcut edges by directly extending existing edges instead of exhaustively checking every pair of each vertex's neighbors in overlay graph.
We summarize the entire node contraction procedure in Algorithm~\ref{alg:nc}.


\noindent {\bf Node Ordering: }
Though many node ordering heuristics are introduced in~\cite{Geisberger:2008}, no objective is formally formalized.
As discussed before, we can see that the number of shortcuts with length $l$ relies on the number of shortcuts with length $l-1$.
Along this line, reducing the number of shortcuts with length $2$ potentially results in fewer shortcuts globally.
Therefore, we now focus on the problem of finding node ordering which achieves minimum number of shortcuts with length $2$.

\bdefin{\bf(Node Ordering Problem)}
Given graph $G=(V,E)$, we try to seek a node ordering $\prec$ on $V$ such that the number of newly added shortcuts with length $2$ ($E_2$) in resulting graph is minimum.
\edefin

\begin{figure}
\centering
\begin{tabular}{c}
\psfig{figure=Figures/nodeorder.eps,scale=0.5}
\end {tabular}
\caption {Linear node ordering}
\label{fig:nodeorder}
\end{figure}

Assuming node ordering is given, we can always collapse the graph into a line following their corresponding orders (see Figure~\ref{fig:nodeorder}).
We now consider whether we need to create a shortcut for a edge $(u,w)$.
Clearly, if there is a intermediary $v$ which is common neighbor of $u$ and $w$ and its order is higher than both $u$ and $w$, no shortcut is needed.
From the viewpoint of vertex $v$, we would say $v$ {\em covers} vertex pair $(u,w)$ if and only if $v \in N(u)$, $v \in N(w)$ and $min(u,w) \prec v$.
Intuitively, vertex with higher order is able to {\em cover} more vertex pairs from its neighbors.
Hence, assigning higher order to vertex covering large number of uncovered vertex pairs naturally becomes reasonable choice.
As the number of vertex pairs with distance $2$ is fixed, more are covered, less shortcuts are probably created.

\input{Figures/GreedyOrder.tex}
%\input{Figures/GreedyOrder1.tex}

We propose an ordering algorithm mimicking greedy algorithms for set cover problem to achieve the goal.
The greedy selection order during procedure is considered as the node ordering.
Let $U = \{(u,v) | d(u,v)=2\}$ including all shortest path with length 2.
For each vertex $v$, it is associated with a set of vertex pairs $C_v=\{(u,w) | d(u,w)=2 \mbox{ and }v\in N(u)\cap N(w)\}$.
We apply greedy selection strategy (Algorithm~\ref{alg:greedyorder}) to obtain the ordering.
During selection procedure, we always pick the vertex that maximally covers the uncovered pairs.
Note that, vertex $x$ is only able to cover the shortest path with both endpoints having lower order than $x$ (i.e., $u,v \notin T$).
To break the tie, we prefer choosing the vertex with larger degree.
This ordering method can also combine with other heuristics to gain better performance.


\comment{
An alternate strategy (Algorithm~\ref{alg:greedyordermin}) directly focuses on minimizing the newly created shortcuts.
In this method, we try to select the node with minimal number of already selected neighbors, because the number of already selected neighbors indicates the amount of potential shortcuts.
Another attractive point is that, we somehow address the uniformity issue such that nodes would be better to be contracted in an uniform order around entire graph instead of concentrating on one region.
If the vertex $v$ is currently selected, all its neighbors potentially create larger number of shortcuts thus are not likely to be selected in the near future.
Note that, to break the tie during selection, we prefer the vertex with larger degree in both algorithms.
These ordering methods can also combine with other heuristics to gain better performance.
}

\comment{
1) node ordering based on $6$-step betweenness (computed by sampling method);
2) fast node contraction (consider 2-hop contraction, 3-hop contraction ...);
}


\section{Search Algorithms with \\ Component-based Structure}
\label{searchalgscomponent}

In this section, we introduce several efficient shortest path finding algorithms based on component structure.
Those components are generated by graph decomposition method.
Basically, social network is organized as star-shape structure such that the central part is the ``core'' of entire graph which entail the major connections among other small outlier components.


\begin{figure}
\centering
\begin{tabular}{c}
\psfig{figure=Figures/starshape.eps,scale=0.5}
\end {tabular}
\caption {Star-shape structure}
\label{fig:starshape}
\end{figure}


\subsection{Graph Decomposition}
\label{decomposition}

The existence of well-connected ``core'' in social network has been demonstrated in empirical studies on several real datasets~\cite{Mislove07}.
By removing a small portion of hub nodes (nodes with high degree), the connectivity of entire graph is significantly break down and forms large number of small-sized components.
They also observe that the distance between two nodes in the ``core'' is roughly $4$ and most of remaining nodes are very few steps away from the core.
According to those interesting observations, social network seems can be organized as a star-shape structure,
where a well-connected core ($C_0$ in Figure~\ref{fig:starshape}) serves as major transportation center bridging the communication between different small components ($C_1$ to $C_7$ in Figure~\ref{fig:starshape}).
Of course, few shortest paths connecting different small components are allowed without involving core component.
Given this star-shape structure, we wish to implement efficient routing for relatively ``long-range'' shortest paths (such as the one with length $5$ or $6$) through central component,
while other ``local'' shortest paths are found within each components.
To meet this goal, we identify certain key properties that good star-shape structure should satisfy:

\noindent 1) {\em Small-sized core with small diameter}: only small portion of vertices (like $5\%$ of total number of vertices) are included in the core;
the length of any shortest path within core is bounded by a small constant.

\noindent 2) {\em Strong connections between core and small components}: most of shortest paths between different small components go through core.

\noindent 3) {\em Weak connections among small components}: few shortest paths among different small components do not involve nodes in the core.

Our algorithm to decompose entire graph into desired structure consists of two main steps:
core extraction step and graph partition on remaining graph.
In the first step, we try to extract the core containing some important segments in the middle part of relatively long-range shortest path (with length $5$ or $6$).
The segment (subpath of ``long-range'' shortest paths) importance is measured by the number of shortest paths go through it (i.e., segment betweenness).
Then, we remove the core from original graph.
For the remaining graph, we apply well-known graph partition software METIS~\footnote{http://glaros.dtc.umn.edu/gkhome/metis/metis/overview} to decompose it into several small components.

\input{Figures/CoreExtraction.tex}

\begin{figure}
\centering
\begin{tabular}{c}
\psfig{figure=Figures/coreshortcut.eps,scale=0.6}
\end {tabular}
\caption {Adding shortcuts}
\label{fig:coreshortcut}
\end{figure}

The core extraction approach is outlined in Algorithm~\ref{alg:coreextraction}.
To begin with, we randomly select a small portion of vertices as roots (Line 2) and perform BFS from those roots to obtain the ``long-range'' shortest paths $P$ with length $5$ and $6$ (Line 5).
All edges in $P$ are stored in a priority queue according to their edge betweenness (Line 6 to 10).
We now concentrate on expanding $V_c$ and $E_c$ by selecting appropriate edges from priority queue (Line 12 to 38).
In the while loop, we iteratively consider the edge with maximum edge betweenness in the current queue (Line 13).
If only one of edge's endpoints $u$ does not belong to core, we check whether this endpoint can be included in core or not.
Especially, we perform BFS by expanding $r$ steps in order to conform if adding this endpoint $u$ still maintains the diameter constraint $r$ (Line 16).
If so, vertex $u$ is included in the core and edge $(u,v)$ is added into $E_c$ (Line 16 to 18).
Since BFS tree $T_u$ might brings some extra vertices to help connect to the core (like vertex $x$ in Figure~\ref{fig:coreshortcut}(a), green ones are vertices in the core),
to maintain $u$'s diameter, we simply add the shortcuts from $u$ to those vertices in the core (like $(u,v_1)$ and $(u,v_2)$ in Figure~\ref{fig:coreshortcut}(b)).
Those operations are summarized in Line 19 to 22.
Another case is that both endpoints $u$ and $v$ are not in the core.
We process both vertices in the same way (Line 25 to 37).
The only difference is that we are allowed to add edge $(u,v)$ if and only if both vertices are contained in the core (Line 34 to 36).
The resulting core is a weighted graph with diameter no more than $r$.


\subsection{Component-based ALT}
\label{compalt}

As mentioned before, landmark selection is playing important role in the performance of ALT.
Here, we propose a method to select landmarks based on the star-shape structure (component-based structure).
For any pair of vertices, a landmark lying behind one of vertices tends to provide tight bound.
Therefore, for random shortest path queries, boundary nodes far away most of vertices would be good choice to be landmark.
In this sense, we consider the landmark selection on the vertices in the small components.
To make sure landmarks are uniformly distributed around the outlier of entire graph, we try to omit the vertices that are close to currently selected one.
By this way, we also avoid putting many landmarks into one component.

To achieve aforementioned goals, we propose a simple landmark selection algorithm based star-shape structure as follows.
For each small component $C_i$, we have a set of vertices $B_i \subseteq C_i$ connecting to the vertices in the core $C_0$.
First, pick a vertex $v$ in $C_1$ that farthest to vertex set $B_1$  and mark the vertices not belonging to core within $3$ steps from $v$ as processed.
Randomly pick one of $C_1$'s neighboring components $C_k$, then select a vertex $u$ that is not marked and farthest away from its corresponding $B_k$.
We proceed such iteration until no landmark can be selected or certain number of landmarks has been selected.
Clearly, we can incorporate those landmarks with ALT method for shortest path routing.


\comment{
\subsection{Component-based CH}
\label{compch}

also consider the relation between unique shortest path system and node order in CH.
}


==> Prob_bak.tex <==
\section{Overview}
\label{overview}

Social networking is playing more and more important role in our daily life.
Coupling with advance of Internet technology, lots of social networking websites such as Facebook.com, Twitter.com and LinkedIn.com are created to facilitate various social actives.
Many existing research are devoted to study the structural properties of such emerging social networks.
One of the most fundamental properties is ``small-world phenomenon'' revealing the fact that most of persons can be connected by very short paths through social networks.
This property is made well-known by social phycologist Stanley Milgram's famous experiment ``six degrees of separation''.
Besides social science, this phenomena is also explored and confirmed in many areas even gaming field.
The game ``six degree of Kevin Bacon'' relying on the concept of ``small world phenomenon'', asks players to try to connect any actors to Kevin Bacon in smallest number of links.
The phenomena is also observed from the data of Facebook and LinkedIn.
In Facebook, one of its well-known applications, so-called ``Six Degrees'', collects around $5.8$ million users and shows that the average pairwise shortest distance is $5.73$.
Also, the report from Sysomos~\footnote{http://www.sysomos.com/insidetwitter/sixdegrees/} observes that around half of users on Twitter are on average $4$ steps away from another while nearly everyone is $5$ steps away.

The aforementioned applications all relate to the fundamental problem: finding shortest path within $6$ steps. Indeed,
this is also consistent with basic principle of building social connections that people always make new friendship
through some other close acquaintances.
%This is also equivalent to finding the persons in the shortest path from themselves to the targeted person they want to know.
Motivated by the striking observation -- ``six degree of separation'',
many preliminary efforts from industrial perspective have been imposed for finding shortest path between two persons with distance no greater than 6 in social network.
One of most famous applications is the service ``How you're connected to A'' developed by LinkedIn, which offers a precise description of friendship chain between you and friend A within $3$ steps.
Microsoft's Renlifang~\footnote{http://renlifang.msra.cn/6du.aspx} allows users to retrieve the shortest path between two entities if their distance is smaller or equal to $6$.
The newly emerged online application ``Six Degrees''~\footnote{http://www.6-degreesonline.com} provides an interactive way to demonstrate how you connect to other people in your facebook network.
The efficiency of those applications are far away from the achievement made by real-time routing on road networks.


Recently, the traditional shortest path finding problem has been extensively studied and applied in numerous computing fields.
However, the applicability of existing methods on our six-degree shortest path problem is hindered by the characteristics of social network data.
Unlike the planar network and road network on which most of research focus, social networks have very high vertex degree in addition to their massive size.
The shortest-path processing techniques designed for road networks do not perform well on such massive and dense graphs.
For some methods aiming at estimating exact shortest distance even with guaranteed approximation ratio,
they are still not applicable in our scenario because the length of most shortest paths is very short (no more than $6$ steps) and the involving of small errors will lead to meaningless results.
Indeed, daunting size of dense large-scale networks makes the most simple and basic graph queries extremely difficult and expensive to process.
Consider performing BFS (breath-first search) on Facebook which currently has more than $750$ million active users and average user has $130$ friends.
The number of users needed to be traversed in six-degree shortest path finding procedure can be up to hundreds of billions which is very costly.


\section{Problem Statement}
\label{prob}

Let $G=(V,E)$ be an unweighted and undirected graph where $V=\{1,2,...n\}$ is the vertex set and $E \subseteq V \times V$ is edge set.
The edge from vertex $u$ and $v$ is denoted by $(u,v)$, and we use $P_{v_0, v_p} = (v_0, v_1, ..., v_p)$ to denote a simple path from $v_0$ to $v_p$.
The length of a simple path in unweighted graph is the number of edges in the path.
Given two vertices $u$ and $v$, their shortest path $SP_{u,v}$ is the path between them with minimal length.
The distance from vertex $u$ to $v$ is the length of shortest path $SP_{u,v}$ from $u$ to $v$, denoted by $d(u,v)$.
For each vertex $u$, its $\epsilon$-neighbors, denoted as $N_{\epsilon}(u)$ is a set of vertices such that their distance to $u$ is no greater than $\epsilon$, i.e., $N_{\epsilon}(u) = \{v \in V | 0 < d(u,v) \le \epsilon\}$.
To facilitate our discussion on six-degree shortest path query,
we say vertex $v$ is $6-reachable$ from vertex $u$ if the distance from $u$ to $v$ is no greater than $6$.
If $u$ and $v$ are $6-reachable$ to each other, their shortest paths (maybe more than one) are {\em 6-degree shortest path} $SP_6(u,v)$.


\bdefin{\bf Six-degree Shortest Path Query (6DSP)}
Given a unweighted and undirected graph $G=(V,E)$, and two vertices $u$ and $v$,
if $u$ and $v$ are reachable from each other and their distance $d(u,v) \le 6$ (i.e., $6-reachable$), six-degree shortest path query returns unique shortest path $SP_6(u,v)$ between them.
Otherwise, the query returns null.
\edefin


\section{Search Algorithms without \\ Structural Organization}
\label{searchalgs}

In this section, we adapt existing shortest path computation methods originally on road networks, ALT ($A^\ast$, landmark and triangle inequality) and contraction hierarchy (CH), for our social network searching scenario.
In general, several novel techniques are proposed to incorporate these methods by taking characteristics of social network data into consideration.
Especially, a new landmark selection strategy is introduced for ALT; a novel node ordering scheme and an efficient node contraction method are discussed in CH.


\subsection{ALT}
\label{alt}

ALT is proposed by Goldberg and Harrelson~\cite{GoldbergSODA05} to considerably reduce the search space by combining $A^\ast$ search, landmark technique and triangle inequality.
Generally, landmark and triangle inequality are used to compute the effective lower bound to facilitate bidirectional $A^\ast$ search.
They demonstrate that the performance of bidirectional $A^\ast$ search can be significantly improved by incorporating lower bound computed based on landmarks instead of Euclidean distance.
Analogous to most of online searching algorithms, ALT mainly consists of two steps: preprocessing and online bidirectional $A^\ast$ search.
During preprocessing step, some landmarks are selected according to certain selection strategies.
Then, for each vertex, their distance to landmarks are precomputed and recorded.
When distance queries come, we use the recorded distance to compute lower bounds (one to estimate the distance from current node to destination in forward search, another for the distance from current node to source in backward search),
and apply them in bidirectional $A^\ast$ shortest path algorithm.
The effective lower bound provided by landmarks would allow us to greatly reduce the search space.
In other words, the performance of ALT method largely relies on the effectiveness of landmark selection.

\input{Figures/ALT.tex}

Here, we first revisit ALT framework and then discuss how to select good landmarks in social networks.
The online search procedure is outlined in Algorithm~\ref{alg:altquery}.
Basically, the forward $A^\ast$ search from $s$ and backward $A^\ast$ search from $t$ are performed in an alternative manner.
During bidirectional search, the minimal length of shortest path $\mu$ so far is updated accordingly (Line 13 to 15).
The algorithm terminates when search procedure picks one vertex from priority in one direction which has been scanned in the other direction (Line 9 to 11).
Note that, potential functions $p_f(v)=\frac{1}{2}(\pi_f(v)-\pi_b(v))+\frac{\pi_b(t)}{2}$ and $p_b(v)=\frac{1}{2}(\pi_b(v)-\pi_f(v))+\frac{\pi_f(t)}{2}$,
where $\pi_f(v) = max_{x \in L} |d(v,x)-d(x,t)|$ and $\pi_b(v)=max_{x \in L}|d(v,x)-d(x,s)|$.


Finding good landmarks is critical for the performance of ALT method.
Most straightforward solution is to randomly select a fixed number of vertices as landmarks.
Clearly, we can do much better in landmark selection.
Since the landmark is used to estimate the lower bound, a good landmark tends to lie behind the shortest paths between a pair of vertices.
Some existing empirical studies~\cite{Mislove07} demonstrate the existence of ``core'' structure (highly connected component with small-world phenomena) in large social network.
They demonstrate that ``core'' plays remarkable role in keeping the remainder of social networks connected.
Based on this observation, the boundary nodes whose diameter is rather close to network diameter are able to serve as good landmark
because most of pair of vertices naturally find one vertex in boundary nodes which lies behind one of them.
Our landmark selection procedure extracts the boundary nodes by sampling method.
We sketch the method in Algorithm~\ref{alg:altlandmark}.

\input{Figures/Landmark.tex}

We start the procedure by randomly sampling a set of vertices and generate shortest path tree by performing BFS traversal from those vertices.
For each shortest path tree, we only consider their leaf nodes as landmark candidate and record their distance information $s(w)$ and $c(w)$ (Line 5 to 9).
Intuitively, boundary nodes of social networks frequently appear in the leaves of BFS tree and their distance in corresponding BFS tree is relatively large in general.
Therefore, we rank those landmark candidates by their average distance serving as leaves in BFS trees (Line 11 to 13).
Finally, we pick the top ranked candidates as landmarks.
In order to make landmark uniformly distributed in entire network, the candidates which is close to currently selected landmark is removed from queue (Line 14 to 16).

%\textcolor{blue}{what if consider the combination of average distance and $c(w)$ (frequency serving as leaf nodes)?}

\comment{
general pruning technique, main idea is to compute feasible lower bound by effective landmarks.
how to select good landmarks highly influence the searching performance of ALT.
bidirectional search

basic procedure
1) landmark selection and landmark distance computation for each vertex;
2) compute consistent feasible function value for each vertex;
3) for $(u,v)$ shortest path query, alternatively run forward search and backward search until certain stopping condition is satisfied (make it clear why they are correct).

landmark selection procedure (main spirit: boundary nodes tend to generate good lower bound since it potentially on left side of source or right side of destination)
1) randomly sample a set of nodes as roots, perform BFS from those root nodes, rank the farthest nodes they can reached based on their average distance to those starting nodes;
2) select $5\%$ top ranked nodes as landmarks (boundary nodes, it is defined as a set of vertices whose diameters are very large);
}


\subsection{Contraction Hierarchy}
\label{ch}

Contraction hierarchies~\cite{Geisberger:2008} is one of techniques exploring highway nature of road network to speedup Dijkstra algorithm.
The basic idea is to construct some short cuts which able to skip traversing ``unimportant'' nodes during online search procedure.
As ALT method, it is made up of two steps: node contraction step and query procedure.
In the first step, nodes are firstly ordered according to their ``importance'' (node importance is heuristically evaluated by linear combination of several factors).
We now create the short cut by contracting the nodes following this order and preserve the shortest path information for remaining vertices.
For each vertex $v$, if there is a unique shortest path $P=(u,v,w)$ such that order of both $u$ and $w$ are higher than $v$,
a shortcut edge $(u,w)$ is introduced to graph.
After that, vertex $v$ and all its incident edges are removed from graph.
Eventually, shortcut edges with edges in original graph constitute overlay graph which will be used for online query.
To answer shortest path queries, bidirectional Dijkstra algorithm is adopted in overlay graph from source and from destination respectively.
For forward search, we only relax the edge $(v,w)$ such that order of $w$ is higher than that of $v$.
Similarly, we only relax the edge $(w,v)$ such that the order of $w$ is higher than that of $v$.
The intuition is that both searches from source and from destination ``climb'' toward and meet at more ``important'' vertex (peaks).


\begin{figure}
\centering
\begin{tabular}{c}
\psfig{figure=Figures/ncexample.eps,scale=0.5}
\end {tabular}
\caption {Generating shortcut with length $3$}
\label{fig:ncexample}
\end{figure}

In the following, we describe the node contraction in six-degree shortest path query context provided that node ordering is given.
Afterward, we discuss how to obtain ``good'' node ordering which potentially reduces the number of added shortcut edges.

\input{Figures/NodeContraction.tex}

\noindent {\bf Node Contraction: }
Since we focus on the shortest path with length no greater than $6$,
the length of shortcut edges which are needed in bidirectional search stage should be no more than $6$.
Therefore, instead of generating the shortcut with arbitrary length, we are able to introduce shortcuts in batch based on exiting shortcuts with smaller length.
Generally, according to node ordering, we firstly scan all vertices to generate the shortcut edges with length 2 and record those shortcuts.
In order to generate shortcuts with length $3$, we only need to consider the endpoints of shortcuts with length 2.
In figure~\ref{fig:ncexample}, edge $(4,1)$ is existing shortcut with length $2$.
To generate shortcut with length $3$, we only consider vertex $1$ and its incident vertices like $5$ with higher order, and check if there is alternate shortest path between $4$ and $5$.
For shortcuts with length $4$, there are two combinations: concatenation of $2$ shortcuts with length $2$, or one with length $1$ and another is shortcut with length $3$.
Theoretically, we can repeat this process until shortcut edges with length $6$.
Due to the consideration of reducing preprocessing time, we only generate the shortcut edges with length no more than $4$.
Even for shortest path with length $6$, those shortcuts can help considerably reduce the search space.
The advantage of this algorithm is that we generate the shortcut edges by directly extending existing edges instead of exhaustively checking every pair of each vertex's neighbors in overlay graph.
We summarize the entire node contraction procedure in Algorithm~\ref{alg:nc}.


\noindent {\bf Node Ordering: }
Though many node ordering heuristics are introduced in~\cite{Geisberger:2008}, no objective is formally formalized.
As discussed before, we can see that the number of shortcuts with length $l$ relies on the number of shortcuts with length $l-1$.
Along this line, reducing the number of shortcuts with length $2$ potentially results in fewer shortcuts globally.
Therefore, we now focus on the problem of finding node ordering which achieves minimum number of shortcuts with length $2$.

\bdefin{\bf(Node Ordering Problem)}
Given graph $G=(V,E)$, we try to seek a node ordering $\prec$ on $V$ such that the number of newly added shortcuts with length $2$ ($E_2$) in resulting graph is minimum.
\edefin

\begin{figure}
\centering
\begin{tabular}{c}
\psfig{figure=Figures/nodeorder.eps,scale=0.5}
\end {tabular}
\caption {Linear node ordering}
\label{fig:nodeorder}
\end{figure}

Assuming node ordering is given, we can always collapse the graph into a line following their corresponding orders (see Figure~\ref{fig:nodeorder}).
We now consider whether we need to create a shortcut for a edge $(u,w)$.
Clearly, if there is a intermediary $v$ which is common neighbor of $u$ and $w$ and its order is higher than both $u$ and $w$, no shortcut is needed.
From the viewpoint of vertex $v$, we would say $v$ {\em covers} vertex pair $(u,w)$ if and only if $v \in N(u)$, $v \in N(w)$ and $min(u,w) \prec v$.
Intuitively, vertex with higher order is able to {\em cover} more vertex pairs from its neighbors.
Hence, assigning higher order to vertex covering large number of uncovered vertex pairs naturally becomes reasonable choice.
As the number of vertex pairs with distance $2$ is fixed, more are covered, less shortcuts are probably created.

\input{Figures/GreedyOrder.tex}
%\input{Figures/GreedyOrder1.tex}

We propose an ordering algorithm mimicking greedy algorithms for set cover problem to achieve the goal.
The greedy selection order during procedure is considered as the node ordering.
Let $U = \{(u,v) | d(u,v)=2\}$ including all shortest path with length 2.
For each vertex $v$, it is associated with a set of vertex pairs $C_v=\{(u,w) | d(u,w)=2 \mbox{ and }v\in N(u)\cap N(w)\}$.
We apply greedy selection strategy (Algorithm~\ref{alg:greedyorder}) to obtain the ordering.
During selection procedure, we always pick the vertex that maximally covers the uncovered pairs.
Note that, vertex $x$ is only able to cover the shortest path with both endpoints having lower order than $x$ (i.e., $u,v \notin T$).
To break the tie, we prefer choosing the vertex with larger degree.
This ordering method can also combine with other heuristics to gain better performance.


\comment{
An alternate strategy (Algorithm~\ref{alg:greedyordermin}) directly focuses on minimizing the newly created shortcuts.
In this method, we try to select the node with minimal number of already selected neighbors, because the number of already selected neighbors indicates the amount of potential shortcuts.
Another attractive point is that, we somehow address the uniformity issue such that nodes would be better to be contracted in an uniform order around entire graph instead of concentrating on one region.
If the vertex $v$ is currently selected, all its neighbors potentially create larger number of shortcuts thus are not likely to be selected in the near future.
Note that, to break the tie during selection, we prefer the vertex with larger degree in both algorithms.
These ordering methods can also combine with other heuristics to gain better performance.
}

\comment{
1) node ordering based on $6$-step betweenness (computed by sampling method);
2) fast node contraction (consider 2-hop contraction, 3-hop contraction ...);
}


\section{Search Algorithms with \\ Component-based Structure}
\label{searchalgscomponent}

In this section, we introduce several efficient shortest path finding algorithms based on component structure.
Those components are generated by graph decomposition method.
Basically, social network is organized as star-shape structure such that the central part is the ``core'' of entire graph which entail the major connections among other small outlier components.


\begin{figure}
\centering
\begin{tabular}{c}
\psfig{figure=Figures/starshape.eps,scale=0.5}
\end {tabular}
\caption {Star-shape structure}
\label{fig:starshape}
\end{figure}


\subsection{Graph Decomposition}
\label{decomposition}

The existence of well-connected ``core'' in social network has been demonstrated in empirical studies on several real datasets~\cite{Mislove07}.
By removing a small portion of hub nodes (nodes with high degree), the connectivity of entire graph is significantly break down and forms large number of small-sized components.
They also observe that the distance between two nodes in the ``core'' is roughly $4$ and most of remaining nodes are very few steps away from the core.
According to those interesting observations, social network seems can be organized as a star-shape structure,
where a well-connected core ($C_0$ in Figure~\ref{fig:starshape}) serves as major transportation center bridging the communication between different small components ($C_1$ to $C_7$ in Figure~\ref{fig:starshape}).
Of course, few shortest paths connecting different small components are allowed without involving core component.
Given this star-shape structure, we wish to implement efficient routing for relatively ``long-range'' shortest paths (such as the one with length $5$ or $6$) through central component,
while other ``local'' shortest paths are found within each components.
To meet this goal, we identify certain key properties that good star-shape structure should satisfy:

\noindent 1) {\em Small-sized core with small diameter}: only small portion of vertices (like $5\%$ of total number of vertices) are included in the core;
the length of any shortest path within core is bounded by a small constant.

\noindent 2) {\em Strong connections between core and small components}: most of shortest paths between different small components go through core.

\noindent 3) {\em Weak connections among small components}: few shortest paths among different small components do not involve nodes in the core.

Our algorithm to decompose entire graph into desired structure consists of two main steps:
core extraction step and graph partition on remaining graph.
In the first step, we try to extract the core containing some important segments in the middle part of relatively long-range shortest path (with length $5$ or $6$).
The segment (subpath of ``long-range'' shortest paths) importance is measured by the number of shortest paths go through it (i.e., segment betweenness).
Then, we remove the core from original graph.
For the remaining graph, we apply well-known graph partition software METIS~\footnote{http://glaros.dtc.umn.edu/gkhome/metis/metis/overview} to decompose it into several small components.

\input{Figures/CoreExtraction.tex}

\begin{figure}
\centering
\begin{tabular}{c}
\psfig{figure=Figures/coreshortcut.eps,scale=0.6}
\end {tabular}
\caption {Adding shortcuts}
\label{fig:coreshortcut}
\end{figure}

The core extraction approach is outlined in Algorithm~\ref{alg:coreextraction}.
To begin with, we randomly select a small portion of vertices as roots (Line 2) and perform BFS from those roots to obtain the ``long-range'' shortest paths $P$ with length $5$ and $6$ (Line 5).
All edges in $P$ are stored in a priority queue according to their edge betweenness (Line 6 to 10).
We now concentrate on expanding $V_c$ and $E_c$ by selecting appropriate edges from priority queue (Line 12 to 38).
In the while loop, we iteratively consider the edge with maximum edge betweenness in the current queue (Line 13).
If only one of edge's endpoints $u$ does not belong to core, we check whether this endpoint can be included in core or not.
Especially, we perform BFS by expanding $r$ steps in order to conform if adding this endpoint $u$ still maintains the diameter constraint $r$ (Line 16).
If so, vertex $u$ is included in the core and edge $(u,v)$ is added into $E_c$ (Line 16 to 18).
Since BFS tree $T_u$ might brings some extra vertices to help connect to the core (like vertex $x$ in Figure~\ref{fig:coreshortcut}(a), green ones are vertices in the core),
to maintain $u$'s diameter, we simply add the shortcuts from $u$ to those vertices in the core (like $(u,v_1)$ and $(u,v_2)$ in Figure~\ref{fig:coreshortcut}(b)).
Those operations are summarized in Line 19 to 22.
Another case is that both endpoints $u$ and $v$ are not in the core.
We process both vertices in the same way (Line 25 to 37).
The only difference is that we are allowed to add edge $(u,v)$ if and only if both vertices are contained in the core (Line 34 to 36).
The resulting core is a weighted graph with diameter no more than $r$.


\subsection{Component-based ALT}
\label{compalt}

As mentioned before, landmark selection is playing important role in the performance of ALT.
Here, we propose a method to select landmarks based on the star-shape structure (component-based structure).
For any pair of vertices, a landmark lying behind one of vertices tends to provide tight bound.
Therefore, for random shortest path queries, boundary nodes far away most of vertices would be good choice to be landmark.
In this sense, we consider the landmark selection on the vertices in the small components.
To make sure landmarks are uniformly distributed around the outlier of entire graph, we try to omit the vertices that are close to currently selected one.
By this way, we also avoid putting many landmarks into one component.

To achieve aforementioned goals, we propose a simple landmark selection algorithm based star-shape structure as follows.
For each small component $C_i$, we have a set of vertices $B_i \subseteq C_i$ connecting to the vertices in the core $C_0$.
First, pick a vertex $v$ in $C_1$ that farthest to vertex set $B_1$  and mark the vertices not belonging to core within $3$ steps from $v$ as processed.
Randomly pick one of $C_1$'s neighboring components $C_k$, then select a vertex $u$ that is not marked and farthest away from its corresponding $B_k$.
We proceed such iteration until no landmark can be selected or certain number of landmarks has been selected.
Clearly, we can incorporate those landmarks with ALT method for shortest path routing.


\comment{
\subsection{Component-based CH}
\label{compch}

also consider the relation between unique shortest path system and node order in CH.
}


==> Prop.tex <==
\section{Proposal}

The scale of graph data is increasing more rapidly than ever. For example, Facebook has 500 million active users
interacting with 900 million objects; Microsoft's Renlifang (EntityCube) records over a billion relationships for over
10 million entities (people, locations, organizations); DBpedia RDF graph contains 3.5 million nodes and approximately
150 million triples (edges); The UniProt RDF dataset, which contains information about proteins and their interactions,
currently has almost 1.6 billion triples (edges). Enabling online and interactive query processing of these giga-scale
graphs is becoming an indispensable component for emerging applications from social sciences, biomedical informatics,
advertisement and marketing research, the semantic web, and homeland security. Scientists and practitioners are in
desperate need to grasp and discover new knowledge from these graphs with exceedingly rich information. By allowing
querying and analyzing giga-scale graphs on even desktop computers, we can greatly facilitate, speedup, and ease the
otherwise extremely difficult discovery process on giga-scale graphs. However, the sheer size of these graphs can make
even the most simple and basic graph queries extremely difficult and expensive to process. In this EAGER project, we
aim to attack two fundamental yet notoriously hard queries on giga-scale graphs: the shortest-path distance query and
the label-constraint path query. Both queries are not only essential for numerous emerging graph-processing tasks, but
also the basis for more advanced applications. Providing efficient and scalable approaches for these two queries can
significantly advance our understanding of and capability for managing gagascale graphs. However, the proposed research
is high-risk, as none of the attempts to handle these emerging online queries on giga-scale graphs has successfully
tackled both efficiency and scalability. Existing techniques which work well on mega-scale or relatively sparse graphs
(like road networks) become infeasible on these giga-scale graphs. Path distance is the same measure made famous by
Milgram¡¯s Six Degrees of Separation. Computing shortest-path distance is a key functionality for people search in a
social network, as it provides a rank for each user based on its closeness to the query user. It is also the basis for
a social graph query (as in Microsoft's Renlifang) which returns a shortest-path between any two people if their
distance is smaller than a certain threshold. The existing approaches are based on simple adoptions of either BFS or
partial materialization. These methods are adequate when the number of vertices as well as edges is either small or
sparse. Though existing techniques are very successful for large but sparse graphs, these emerging giga-scale graphs
have quite different characteristics. Instead of being spatial, with edge weight, and having low vertex degree, they
are non-spatial, non-weighted, and have very high vertex degree in addition to their massive size. The shortest-path
processing techniques designed for road networks do not perform well on massive and dense graphs. Recently, in the
field of complex network, backbone structures (a core substructure of vertices and edges) have been discovered to take
a center role in network communication and coordination. Though there is no explicit highway structure in the road
network, such backbones still enable the communication and coordination in those much more complex networking systems.
In this project, we plan to leverage the backbonetheory to construct index and facilitate query processing for
giga-scale graphs. In addition, we will study how to utilize the state-of-the-art bipartite set cover framework to help
minimize the labeling cost and deliver query efficiency. Finally, we will apply adaptive sampling and other
approximation approach to deal with scalability. We believe though this is a high-risk approach as it tries to leverage
several emerging technologies to address the shortestpath computation problem, our earlier work on 3-hop reachability
(SIGMOD'09) and the latest work on privacypreserving shortest path computation in Cloud (SIGMOD'11) do prepare us to
attack this problem successfully.


==> Query.tex <==
\section{Exact and Fast Shortest Path \\ Query Processing}
\label{query}
 
To find the $6$-degree shortest path (or $k$ in general) between vertex pair $(s,t)$, our query processing procedure in Hub$^2$-Labeling framework consists of two steps:

\noindent{\bf Step 1 (Distance Estimation): } Using the distance matrix Hub$^2$ and core-hubs labeling $L_{H}(s)$ and $L_{H}(t)$, we approximate the distance  $d_H(s,t|\mathcal{H})$ and the shortest path $SP_H(s,t|\mathcal{H})$ as follows:
\beqnarr
\label{recovereqn}
d_H(s,t|\mathcal{H}) = min_{x \in L_{H}(s) \wedge y \in L_{H}(t)} \{ d(s,x)+d(x,y)+d(y,t) \} \nonumber \\
SP_H(s,t|\mathcal{H}) = SP(s,x^\ast) \circ SP(x^\ast,y^\ast) \circ SP(y^\ast,t) \ \ \  (*)\nonumber \\
\text{ where } (x^\ast,y^\ast) = \underset{x \in L_{H}(s) \wedge y \in L_{H}(t)}{\operatorname{argmin}} d(s,x)+d(x,y)+d(y,t) \nonumber
\eeqnarr
%If $d_H(s,t|L) > 6$, we set $d_H(s,t|L)=6$ and $SP_H(s,t|L)=\emptyset$.

\noindent{\bf Step 2 (Hub-Avoidance Bidirectional BFS (HBBFS)):} A bidirectional BFS from $s$ and $t$ is performed and the search step is constrained by the minimum between $k$ (for $k$-degree shortest path) and $d_H(s,t|\mathcal{H})$. 
In particular, none of the hubs in the hub-set $\mathcal{H}$ need to be expanded during the bidirectional search. 
Thus, the bidirectional BFS search can effectively prune the search space.

In Subsection~\ref{bidirection}, we present the  Hub-avoidance Bidirectional BFS and prove its correctness. 
In Subsection~\ref{fastestimation}, we introduce techniques to speed up the estimation process (in Step $1$) and compact representation for recovering the shortest path (also in Step $1$). 
 
\subsection{Fast Hub-Avoidance Bidirectional BFS} 
\label{bidirection}
The fast hub-avoidance bidirectional BFS is sketched in Algorithm~\ref{alg:step2query}.
Note that {\em BackwardSearch} is essentially the same as the {\em ForwardSearch} and is omitted for simplicity.  
Initially, the $dist$ is determined to be the smallest one between the length of shortest path $d_H(s,t|\mathcal{H})$ and $6$ (or $k$ in general) (Line 3).
The main loop employes a forward search and a backward search in an alternating manner (Lines $4-12$).
In the BFS search procedure {\em ForwardSearch} (and {\em BackwardSearch}), 
each hub in $\mathcal{H}$ is excluded from the queue to avoid expanding their neighbors (Line 9).
Note that, the typical stop condition in the bidirectional search is that one direction visit a vertex already scanned in the other direction.
To fully utilize $d_H(s,t|L)$ as upper bound, we adopt a better criterion: the search terminates when the sum of distance labels of top elements in queues of the forward search and the backward search is no less than the length of shortest path seen so far (Line 10). We note that this criterion is firstly introduced in~\cite{GoldbergW05}.

\input{Figures/BiBFSQuery.tex}

The correctness of our query processing procedure can be observed as follows. 
Any vertex pair with distance no more than $6$ can be decomposed into two categories:
1) vertex pairs having at least one shortest path passing through at least one hub in the hub-set $\mathcal{H}$;
and 2) vertex pairs whose shortest paths never pass through any hub in $\mathcal{H}$.
Clearly, there is no overlapping between these two categories.
Lemma~\ref{step1lemma} confirms that {\em a shortest path between vertex pairs in the first category can always be found in Step $1$.}

\blemma
\label{step1lemma}
Given graph $G=(V,E)$ and hub-set $\mathcal{H}$, for any vertex pair $(s,t)$ with distance no greater than $6$ (i.e., $d(s,t) \le 6$), if there exists one hub $x^\prime \in \mathcal{H}$ satisfying $d(s,t)=d(s,x^\prime)+d(x^\prime,t)$,
then, we can always find $x \in L_{H}(s)$ and $y \in L_{H}(t)$ such that $d(s,t)=d(s,x)+d(x,y)+d(y,t)$.
\elemma
Its proof is similar to the one for Lemma~\ref{goodcorepath} and is omitted for simplicity. 
Basically, if there exists a $6$-degree shortest path between $u$ and $v$ which passes through a hub $x^\prime \in \mathcal{H}$,
then, we guarantee to recover one of such paths using the core-hub labeling together with the distance-matrix Hub$^2$. 
Specifically, such a shortest path is described by Equation (*). 
%~\ref{recovereqn}. 
If such an approximate shortest path computed in Step $1$ is not an exact one, we can guarantee to extract an exact shortest path in Step 2 using the local bidirectional search.

\blemma
\label{step2lemma}
Given graph $G=(V,E)$ and hub-set $\mathcal{H}$, for any vertex pair $(s,t)$ with distance $d(s,t) \le 6$,
if estimated distance $d_H(s,t|\mathcal{H}) > d(s,t)$,
Algorithm~\ref{alg:step2query} can always discover an exact shortest path (with no intermediate hub in $\mathcal{H}$).
\elemma
\bproof
Without loss of generality, suppose $SP(s,t)=(u_0,...,u_p)$ ($1 \le p \le 6$) is any shortest path from $s$ to $t$, where $u_0=s$ and $u_p=t$.
As estimated distance is greater than exact distance, $SP(s,t)$ is not found in Step $1$, meaning $u_i \notin L$ ($0 \le i \le p$) (according to lemma~\ref{step1lemma}).
Now, we consider a new graph $G^\prime=(V\setminus \mathcal{H}, E^\prime)$ by removing all hubs in $\mathcal{H}$ and their incident edges from original graph $G$.
It is not hard to see that, all shortest paths $SP(s,t)$ from $s$ to $t$ are still preserved in the graph $G^\prime$,
because every edge involved in these shortest paths is not incident to hubs in $\mathcal{H}$.
On the other hand, Algorithm~\ref{alg:step2query} is essentially equivalent to performing traditional bidirectional BFS on new graph $G^\prime$.
Therefore, we are able to find one $SP(u,v)$ using traditional bidirectional BFS on $G^\prime$ (Step $2$).
\eproof



\subsection{Fast Estimation and Shortest Path \\ Extraction}
\label{fastestimation}

Here, we discuss several techniques to speed up the distance estimation and compactly store the precomputed shortest paths. 

\begin{figure}
\centering
\begin{tabular}{c}
\psfig{figure=Figures/jointorder.eps,scale=0.65}
\end {tabular}
\caption{Levelwise Organization of Core-Hubs}
\label{fig:jointorder}
\end{figure}

\noindent{\bf Core-Hubs Levelwise Organization and Fast Distance Estimation:}
Given any vertex pair $(s,t)$ and their landmark indices $L_{H}(s)$ and $L_{H}(t)$,
the straightforward approach to estimate their shortest path is to perform a pairwise join on $L_{H}(s)$ and $L_{H}(t)$ based on Eq.~\ref{corepath}. This takes a total of $|L_{H}(s)| \times |L_{H}(t)|$  comparisons, which can be rather expensive.
To address this issue, we rank and store the core-hubs in $L_H(u)$ according to their distance to $u$ and utilize such structure for effectively pruning. 
\comment{
We observe that, when we check landmark pair $x \in L_{H}(s)$ and $y \in L_{H}(t)$,
if the shortest distance so far $dist$ is smaller than $d(s,x)+d(y,t)$, then we do not need to actually perform join comparison on $(x,y)$.
Further, any landmark pair satisfying such condition is not necessary to be accessed in the future, which potentially avoids many pairwise join operations.}


Specifically, we decompose  $L_{H}(u)$ into $6$ sublists $L^k_{H}(u)$,
where each sublist $L^k_{H}(u)$ contains hub $x_i$ with distance to $u$ is $k$, i.e., $d(u,x_i) = k$ ($1 \le k \le 6$).
Given this, pairwise join on $L_{H}(s)$ and $L_{H}(t)$ becomes pairwise join on two sets of sublists $L^k_{H}(s)$ ($1 \le k \le 6$) and $L^{k^\prime}_{H}(t)$ ($1 \le k^\prime \le 6$).
As shown in figure~\ref{fig:jointorder}, the connection between upper $L^p_{H}(s)$ and lower $L^q_{H}(t)$ indicates possible pairwise join on two sublists.
The value attached to each connection is the sum of distances $d(s,x)+d(y,t)=p+q$, where $x \in L^p_{H}(s)$ and $y \in L^q_{H}(t)$.
There is no connection between $L^4_{H}(s)$ and $L^4_{H}(t)$, because $d(s,x^\prime)+d(y^\prime,t)=8 > 6$ (i.e., the upper bound is $6$ in the $6$-degree shortest path query), where $x^\prime \in L^4_{H}(s)$ and $y^\prime \in L^4_{H}(t)$.

Using such a levelwise organization, we perform pairwise join on two sublists following the ascending order of value attached to corresponding connections between these two sublists (shown in Figure~\ref{fig:jointorder}).
Basically,  we first perform pairwise join on $L^1_{H}(s)$ and $L^1_{H}(t)$; then on $(L^1_{H}(s),L^2_{H}(t))$, $(L^2_{H}(s),L^1_{H}(t))$,$(L^2_{H}(s),L^2_{H}(t))$,..., etc. 
Given this, let us denote $d$ to be the shortest path length obtained by pairwise join so far.
Assuming we are currently working on landmarks from sublist pair $(L^p_{H}(s),L^q_{H}(t))$,
if $d < p+q$, then we terminate the pairwise join immediately. 
This is because the following sublist pair $(L^{p^\prime}_{H}(s),L^{q^\prime}_{H}(t))$ is impossible to produce better result since they have $p^\prime+q^\prime \ge p+q > d$.
This early termination strategy based on the levelwise organization can help us effectively prune unnecessary pairwise join operations and improve the query efficiency.

\noindent{\bf Compact Path Representation and Fast Extraction:}
For each vertex $u$,  its hub index $<x_i: d(x_i,u),SP(x_i,u)> \in L_{H}(u)$ can be simplified as
$<x_i,SP(x_i,u)>$ using the levelwise organization. 
However, the explicit materialization of shortest path $SP(x_i,u)$ can still be rather expensive. 
To deal with this problem, we utilize the idea from IP routing table stored in each router for delivering IP packages. 
In the IP routing table, each entity basically contains two elements $<portID,destination>$,
where $portID$ indicates the position of neighboring routers which could help deliver the package to destination.
Simply speaking, $portID$ tells us what is the next step to reach destination using local information.
Given this, instead of recording entire path, we use one port number $portID(u,y_i)$ to denote the next vertex of $u$ which leads to $y_i$ along shortest path $SP(u,y_i)$. 
Thus, an entry $<x_i,SP(x_i,u)> \in L_H(u)$ ($7$ integers in the worst case) is simplified as $<x_i,portID(u,y_i)>$ ($2$ integers), which can significantly save the memory.

\comment{
Moreover, since the next vertex $u^\prime$ in $SP(u,y_i)$ from $u$ should be $u$'s immediate neighbor,
$portID(u,y_i)$ can be the offset of $u^\prime$ in $u$'s adjacent list.
For example, $u$ has neighbors $(u_1,u_2,u_3,u_4)$ ordered by their IDs, then their corresponding $portID$ should be $(0,1,2,3)$.
In this sense, triple $<x_i,SP(x_i,u)>$ ($7$ numbers in the worst case) is simplified as $<x_i,portID(u,y_i)>$ ($2$ numbers), which significantly save the memory.
In our implementation, we use $3$ bytes to store landmark id $x_i$ and $3$ bytes to record $portID$, thus each index takes $6$ bytes in total.
%\noindent{\bf Shortest Path Estimation: }
}

Now, let us consider how to effeciently extract the shortest path $SP_H(s,t|\mathcal{H})$ using the above compact representation. 
First, given vertex pair $(s,t)$, if both $s$ and $t$ are hubs, we can directly obtain their shortest path from the distance matrix Hub$^2$.
Otherwise, we apply the following procedure: 
We start by finding two intermediate hubs $x \in L_{H}(s)$ and $y \in L_{H}(t)$ which achieves minimal value of $d(s,x)+d(x,y)+d(y,t)$. This is done using the speedup techniques based on the the levelwise organization of the core-hubs.
Since the shortest path between hubs $SP(x,y)$ is directly materialized in Hub$^2$, we focus on constructing $SP(s,x)$ and $SP(y,t)$. 
Let us start with $SP(s,x)$: 
{\em
Staring from $s$, we are able to obtain the next vertex in $SP(s,x)$ by checking its landmark indices $<x,portID(s,x)>$.
The $portID$ together with $s$'s adjacent list can identify the next vertex $s_1$ of $s$ leading to $x$ through shortest path.
Then, we turn to extracting the next vertex $s_2$ of $s_1$ in the shortest path $SP(s_1,x)$ by the same means.
We repeat this process until $s_p$ is the immediate neighbor of hub $x$, then we have the vertex sequence $(s,s_1,...,s_p,x)$ as shortest path.}
Similarly, we can extract the vertex sequence $(y,t_q,...,t_1,t)$ to represent $SP(y,t)$.
Finally, we concatenate three vertex sequences and form resulting estimated shortest path: $SP_H(s,t|\mathcal{H})$$=$$(s,s_1,...,s_p,x,...,y,t_q,...,t_q,t)$.









\comment{
Given landmarks $L$, for any vertex pair $(s,t)$, we are able to approximate their shortest path and distance by following expression:
{\small
\beqnarr
d^c(s,t|L) = min_{x \in L^c_{out}(s) \wedge y \in L^c_{in}(t)} \{ d(s,x)+d(x,y)+d(y,t) \} \nonumber \\
SP^c(s,t|L) = SP(s,x^\ast) \circ SP(x^\ast,y^\ast) \circ SP(y^\ast,t) \nonumber \\
\text{ where } x^\ast = \underset{x \in L^c_{out}(s) \wedge y \in L^c_{in}(t)}{\operatorname{argmin}} d(s,x)+d(x,y)+d(x,t) \nonumber
\eeqnarr
}
Note that, since this is only used to estimate the shortest path,
we do not consider the length constraint here, such that estimated path length is not greater than $6$.

Recall that our goal is to generate the {\em exact} shortest path with length no greater than $6$.
In the following, we introduce an important observation which would suggest...



Given the local landmark indices, we are only able to approximate the shortest path between any two vertices.
As any small error arisen by approximation is not acceptable in social networks with small diameters,
we aim at finding one exact shortest path for any vertex pair here.
To achieve this goal, we describe an efficient query processing procedure by leveraging local landmark indexing and bidirectional BFS.
Specifically, given vertex pair $(s,t)$, the query procedure typically involves two steps:

\noindent 1) we generate one approximated shortest path $SP(s,t|V^\ast)$ (distance $d(s,t|V^\ast)$) utilizing local landmark indices $L^e_{out}(s)$ and $L^e_{in}(t)$;

\noindent 2) a variant of bidirectional BFS is employed to complement inaccurate result generated by landmark-based method in order to obtain exact shortest path.

\input{Figures/queryAlg.tex}

Rather than traditional bidirectional BFS accessing the vertices from both direction without any constraint,
our new method utilizes the distance obtained from step 1 as upper bound to reduce the search space.
On the other hand, as we know, if the exact shortest path goes though some landmarks, it would be guaranteed to be found in the step 1.
Therefore, during BFS traversal procedure, we do not need to access landmarks which are essentially high-degree vertices in the social network.
This would further dramatically reduce the search space which is caused by accessing high-degree vertices with even hundreds of thousands of neighbors in the social network.
}

